Flexibility of Two-Dimensional Euler Flows with Integrable Vorticity

We propose a new convex integration scheme in fluid mechanics, and we provide an application to the two-dimensional Euler equations. We prove the flexibility and nonuniqueness of $L^\infty L^2$ weak solutions with vorticity in $L^\infty L^p$ for some $p>1$, surpassing for the first time the critical scaling of the standard convex integration technique. To achieve this, we introduce several new ideas, including: (i) A new family of building blocks built from the Lamb-Chaplygin dipole. (ii) A new method to cancel the error based on time averages and non-periodic, spatially-anisotropic perturbations.

==> April_7_2024_FILE.tex <==



\begin{abstract}
We propose a new convex integration scheme in fluid mechanics, and we provide an application to the two-dimensional Euler equations. We prove the nonuniqueness of $L^2$ solutions with vorticity in $L^p$ for some $p>1$, surpassing for the first time the critical scaling of the standard convex integration technique.

To achieve this, we introduce several new ideas, including:
\begin{itemize}
    \item[(i)] A new family of building blocks built from the Lamb-Chaplygin dipole,
    
    \item[(ii)] A new method to cancel the error based on time averages and spatially-anisotropic perturbations.
\end{itemize}
\end{abstract}


{\color{blue}
\begin{enumerate}[label = (\roman*)]
    \item AK: It might be a good idea to not use the phrase `it is immediate' too often as it makes the writing monotone. Also, do not forget to provide the correct reference to equations from where the `immediate' thing follows.
\end{enumerate}
}








\section{Introduction}






\section{Principal Building Block}
\label{sec: principal bb}

In this section, we construct the principal building block velocity field for our convex integration scheme. The main ingredient of our construction is the {\it Lamb--Chaplygin dipole}, an exact solution of the 2D Euler equation on $\mathbb{R}^2$, which translates with constant velocity without deforming.
Our main goal is to find an approximate solution corresponding to this dipole on $\mathbb{T}^2$, through a patching argument. 

\bigskip

The Lamb--Chaplygin dipole consists of two regions: a circular inner core of some fixed radius where the vorticity of opposite signs concentrate, and the complement of the core where the velocity field is irrotational and coincides with the {\it doublet flow}.
The Lamb--Chaplygin dipole can be understood as the desingularization of the doublet flow.





% The Lamb--Chaplygin dipole in exact solution defined on $\mathbb{R}^2$. We find an approximate solution corresponding to this dipole on $\mathbb{T}^2$ through a patching argument. 

% We first define a periodic analog of the doublet flow with the help of a Weierstrass $\wp$ function. The idea is that the periodic doublet in the leading order is the same as the doublet flow close to the singularity at the origin. Therefore, in the outside region of the Lamb--Chaplygin dipole, we patch it with the periodic doublet with the help of a cutoff function. We show that the errors generated in the process of patching are quite small. In the next few subsection, we carry out this construction process.




\subsection{Doublet Flow on $\mathbb{R}^2$}
\label{subsec: doublet}
A doublet flow is a divergence-free potential flow on $\mathbb{R}^2 \setminus \{0\}$. We denote as $x=(x_1,x_2)\in \R^2$ points in the Euclidean plane.
In complex notation, the potential $\wt{\Phi}$ and the stream function $\wt{\Psi}$ of the doublet flow are given by
\begin{align}
\wt{\Phi}(x_1, x_2) + i \wt{\Psi}(x_1, x_2) \coloneqq - \frac{1}{z}, \quad \text{where} \quad z = x_1 + i x_2\, .
\end{align}
We define the velocity field $\wt{V} = (\wt{V}_1, \wt{V}_2)$ as
\begin{align}
\wt{V}_1(x_1, x_2) - i \wt{V}_2(x_1, x_2) \coloneqq  \frac{1}{z^2}\, .
\end{align}
From our definition, it is clear that
\begin{align}
\wt{V} = {\color{blue} -}\nabla^\perp \wt{\Psi} = \nabla \wt{\Phi}\, ,
\label{principal bb: V tilde}
\end{align}
{\color{blue}for Anuj: here I am not sure about signs, I added a minus sign to make 2.2 and 2.3 agree but this would impact the rest. Perhaps we should instead change sign of $\tilde V_1$ in 2.2?}
where $\nabla^\perp = (-\partial_2,  \partial_1)$. Next, we define the pressure field
\begin{align}
\wt{P} = \partial_1 \wt{\Phi} - \frac{|\nabla \wt{\Phi}|^2}{2}.
\label{principal bb: P tilde Phi tilde}
\end{align}
and notice that
\begin{equation}\label{eq:doublet1}
    -\partial_1 \wt{V} + (\wt{V} \cdot \nabla) \wt{V} + \nabla \wt{P} = 0 \, ,
    \quad \text{on $\R^2 \setminus \{0\}$}\, .
\end{equation}







\begin{lemma}
\label{lemma: div tensor V x}
For the velocity field $\wt{V}$ as defined in (\ref{principal bb: V tilde}) for $x \in \mathbb{R}^2 \setminus \{0\}$, we have
\begin{align}
\div (\wt{V} \otimes x) = 0.
\label{principal bb: div tensor V x}
\end{align}
\begin{proof}
The conclusion follows from the following identities
\begin{align}
\wt{V}_1(x_1,x_2)  x = %{\color{blue}-}
\nabla^\perp \left(\frac{x_1 x_2}{x_1^2 + x_2^2}\right) \qquad \text{and} \qquad \wt{V}_2(x_1,x_2)  x = %{\color{blue}-}
\nabla^\perp \left(\frac{x_2^2}{x_1^2 + x_2^2}\right)\, .
\end{align}
\end{proof}
\end{lemma}
For a given $r > 0$, we define rescaled doublet flow as follows:
\begin{align}
\wt{\Phi}_{r}(x) = \wt{\Phi}\left(\frac{x}{r}\right), \quad 
\wt{\Psi}_{r}(x) = \wt{\Psi}\left(\frac{x}{r}\right), \quad 
\wt{V}_{r}(x) = \frac{1}{r}\wt{V}\left(\frac{x}{r}\right), \quad
\wt{P}_{r}(x) = \frac{1}{r^2}\wt{P}\left(\frac{x}{r}\right) \, .
\end{align}
{\color{blue} It is then immediate to check} from
 \eqref{eq:doublet1} that
\begin{align}\label{eq:doublet2}
- \frac{1}{r} \partial_1 \wt{V}_{r} + (\wt{V}_{r} \cdot \nabla) \wt{V}_{r} + \nabla \wt{P}_{r} = 0\, , \quad
\text{for every $x\in \R^2\setminus \{0\}$}\, .
\end{align}
Notice that, by homogeneity we have
\begin{equation}
    \wt{\Phi}_r = r \wt{\Phi} \, ,
    \quad
    \wt{\Psi}_r = r \wt{\Psi} \, ,
    \quad
    \wt{V}_r = r \wt{V} \, ,
\end{equation}
hence, {\color{blue} it is immediate to check} the following estimates
\begin{align}
|\nabla^n \wt{\Psi}_r| \leq C(n) \frac{r}{|x|^{n+1}}, \quad 
|\nabla^n \wt{\Phi}_r| \leq C(n) \frac{r}{|x|^{n+1}}, \quad 
|\nabla^n \wt{V}_r| \leq C(n) \frac{r}{|x|^{n+2}} \, ,
\label{principal bb: estimates on doublet}
\end{align}
for every $n\in \N$.







\subsection{Desingularization of the Doublet Flow: The Lamb--Chaplygin Dipole}

To describe the velocity field in this section, we use polar coordinates $\rho$ and $\theta$, where $x_1 = \rho \cos\theta$ and $x_2 = \rho \sin \theta$. 

The Lamb--Chaplygin dipole is a desingularization of the doublet flow \cite{meleshko1994chaplygin}. It consists of two regions: 

\begin{itemize}
    \item[(i)] $\rho \leq 1$ the desingularized region, where the vorticity is nonzero,

    \item[(ii)] $\rho \geq 1$, where the flow is potential given in section \ref{subsec: doublet}.
\end{itemize}
We define the stream function $\ol{\Psi}$ for this flow as
\begin{align}
\ol{\Psi} \coloneqq 
\begin{cases}
\rho \sin \theta - \frac{2 J_1(b\rho)}{b J_0(b)} \sin \theta \qquad & \text{when} \quad \rho \leq 1, \\
\frac{\sin \theta}{\rho} \qquad & \text{when} \quad \rho \geq 1. 
\end{cases}
\end{align}
Here, $J_0$ and $J_1$ are the Bessel functions of first kind of zero and first order respectively. The number $b \approx 3.831705970\dots$ is the first non-trivial zero of $J_1$. It is clear that for $\rho \geq 1$
\begin{align}
\ol{\Psi} = \wt{\Psi}.
\end{align}
Using this stream function, we define the velocity field as
\begin{align}
\ol{V} ={\color{blue}-} \nabla^\perp \ol{\Psi}.
\end{align}
We note that 
\begin{align}
\ol{V} = \nabla \wt{\Phi}, \quad \text{when } |x| > 1.
\label{principal bb: lc outside rad 1}
\end{align}
The velocity field defined in such a way belongs to $C^{1, 1}$, i.e., the derivative is Lipschitz. We define the pressure field in the two regions separately as well. 
\begin{align}
\ol{P} = \ol{V}_1 - \frac{b^2}{2} (\ol{\Psi} - x_2)^2 - \frac{\ol{V}_1^2 + \ol{V}_2^2}{2} \quad \text{for} \quad \rho \leq 1, \qquad \qquad \ol{P} = \ol{V}_1 - \frac{\ol{V}_1^2 + \ol{V}_2^2}{2} \quad \text{for} \quad \rho \geq 1.
\end{align}
Finally, we define the rescaled variables for a given $r > 0$ as
\begin{align}
\ol{\Psi}_{r} = \ol{\Psi}\left(\frac{x}{r}\right), \quad 
\ol{V}_{r} = \frac{1}{r}\ol{V}\left(\frac{x}{r}\right), \quad
\ol{P}_{r} = \frac{1}{r^2}\ol{P}\left(\frac{x}{r}\right).
\label{principal bb: scaled lamb chaplygin}
\end{align}
A simple computation shows
\begin{align}
- \frac{1}{r} \partial_1 \ol{V}_{r} + (\ol{V}_{r} \cdot \nabla) \ol{V}_{r} + \nabla \ol{P}_{r} = 0\, .
\label{principal bb: scaled lamb chaplygin eqn}
\end{align}
From our definition, we note the following estimates
\begin{align} 
|\nabla^n \ol{V}_r| \leq C(n) \frac{1}{r^{n+1}} \quad \text{when } |x| < r \qquad \text{and} \qquad |\nabla^n \ol{V}_r| \leq C(n)  \frac{r}{|x|^{n+2}} \quad \text{when } |x| > r.
\label{principal bb: estimate on Vbar}
\end{align}


\subsection{Decomposition of the Lamb--Chaplygin Vortex}
\label{subsec:Lamb-Chaplygin}

Fix $\alpha\in (0,1)$. We consider a smooth cutoff function $\rchi : [0, \infty) \to \mathbb{R}$ such that $\rchi(x)=0$ for $x\leq 1 $, and $\rchi(x) = 1$ for $x\geq 2$. Define
\begin{align}\label{def:cutoff}
\rchi_\alpha(x):= \rchi\Big(\frac{|x|}{r^\alpha}\Big) \, ,
\end{align}
a pressure field $\Pi : \mathbb{R}^2 \to \mathbb{R}$ as 
\begin{align}
\Pi(x) \coloneqq \rchi_\alpha(x) \wt{\Phi}_r(x) = r \chi_\alpha(x) \wt{\Phi}(x)\, . 
\label{principal bb: req pressure}
\end{align}
and a velocity field
\begin{align}
W_r(x) \coloneqq 
\ol{V}_r(x) - \nabla \Pi(x) =
\ol{V}_r(x) - r\nabla (\rchi_\alpha(|x|) \, \wt{\Phi}(x)).
\label{principal bb: decomposition}
\end{align}
Notice that $W_r$ is not divergence-free. Indeed,
\begin{align}\label{divWr}
\div W_r = - \Delta (\rchi_\alpha \wt{\Phi}_r) = \Delta \rchi_\alpha \wt{\Phi}_r + 2 \nabla \rchi_\alpha \cdot \nabla \wt{\Phi}_r \, .
\end{align}



\begin{lemma}
\label{lemma: properties Pi Wr}
Let $\Pi$ and $W_r$ be as defined in (\ref{principal bb: req pressure}) and (\ref{principal bb: decomposition}), respectively. Then the following statements hold.
\begin{enumerate}[label = (\roman*)]
\item $\supp \Pi \subseteq \mathbb{R}^2 \setminus B_{r^\alpha}(0)$ and $\supp W_r \subseteq B_{2 r^\alpha}(0)$,

\item $\norm{W_r}_{L^1} \leq C(\alpha) r |\log r|$, and $\norm{W_r}_{L^p} \leq C(p) r^{\frac{2}{p} - 1}$ for every $p \in (1, \infty]$,
\item 
$
{\color{blue}\norm{D  W_r}_{L^p} }\leq C(p) r^{\frac{2}{p} - 2}$ for every $p\in (1,\infty]$, and  $\norm{\div W_r}_{L^p} \leq C(p) \, r^{1 - \alpha} \, r^{\alpha \left(\frac{2}{p} - 2\right)}$ for every $p\in [1,\infty]$.
\\
{\color{red}
$\norm{\div \nabla W_r}_{L^p} \leq C(p) \, r^{1 - 2 \alpha} \, r^{\alpha \left(\frac{2}{p} - 2\right)}$}\footnote{EB: this is not used in the current version}
\item 
\begin{align}
\frac{1}{r}\int_{\mathbb{R}^2} W_r = 
\begin{pmatrix}
2 \pi \\
0
\end{pmatrix}.
\label{principal bb: main Wr integral}
\end{align}
\end{enumerate}
\end{lemma}
\begin{proof}
The first item (i) {\color{blue} immediately follows} from (\ref{principal bb: req pressure}), (\ref{principal bb: lc outside rad 1}), (\ref{principal bb: scaled lamb chaplygin}) and (\ref{principal bb: decomposition}).
From \eqref{def:cutoff} and (\ref{principal bb: estimates on doublet}), we obtain 
\begin{align}
|\Pi| \leq C \frac{r}{|x|}\, ,
\qquad
|\nabla \Pi| \leq C \frac{r}{r^\alpha} \frac{1}{|x|} + C \frac{r}{|x|^2}\, , \qquad 
|\nabla^2 \Pi| \leq C \frac{r}{r^{2 \alpha}} \frac{1}{|x|} + C \frac{r}{|x|^3}\, ,
\label{principal bb: estimate Pi nn}
\end{align}
for every $x\in \R^2$.
As $W_r \equiv \ol{V}_r$ when $x \in B_{r^\alpha}(0)$, from (\ref{principal bb: estimate on Vbar}) we get that
\begin{align}
|W_r| \leq C \frac{1}{r} \quad \text{when} \quad |x| \leq r, \qquad 
 |W_r| \leq C \frac{r}{|x|^2} \quad \text{when} \quad r < |x| \leq 2r^\alpha \, .
 \label{principal bb: est 1 Wr}
\end{align}
Combining (i) with (\ref{principal bb: est 1 Wr}), (ii) easily follows.


\bigskip

{\color{blue} Maria'sTODO For the derivative of the velocity field $W_r$, we note that $\nabla \times W_r = \nabla \times \ol{V}_r$, so $\nabla \times W_r = 0$ on $|x|>r$ since $\ol{V}_r$ coincides with the doublet flow. Moreover 
\begin{equation}
    |\nabla \times W_r| \leq |\nabla \ol{V}_r| \leq C \frac{1}{r^2} \quad \text{when} \quad |x| \leq r \, ,
    \label{principal bb: estimate on curl Wr}
\end{equation}
and the estimate on the $L^p$ norm of $\nabla \times W_r$  follows. \\
AK: $\nabla \times W_r$ is also not zero in the annulus.
}{\color{red} For the curl of the velocity field $W_r$, we note that $\nabla \times W_r = \nabla \times \ol{V}_r$, so $\nabla \times W_r = 0$ on $|x|>r$ since $\ol{V}_r$ coincides with the doublet flow. Moreover 
\begin{equation}
    |\nabla \times W_r| \leq |\nabla \ol{V}_r| \leq C \frac{1}{r^2} \quad \text{when} \quad |x| \leq r \, ,
    \label{principal bb: estimate on curl Wr}
\end{equation}
and the estimate on the $L^p$ norm of $\nabla \times W_r$  follows. \\
AK: $\nabla \times W_r$ is also not zero in the annulus.
}
% {\color{red}
% MARIA: IN LINE AND NOT FORMULA
% \begin{align}
% & |\nabla \times W_r| \leq |\nabla \ol{V}_r| \leq C \frac{1}{r^2} \quad \text{when} \quad |x| \leq r,  \nonumber \\
% & |\nabla \times W_r| \leq |\nabla \ol{V}_r| + |\nabla \Pi| \leq C r^{1 - 3\alpha} \quad \text{when} \quad r^\alpha \leq |x| \leq 2 r^{\alpha}, \nonumber 
% \\
% & \nabla \times W_r \equiv 0, \quad \text{otherwise}. 
% \label{principal bb: estimate on curl Wr}
% \end{align}
% }
% The estimates (\ref{principal bb: estimate on curl Wr}) provides the required $L^p$ estimate on the curl of $W_r$ as stated in (iii). 
Then, we note that $\div W_r$ is nonzero only in the annulus $B_{2 r^\alpha}(0) \setminus B_{r^\alpha}(0)$ and that $|\div W_r| \leq C r^{1 - 3 \alpha}$, which completes the proof of (iii).


\bigskip

Finally, we compute the space integral of $\frac{1}{r}W_r$. From equation \eqref{divWr} and integrating by parts twice, we obtain
\begin{align}
\frac{1}{r}\int_{\mathbb{R}^2} W_r \, {\rm d} x & = - \frac{1}{r}\int_{\mathbb{R}^2} \div W_r
\begin{pmatrix}
    x_1 \\
    x_2
\end{pmatrix} \, {\rm d} x  \nonumber \\
& = \frac{1}{r}\int_{\mathbb{R}^2} \left(\Delta \rchi_\alpha \wt{\Phi}_r + 2 \nabla \rchi_\alpha \cdot \nabla \wt{\Phi}_r\right)
\begin{pmatrix}
    x_1 \\
    x_2
\end{pmatrix} \, {\rm d} x
\nonumber\\ \nonumber
& = - \frac{1}{r}\int_{\mathbb{R}^2}   \wt{\Phi}_r 
\nabla \rchi_\alpha % \begin{pmatrix}
% \partial_1 \rchi_\alpha \\
% \partial_2 \rchi_\alpha
% \end{pmatrix}
{\rm d} x \; + \;
 \frac{1}{r} \int_{\mathbb{R}^2} \nabla \rchi_\alpha \cdot \nabla \wt{\Phi}_r 
\begin{pmatrix}
    x_1 \\
    x_2
\end{pmatrix}  \, {\rm d} x  \nonumber \\
& = \int_{\mathbb{R}^2}   
\frac{\rchi_\alpha^\prime}{\rho} 
\begin{pmatrix}
\cos^2 \theta  \\
\cos \theta \, \sin \theta
\end{pmatrix}
\, \rho \, {\rm d} \rho \, {\rm d} \theta \; + \;
\int_{\mathbb{R}^2}   
\frac{\rchi_\alpha^\prime}{\rho} 
\begin{pmatrix}
\cos^2 \theta \\
\cos \theta \, \sin \theta
\end{pmatrix}
 \, \rho \, {\rm d} \rho \, {\rm d} \theta \nonumber \\
& = 
\begin{pmatrix}
2 \pi \\
0
\end{pmatrix}.
\label{principal bb: new calc avg W r}
\end{align}
In the fourth line, we used the polar coordinate system $(\rho, \theta)$ along with the identities
\begin{align}
\nabla \rchi_\alpha = \begin{pmatrix}
\cos \theta \\
\sin \theta
\end{pmatrix}\, \rchi^\prime_\alpha, %\qquad \partial_2 \rchi_\alpha = \sin \theta \, \rchi^\prime_\alpha,
\qquad
\wt{\Phi}_r = - r \frac{\cos \theta}{\rho}, \qquad \nabla \rchi_{\alpha} \cdot \nabla \wt{\Phi}_r = \partial_{\rho} \rchi_{\alpha} \partial_\rho \wt{\Phi}_r 
= r\frac{\rchi_\alpha^\prime}{\rho^2} \cos \theta.
\end{align}
\end{proof}





\subsection{Compactly Supported Approximate Solution}


In this section, we demonstrate that the compactly supported velocity field $W_r$ constructed in section \ref{subsec:Lamb-Chaplygin} (when translated with speed $r^{-1}$ in the $x_1$ direction) is an approximate solution to the Euler equation. {\color{red} This property enables us to utilize $W_r$ as the principal term of the constant-speed building block. AK: Not clear what this line means.}

In the forthcoming sections, we will work with building blocks traveling with nonconstant speed. To maintain the property of being an almost Euler solution, we must vary their radius in time as well. Thus, the dependence of $W_r$ on the scale parameter $r>0$ will play a central role. A fundamental identity is given by \eqref{principal bb: eqn partial r W_r}, which involves the derivative with respect to $r>0$. {\color{red} AK: generally it is not a good idea to refer to a equation that appears later unless it is an appendix.}





\begin{proposition}[Constant-Speed Building Blocks, Principal Part]
\label{prop:bb constant spead}
Fix $\alpha\in (0,1)$.
Let the velocity field $W_r$ be as defined in (\ref{principal bb: decomposition}). Then there exists pressure fields $P_1, P_2 \in C^{1, 1}(\mathbb{R}^2; \mathbb{R}^2)$ and tensors $F_1, F_2 \in C^{1, 1}(\mathbb{R}^2; \mathbb{R}^{2\times 2})$, such that
\begin{align}
 - \frac{1}{r} \partial_1 W_r + \div (W_r \otimes W_r) + \nabla P_1 = \div(F_1), \label{principal bb: eqn W_r} 
 \\
 \partial_r W_r = \frac{1}{r} W_r + \nabla P_2 + \div(F_2). \qquad \quad
 \label{principal bb: eqn partial r W_r} 
\end{align}
Moreover, the following properties hold:
\begin{enumerate}[label = (\roman*)]
\item 
$\supp P_1, \, \supp P_2, \, \supp F_1, \, \supp F_2 \subseteq B_{9 r^\alpha}(0)$,

\item $\norm{F_1}_{L^{3/2}} \le C r^{2-3\alpha}$ and $\norm{F_2}_{L^{3/2}} \leq C r^{1/3}$.

\item $\norm{\nabla P_2}_{L^\infty} + \norm{\div(F_2)}_{L^\infty} \le C r^{-2}$.
\end{enumerate}
\end{proposition}

\begin{remark}
From (\ref{principal bb: eqn W_r}), it is clear that $W_r(x - t r^{-1} e_1)$ is an approximate solution to the Euler equation.
\end{remark}

\begin{remark}[Space-time smoothing of $W_r$]
\label{rmk:smoothing}
    The velocity field $W_r$, pressure fields $P_1, P_2$, and tensors $F_1$, $F_2$ are almost $C^2$ but not smooth. However, we can smooth them out according to
    \begin{equation}
        W_r \ast \rho_\ell \, ,
        \quad 
        P_1\ast \rho_\ell \, ,
        \quad
        P_2 \ast \rho_\ell \, ,
        \quad
        F_2 \ast \rho_\ell
    \end{equation}
    where $\rho_\ell$ is a smooth convolution kernel supported at scale $\ell$. We then replace $F_1$ with
    \begin{equation}
        F_1 \ast \rho_\ell + (W_r \otimes W_r)\ast \rho_\ell - (W_r\ast \rho_\ell) \otimes (W_r\ast \rho_\ell) \, ,
    \end{equation}
    which is smooth as well.
    If $\ell$ is chosen small enough, then the regularized velocity field, pressure fields, and error tensors will satisfy all the properties in Proposition \ref{prop:bb constant spead}.
\end{remark}




\begin{proof}[Proof of Proposition \ref{prop:bb constant spead}]
We begin by deriving equation (\ref{principal bb: eqn W_r}) and proving the relevant properties of $P_1$ and $F_1$. 
Using (\ref{principal bb: scaled lamb chaplygin eqn}), (\ref{principal bb: req pressure}) and (\ref{principal bb: decomposition}), we discover that $W_r$ satisfies
\begin{equation}
\begin{split}
- \frac{1}{r} \partial_1 W_r - \frac{1}{r} \partial_1 \nabla \Pi + \div(W_r \otimes W_r) + & \div(W_r \otimes \nabla \Pi + \nabla \Pi \otimes W_r) 
\\&+ \div(\nabla \Pi \otimes \nabla \Pi) + \nabla \ol{P}_r = 0 \, .
\end{split}
\label{principal bb: initial eqn Wr}
\end{equation}
Next, we have the following identity:
\begin{align}
\div (\nabla \Pi \otimes \nabla \Pi) = \Delta \Pi \, \nabla \Pi +  \nabla \frac{|\nabla \Pi|^2}{2} \, .
\label{principal bb: a simple identity}
\end{align}
From this, we note that the average of $\Delta \Pi \, \nabla \Pi$ is zero:
\begin{align}
 \int_{\mathbb{R}^2} \Delta  \Pi \, \nabla \Pi \, d x & = \int_{\mathbb{R}^2} \div (\nabla \Pi \otimes \nabla \Pi) \, d x - \int_{\mathbb{R}^2} \nabla \frac{|\nabla \Pi|^2}{2} \, d x \nonumber \\
& = \lim_{R \to \infty} \int_{B_R(0)} \div (\nabla \Pi \otimes \nabla \Pi) \, dx - \lim_{R \to \infty} \int_{B_R(0)} \nabla \frac{|\nabla \Pi|^2}{2} \, d x \nonumber \\
& = \lim_{R \to \infty} \int_{\partial B_R(0)} \nabla \Pi  (\nabla \Pi \cdot n ) \, d s - \lim_{R \to \infty} \int_{\partial B_R(0)}  \frac{|\nabla \Pi|^2}{2} \, n \, d s \nonumber \\
& = 0
\end{align}
We notice that  $\Pi = \wt{\Phi}_r$ when $|x| \geq 2 r^\alpha$.  Using estimates on $\wt{\Phi}_r$ from (\ref{principal bb: estimates on doublet}), we see that $\nabla \Pi \leq C r |x|^{-2}$ for $|x| \geq 2 r^{\alpha}$. This implies that we have good enough decay of integrands in the third line to conclude the last line. Next, using the definition of the pressure $\Pi$ from (\ref{principal bb: req pressure}), we get
\begin{align}
\Delta \Pi \, \nabla \Pi = \left(\Delta \rchi_\alpha \, \wt{\Phi}_r + 2 \nabla \rchi_\alpha \cdot \nabla \wt{\Phi}_r \right) \left(\nabla \rchi_\alpha \wt{\Phi}_r + \rchi_\alpha \nabla \wt{\Phi}_r\right).
\end{align}
From the first term in the parentheses on the right-hand side and the definition of the cutoff function $\rchi_\alpha$, we see that $\supp \Delta \Pi \, \nabla \Pi \subseteq B_{2 r^\alpha}(0) \setminus B_{r^\alpha}(0)$.  Using this fact along with equation (\ref{principal bb: initial eqn Wr}) and identity (\ref{principal bb: a simple identity}), we see that $W_r$ satisfies equation (\ref{principal bb: eqn W_r}) if we define
\begin{align}
P_1 = \ol{P}_r - \frac{\partial_1 \Pi}{r}  + \frac{|\nabla \Pi|^2}{2}, \label{principal bb: def P1} \\
F_1 = W_r \otimes \nabla \Pi + \nabla \Pi \otimes W_r + \mathcal{R}_0(\Delta \Pi \nabla \Pi) \, .
\label{principal bb: def F1}
\end{align}
% The tensor $F_1$ as defined is symmetric. 
When $|x| \geq 2 r^{\alpha}$, we see that $\ol{P}_r = \wt{P}_r$ and $\Pi = \ol{\Phi}_r = \wt{\Phi}_r$. Therefore from (\ref{principal bb: P tilde Phi tilde}) and (\ref{principal bb: def P1}), we see that $P_1 = 0$, when $|x| \geq 2 r^{\alpha}$. Hence, $\supp P_1 \subseteq B_{2 r^\alpha}(0)$. From Proposition \ref{prop:Bogovskii2}, we also see that $\supp A \subseteq B_{9 r^\alpha}(0)$, which after combining with (i) in Lemma \ref{lemma: properties Pi Wr} implies $\supp F_1 \subseteq B_{9 r^\alpha}(0)$.

\bigskip


We now estimate the $L^1$ norm of $F_1$. From (i) in Lemma \ref{lemma: properties Pi Wr}, (\ref{principal bb: estimate Pi nn}), (\ref{principal bb: est 1 Wr})% and (\ref{principal bb: est 2 Wr})
, we see that
\begin{align}
|W_r| \, |\nabla \Pi| \leq C \frac{r^2}{r^{4 \alpha}} \quad \text{when} \quad r^\alpha \leq |x| \leq 2 r^\alpha \qquad \text{and} \qquad |W_r| \, |\nabla \Pi| = 0 \quad \text{otherwise}.
\end{align}
From this, we obtain that 
% {\color{red} add lemma about R0
% \begin{lemma} \label{lemma:inv-div} 
% Let $v\in C^1_c(B_1)$ be a %divergence-free 
% vector field supported in $B_1$ satisfying $\int_{\R^3} v = 0$ and $\int_{\R^3} (x_1 v_2 - x_2 v_1) = 0 $ . Then there exists an % $-1$-pseudo-differential 
% operator $\RR_c$ such that $\RR_c(v) \in C^1_c(\R^3; {\rm Sym}^{2\times 2})$ is compactly supported in $B_1$ and
% \begin{equation}
% \label{eqn:invert-div}
% \div (\RR_c(v)) = v \qquad \mbox{in } \R^3.
% \end{equation}
% Moreover for every $k \in \N$ and $p \in (1,\infty)$  we have the estimate 
% \begin{equation}
% \label{ts:maps-in-W1p}\|\RR_c(v)\|_{W^{k,p}(\R^3)} \leq C \|v\|_{W^{k-1,p}(\R^3)}.
% \end{equation}
% I NEED IT ALSO FOR $k=0$...
% % If moreover $v= \div \tilde R \in C^1_c(B_1)$, where $\tilde R \in C^2(\R^3; {\rm Sym}^{3\times 3})$ is a symmetric matrix  (not necessarily compactly supported in $B_1$) satisfying $\norm{\tilde R}_{L^p_*} < \infty$  for some $p \in (1,\infty)$, then we have 
% % \begin{align}
% % \|\RR_c(\div \tilde R)\|_{L^{p}(\R^3)} &\leq C \norm{\tilde R}_{L^p_*(\R^3)} \label{ts:maps-in-Lp}
% % \end{align}
% % for a universal constant $C>0$.
% %mantain support, give symmetric tensor, scale properly in r
% \end{lemma}\begin{proof}
%     Bogowski operator, but for functions, from Galdi's book
% \end{proof}
% }
\begin{align}
\norm{W_r \otimes \nabla \Pi + \nabla \Pi \otimes W_r}_{L^1} \leq C r^{2 - 2 \alpha}\, .
\label{Principal BB: W_r Pi}
\end{align}
Next, we note that $\supp \Delta \Pi \nabla \Pi \subseteq B_{2 r^\alpha}(0) \setminus B_{r^\alpha}(0)$ and $|\Delta \Pi \nabla \Pi| \leq C \frac{r^2}{r^{5 \alpha}}$, which gives
\begin{align}
\norm{\Delta \Pi \nabla \Pi}_{L^p} \leq C(p) r^{2 - 3\alpha} r^{\alpha(\frac{2}{p}-2)} \, , \quad \text{for every $p\in (1,\infty)$}\, .
\end{align}

From appendix ZZ, we note that $\Delta \Pi \nabla \Pi$ satisfy the condition (\ref{Appendix A: extra cond. for symmetry}). Therefore, an application of Proposition XX along with the compact support of $\Delta \Pi \nabla \Pi$ provides us with the following estimate
\begin{align}
\norm{\mathcal{R}_0 (\Delta \Pi \nabla \Pi)}_{L^1} \leq \norm{\mathcal{R}_0 (\Delta \Pi \nabla \Pi)}_{L^p} \leq C(p) r^\alpha \norm{\Delta \Pi \nabla \Pi}_{L^p} \leq C(p) r^{2 - 2\alpha} r^{\alpha(\frac{2}{p}-2)} \, , \quad \text{for every $p\in (1,\infty)$}\, .
\end{align}


%From Proposition \ref{prop:Bogovskii2}, we deduce
%\begin{align}
%\norm{A}_{L^p} \leq C(p) r^{2 - 2\alpha} r^{\alpha(\frac{2}{p}-2)} \, , \quad \text{for every $p\in (1,\infty)$}\, .
%\end{align}
{ \color{red} AK: Currently half of the $F_1$ error is calculated in $L^1$ (see \ref{Principal BB: W_r Pi}) and final result in mentioned in $L^{3/2}$.}
Therefore, if we choose $p=3/2$, we get the required $L^{3/2}$ estimate on $F_1$.


\bigskip


Now we focus on equation (\ref{principal bb: eqn partial r W_r}). We first observe that
\begin{align}
\partial_r \ol{V}_r 
= 
- \frac{1}{r} \ol{V}_r - \left(\frac{x}{r} \cdot \nabla \right) \ol{V}_r 
= 
\frac{1}{r} \ol{V}_r - \div\left(\ol{V}_r \otimes \frac{x}{r}\right)\, ,
\end{align}
and $\partial_r \wt{\Phi}_r = \partial_r (r \wt{\Phi}) = \frac{1}{r} \wt{\Phi}_r$.
From which we see that
\begin{align}
\partial_r W_r = \frac{1}{r} W_r - \nabla (\wt{\Phi}_r \partial_r \rchi_\alpha) - \div\left(\ol{V}_r \otimes \frac{x}{r}\right). 
\label{principal bb: partial r Wr inter 1}
\end{align}
From
\begin{align}
\partial_r W_r = \partial_r \left( r \frac{W_r}{r} \right) = \frac{W_r}{r} + r \partial_r \frac{W_r}{r},
\end{align}
we see that for any $R > 2 r^{\alpha}$, we have
\begin{align}
\int_{B_R(0)} \partial_r W_r \, {\rm d} x = \frac{1}{r} \int_{B_R(0)} W_r \, {\rm d} x \,  + r \partial_r \left(\frac{1}{r} \int_{B_R(0)} W_r \, {\rm d} x\right)\, = \frac{1}{r} \int_{B_R(0)} W_r \, {\rm d} x.
\end{align}
In particular, we get
\begin{align}
\int_{\mathbb{R}^2} \partial_r W_r \, {\rm d} x  = \frac{1}{r} \int_{\mathbb{R}^2} W_r \, {\rm d} x.
\end{align}
Using this information in  (\ref{principal bb: partial r Wr inter 1}) and noting that $\supp \partial_r \rchi_\alpha \subseteq \ol{B}_{2 r^\alpha}(0)$, we obtain 
\begin{align}
\int_{\mathbb{R}^2} \div\left(\ol{V}_r \otimes \frac{x}{r}\right) \, {\rm d} x = 0.   
\label{principal bb: div Vr x inf 1}
\end{align}
We also note that when $|x| \geq r$, we have $\ol{V}_r = \wt{V}_r$ which combined with lemma \ref{lemma: div tensor V x} leads to
\begin{align}
\supp \div\left(\ol{V}_r \otimes \frac{x}{r}\right) \, \subseteq \, B_r(0). 
\label{principal bb: div Vr x inf 2}
\end{align}
Moreover, from (\ref{principal bb: estimate on Vbar}) we get
\begin{align}
\norm{\div\left(\ol{V}_r \otimes \frac{x}{r}\right)}_{L^\infty} \le C \frac{1}{r^2}\, .
\end{align}
Hence, for every $p\in [1,\infty]$ we get
\begin{equation}
    \norm{\div\left(\ol{V}_r \otimes \frac{x}{r}\right)}_{L^p}
    \le C r^{\frac{2}{p} - 2}\, .
    \label{principal bb: div Vr x inf 3}
\end{equation}
Thanks to Proposition \ref{prop:Bogovskii2}, there exists a tensor $F_2$ supported on $B_r(0)$, such that $\div(F_2) = -\div\left(\ol{V}_r \otimes \frac{x}{r}\right)$ and 
\begin{equation}
    \| F_2 \|%_{L^1} \le \| F \|
    _{L^p} \le C(p) r \|\div\left(\ol{V}_r \otimes \frac{x}{r}\right)\|_{L^p}
    \le C(p) r^{\frac{2}{p} - 1}
\end{equation}
%{\color{red} AK: F is not introduced, $F_2$ maybe}
for every $p\in (1,\infty)$. So, for $p=3/2$ we have $\| F_2 \|_{L^1} \le C r^{1/3}$.
In conclusion, $W_r$ and $F_2$ satisfy (\ref{principal bb: eqn partial r W_r}) with $P_2 = - \wt{\Phi}_r \partial_r \rchi_\alpha$.
% \begin{align}
% P_2 = - \wt{\Phi}_r \partial_r \rchi_\alpha \, .
% \end{align}
% Finally, noting (\ref{principal bb: div Vr x inf 1}), (\ref{principal bb: div Vr x inf 2}) and (\ref{principal bb: div Vr x inf 3}) and using Lemma YY the estimate on $F_2$ is
% \begin{align}
% \norm{F_2}_{L^1} \leq C r^{1 - \varepsilon}.
% \end{align}
\end{proof}










\subsubsection{Building Block with Non-constant Speed}
\label{sec:BB nonconstant speed}





Let $r: \mathbb{T}^2 \to (0,\infty)$ be a smooth positive function satisfying $\| r \|_{L_x^\infty} < \frac{1}{9}$. It should be considered as a space-dependent spatial scale. In the following sections, we will adjust $r(x)$ in relation to the Reynolds stress tensor in \eqref{eq:ER}.

We also consider a smooth function $\eta: \mathbb{R} \to [0,\infty)$. It should be understood as a time-dependent cut-off function.  It will be used to keep our family of building blocks disjoint in time.





\bigskip



Next, we define the trajectory of the center of our building block. We want it to travel on a linear periodic trajectory in the two-dimensional torus. More precisely, given any unit vector $\xi\in \mathbb{R}^2$ with rationally dependent components, the center of mass
$x: \R \to \mathbb{T}^2$ will solve the ODE
\begin{align}\label{eq:ODE}
\begin{cases}
    x'(t) = \frac{\eta(t)}{r(x(t))} \xi,
    \\
    x(0) = x_0 \, ,
\end{cases}
\end{align}
In the sequel, the time-period of the linear trajectory $t\to t \xi$ will play the role of the frequency parameter $\lambda_{q+1}$ in classical convex integration schemes. To obtain this, the trajectory realizes a $1/\lambda_{q+1}$-dense set on the torus. 

{\color{blue}Maria: Add a picture with the trajectory, the ball moving.}

\bigskip

The velocity field in \eqref{eq:ODE} depends on the inverse of the space-dependent scale $r(x)$ so that the building block will spend more time in locations where the scale is large and leave quickly from locations where the scale is small. This will be key in our new mechanism of error cancellation. The function $\eta(t)$ in \eqref{eq:ODE} mainly serves as a time cut-off.




\bigskip




The principal building block is given by
\begin{align}\label{eq:V^p after W}
V^p(x,t) = \eta(t) \, W_{r(x(t))}(x - x(t)).
\end{align}
where $W_r\in C^\infty$ is  smoothed according to Remark \ref{rmk:smoothing} {\color{blue} and with $\alpha=1/4$ - keep track explicitly of bounds on alpha}, and rotated so that it solves
\begin{align}\label{eq:Wxi}
 - \frac{1}{r} (\xi \cdot \nabla) W_r + \div (W_r \otimes W_r) + \nabla P_1 = \div(F_1) \, ,  
 \\
 \partial_r W_r = \frac{1}{r} W_r + \nabla P_2 + \div(F_2) \, , 
 \quad \text{on $\R^2$} \, .
\end{align}
As they are compactly supported, we consider the one-periodized version of $W_r$, $P_1$, $P_2$, and $F_1$, $F_2$, and associate them with functions on the $2$-dimensional torus $\mathbb{T}^2$. Finally, we correct the divergence of $V^p$ by adding a corrector
\begin{equation}\label{eq:V}
    \begin{split}
         &V(x,t) := V^p(x,t) + V^c(x,t)
         \\
         & V^c(x,t) := - \nabla \Delta^{-1} \div V^p(x,t) \, ,
         \quad \text{on $\mathbb{T}^2$.}
    \end{split}
\end{equation}
Let us stress that $V^c\in C^\infty$ is defined on $\mathbb{T}^2$, and it is not compactly supported. 





\bigskip


In the following proposition, we use the shorthand notations $r(t) \coloneq r(x(t))$. 








\begin{proposition}[Building Block]\label{prop:build-block1}
Let $V$ be as in \eqref{eq:V}.
There exists $S \in C^\infty (\mathbb{T}^2 \times \R; \mathbb{R}^2)$, $P\in C^\infty ( \mathbb{T}^2 \times \R; \mathbb{R})$, and a symmetric tensor $F\in C^\infty(\mathbb{T}^2 \times \R; \mathbb{R}^{2\times 2})$ such that
\begin{equation}\label{eq:EulerV}
\begin{cases}
\partial_t V + \div(V\otimes V) + \nabla P 
=  S \frac{d}{dt} \left(\eta(t) \, r(t)\right)   +  \div(F) \, ,
\\
\div(V)  = 0\, ,
\end{cases}
\quad\quad \text{on $\mathbb{T}^2\times \R_+$}
\end{equation}
Moreover, the following estimates hold:
\begin{enumerate}[label = (\roman*)]
\item $\| F \|_{L^\infty_t L^{3/2}_x} \le C \| \eta \|_{L^\infty}^2 \| r \|_{L^\infty}^{1/3}(1 + \| \nabla \log(r)\|_{L^\infty_x})$.


% (Estimate on the Raynold stress tensor $F$)
% \begin{equation}
% \norm{F}_{L_t^\infty L_x^1} 
% \le C (\norm{\eta}_{L_t^\infty}^2 \norm{\nabla r}_{L_x^\infty} + \norm{\eta}_{L_t^{\infty}} \norm{r}_{L_x^\infty} )
% \end{equation}


\item For every $p\in (1,\infty)$, it holds
\begin{align}
& { \color{red}  \| V \|_{L^\infty_t L^p_x} 
        +  \| r \|_{L^\infty_x} \| D V \|_{L^\infty_t L^p_x}
        \le C(p) \| \eta \|_{L^\infty_t } \| r \|_{L^\infty_x}^{\frac{2}{p} - 1} \, ,}
        \\
& {\color{red} \text{Can not multiply $r$ in L infinity with DV if the power is negative.} } \\
        &\| \partial_t V \|_{L^1_t L^p_x}  \le C(p) \norm{\eta^2}_{L^\infty_t} \norm{r^{-3}}_{L^\infty_x}(1 + \| \nabla \log (r)\|_{L^\infty_x}) + C(p)  \norm{\eta'}_{L^\infty_t} \norm{r^{-1}}_{L^\infty_x} \, ,
        \\
        & \| S(\cdot, t) \|_{L_x^p}
    \le C(p)  \, r(t)^{\frac{2}{p}-2}\, .
\end{align}
{\color{red} AK: to obtain estimate on $DV$ you need estimate $DV^p$ or $D W_r$ which is not there in Lemma \ref{lemma: properties Pi Wr}. }


% \item (Estimates on $V$) 
% \begin{align}
% &\| V(\cdot, t) \|_{L_x^1} 
% \leq C 
% \, \eta(t)\, r(t) \, |\log r(t)|, 
% \quad 
% \| V(\cdot, t) \|_{L_x^p} 
% \leq C(p) \, \eta(t) \, r(t)^{\frac{2}{p}-1} \quad
% \text{ for } p \in (1, \infty],
% \\
% & \|\nabla \times V(\cdot, t) \|_{L_x^p} \le C(p) \, \eta(t) \, r(t)^{\frac{2}{p}-2}
% \quad
% \text{ for } p \in [1, \infty],
% \\
% & \| V \|_{C^1_{x,t}} \le C (\eta(t)r(t)^{-2} + \eta^\prime(t)r(t)^{-1})
% \end{align}


% \item (Estimate on the source term $S$)
% \begin{align}
%      \| S(\cdot, t) \|_{L_x^p}
%     \le C(p)  \, r(t)^{\frac{2}{p}-2}\, ,
%     \quad 
%     \quad
% \text{ for } p \in [1, \infty],
% \end{align}

% \begin{align}
% \supp S(\cdot, t) \subseteq B_{r(t)}(x(t)), \qquad   \int_{\mathbb{T}^2} S(x,t)\, {\rm d} x =  \xi .
% \end{align}




\item For every $t\in \R_+$,  $S(\cdot, t)$ is supported on $B_{r(t)}(x(t))$, and 
\begin{align}
  \int_{\mathbb{T}^2} S(x,t)\, {\rm d} x =  2\pi \xi .
\end{align}
{\color{red} The support of $S$ is not $r(t)$.}

\end{enumerate}
\end{proposition}


The major difference between \eqref{eq:EulerV} and \eqref{principal bb: eqn W_r} is the presence of the source term $ \left(\eta \, r\right)' S$ produced by the non-constant speed of $V$ and the cut-off function $\eta$. We will take advantage of this source term to cancel the error in the iteration scheme. 






\begin{proof}
From \eqref{eq:Wxi}, we have
\begin{align}
\partial_t V + \div(V \otimes V) &= \partial_t V^p + \partial_t V^c + \div (V^p \otimes V^p) 
\\&+ \div (V^p \otimes V^c + V^c \otimes V^p) + \div (V^c \otimes V^c) \, ,
\end{align}
then, by using once more \eqref{eq:Wxi}, we obtain
\begin{align}
\partial_t V^p(x,t) & = \partial_t (\eta(t) W_{r(x(t))}(x - x(t))) 
\\& 
= - \frac{\eta^2}{r} (\xi \cdot \nabla) W_{r} + \eta r^\prime \partial_r W_r  + \eta^\prime W_r \nonumber 
\\&
= - \frac{\eta^2}{r} (\xi \cdot \nabla) W_r + \eta r^\prime \left(\frac{1}{r} W_r + \nabla P_2 + \div (F_2) \right)  + \eta^\prime W_r \nonumber 
\\&
= - \frac{\eta^2}{r} (\xi \cdot \nabla) W_r  + (\eta r)^\prime \frac{1}{r}W_r + \nabla (\eta r^\prime P_2) + \div (\eta r^\prime F_2) \, .
\end{align}
Since,
\begin{align}
\div(V_p \otimes V_p) &= \eta^2 \div(W_r \otimes W_r) 
\\
\partial_t V^c & = - \nabla \partial_t \Delta^{-1} \div V^p
\end{align}
% which gives
% \begin{align}
% \partial_t V^p + \div(V_p \otimes V_p) = \eta^2 \left(- \frac{1}{r} \xi \cdot \nabla W_r + \div(W_r \otimes W_r) \right) + (\eta r)^\prime \frac{1}{r}W_r + \nabla (\eta r^\prime P_2) + \div (\eta r^\prime F_2) \nonumber \\ 
% = \eta^2 \left( - \nabla P_1 + \div F_1 \right) + (\eta r)^\prime \frac{1}{r}W_r + \nabla (\eta r^\prime P_2) + \div (\eta r^\prime F_2)
% \end{align}
% We also note 
% \begin{align}
% \partial_t V^c = - \nabla \partial_t \Delta^{-1} \div V^p
% \end{align}
we conclude that
\begin{align}
\partial_t V + \div(V \otimes V) +\nabla P 
=
S \frac{d}{dt} \left(\eta(t) r(t) \right) + \div (F)
\end{align}
where
\begin{align}
P &= \partial_t \Delta^{-1} \div V^p + \eta^2 P_1 - \eta r^\prime P_2 
\\
F & = \eta^2 F_1 + \eta r^\prime F_2 + V^p \otimes V^c + V^c \otimes V^p + V^c \otimes V^c 
\\
S & = \frac{1}{r} W_r \, .
\end{align}
Notice that, as defined, $F$ might be not symmetric. To solve this issue, we replace $\eta^2 F_1 + \eta r' F_2$ with 
\begin{equation}
    F_3:= \mathcal{R}_0 \div(\eta^2 F_1 + \eta r' F_2) \, .
\end{equation}
{ \color{red} AK: this is not true. You need to ensure condition (\ref{Appendix A: extra cond. for symmetry}). Therefore, I reverted back to make $F_1$ and $F_2$ symmetric.} \\
{\color{blue}EB: Why it is not true? Condition (\ref{Appendix A: extra cond. for symmetry} does not even make sense on the torus (it is necessary on $\R^2$). The opeator $\mathcal{R}_0$ is well-defined and symmetric on the torus.} \\
{\color{red} AK: the condition (\ref{Appendix A: extra cond. for symmetry}) is needed at some place. Currently, there is no reference. How this is used? Also, how the tensor $A$ is symmetric once (\ref{Appendix A: extra cond. for symmetry}), the detail is missing. If the condition (\ref{Appendix A: extra cond. for symmetry}) is not needed then it can be removed.
}



{ \color{red} AK: this is not true for a general $\eta$. I have reverted back to the previous below. \\
By construction (see \eqref{eq:R0}) $F_3$ is symmetric, and  $\div(F_3)=\div(\eta^2 F_1 + \eta r' F_2)$. Moreover, for every $p\in (1,\infty)$ we have
\begin{equation}
    \| F_3\|_{L^\infty_tL^p_x}
    \le C(p) \|\eta^2 F_1 + \eta r' F_2\|_{L^p}
    \le C(p) \| \eta \|_{L^\infty_t}^2( \| F_1 \|_{L^p} + \| \nabla \log(r)\|_{L^\infty_x} \| F_2 \|_{L^p})
\end{equation}
}
\begin{align}
    \| F_3\|_{L^\infty_tL^p_x}
    \le C(p) \|\eta^2 F_1 + \eta r' F_2\|_{L^p}
    \le C(p) (\| \eta \|_{L^\infty_t}^2 + \norm{\eta}_{L^\infty_t})( \| F_1 \|_{L^p} + \| \nabla \log(r)\|_{L^\infty_x} \| F_2 \|_{L^p})
\end{align}

as a consequence of \eqref{eq:R0est2}. By Proposition \ref{prop:bb constant spead} (ii) with { \color{red} $\alpha\in (0,6/5)$}, we conclude that
\begin{equation}
    \| F_3 \|_{L^\infty_t L^{3/2}_x} \le C (\| \eta \|_{L^\infty_t}^2 + \norm{\eta}_{L^\infty_t}) \| r \|_{L^\infty}^{1/3}(1 + \| \nabla \log(r)\|_{L^\infty_x})\, .
\end{equation}



\bigskip

From the classical Calderon-Zygmund theory, we have
\begin{equation}
\begin{split}
     \| V^c(\cdot, t) \|_{L^p} &\le C(p) \|\eta \|_{L^\infty_t} \| W_{r(t)} \|_{L^p}
     \\
     \| D V^c(\cdot, t)\|_{L^p}
     & \le C(p)\|\eta \|_{L^\infty_t} \| \div W_{r(t)}\|_{L^p} \, ,
     \quad
     \text{for every $p\in (1,\infty)$} \, .
\end{split}
\end{equation}
Since $\|\div W_r \|_{L^\infty} \le C r^{1/3}$ for $\alpha\in (0,2/9)$, we deduce that
\begin{equation}
    \| V^c \|_{L^p}
    \le
    \| D V^c \|_{L^\infty_t L^p_x} \le C(p) \|\eta \|_{L^\infty_t}\| r \|_{L^\infty_x}^{1/3} \, ,
    \quad \text{for every $p\in (1,\infty)$} \, ,
\end{equation}
where in the first estimate we used the Poincarè ({\color{red} accent is wrong}) inequality.
In particular, we can bound 
\begin{align}\label{z12}
\norm{V^p \otimes V^c + V^c \otimes V^p + V^c \otimes V^c}_{L^\infty_tL^{p/2}_x} 
&\leq 2 \norm{V^p}_{L^\infty_t L^2_x} \norm{V^c}_{L^\infty_t L^p_x} + \| V^c \|_{L^\infty_t L^p_x}^2
\\&
\leq C(p) \|\eta\|_{L^\infty_t}^2 \| r \|_{L^\infty_x}^{1/3}\, ,
\end{align}
for every $p\in (1,\infty)$. In \eqref{z12} we used the estimate
\begin{equation}
    \| V^p \|_{L^\infty_t L^p_x} 
    \le \| \eta W_r \|_{L^p}
    \le C(p) \|\eta\|_{L^\infty_t} \| r \|_{L^\infty_x}^{\frac{2}{p} - 2} \, , \quad \text{for every $p\in (1,\infty)$} \, ,
\end{equation}
with $p=2$. ({\color{red} AK: If the estimate with $p = 2$ is used should that reflect in (2.81)})


\bigskip

We finally estimate $\partial_t V$ and $D V$ in $L^p$.
We begin by noticing that
\begin{equation}
    \| D_{x,t} V^c \|_{L^\infty_t L^p_x} \le C(p) \| D_{x,t} V^p\|_{L^\infty_t L^p_x} \, ,
    \quad \text{for every $p\in (1,\infty)$}
\end{equation}
by Calderon-Zygmund theory, since $V^c= - \nabla \Delta^{-1}\div(V^p)$. Hence, it will be enough to estimate $D_{x,t} V^p$. From Lemma \ref{lemma: properties Pi Wr}, {\color{blue} it is immediate} to bound the bound the space derivative:
\begin{equation}
    \| D V^p(\cdot, t) \|_{L^p_{x}}
    \le 
    \eta \| W_r \|_{L^p_{x}}
    \le C \eta r^{\frac{2}{p}-2} \, .
\end{equation}
To bound the time derivative, we restart from the identity
\begin{align}
\partial_t V^p =
- \frac{\eta^2}{r} (\xi \cdot \nabla) W_r  + (\eta r)^\prime \frac{1}{r}W_r + \nabla (\eta r^\prime P_2) + \div (\eta r^\prime F_2) \, ,
\end{align}
which implies
\begin{equation}
    \begin{split}
        \| \partial_t V^p(\cdot, t)\|_{L^\infty_x} 
        & \le \frac{\eta^2}{r} \| D W_r \|_{L^\infty_x} 
        +|\eta'| \| W_r \|_{L^\infty}
        \\&
        + \eta |r'| \left(\frac{1}{r}\| W_r \|_{L^\infty_x} + \|\nabla P_2 \|_{L^\infty_x}
        + \| \div (F_2) \|_{L^\infty_x}\right)
        \\&
        \le C\eta^2 r^{-3} + C|\eta'|r^{-1} + C\eta |r'| r^{-2} \, ,
    \end{split}
\end{equation}
({\color{red} AK: Estimate on $\norm{D W_r}_{L^\infty_x}
$}) where we used Lemma \ref{lemma: div tensor V x} and Proposition \ref{lemma: properties Pi Wr} (iii).

\bigskip \bigskip

% Let the Sobolev exponent $p^\ast$ be defined through
% \begin{align}
% \frac{1}{p} - \frac{1}{p^\ast} = \frac{1}{2}.
% \end{align}
% From the classical CZ theory we have the following estimate
% \begin{align}
% \norm{V^c}_{L^{p^\ast}}  \leq C(p) \eta(t) \norm{ \div W_{r(t)} }_{L^p} \qquad \text{ for any } p \in (1, \infty),
% \end{align}
% which means
% \begin{align}
% \norm{V^c}_{L^{p^\ast}}  \leq C(p) \eta(t) r(t)^{1 - \alpha} r(t)^{\alpha \left(\frac{2}{p} - 2\right)} \qquad \text{ for any } p \in (1, \infty).
% \end{align}
% We also have
% \begin{align}
% \norm{V^c}_{L^{p}}  \leq C(p) \eta(t) \norm{ W_{r(t)} }_{L^p} \qquad \text{ for any } p \in (1, \infty],
% \end{align}
% which implies
% \begin{align}
% \norm{V^c}_{L^{p}}  \leq C(p) \eta(t) \norm{ W_{r(t)} }_{L^p} \leq C(p) \eta(t) r(t)^{\frac{2}{p} - 1} \text{ for any } p \in (1, \infty].
% \end{align}

% Let's quickly calculate bounds on the error, we start by noticing
% \begin{align}
% \norm{V^c}_{L^{2}}  \leq C(\varepsilon) \eta(t) r(t)^{1 - \alpha - \varepsilon}.
% \end{align}
% Therefore, we get
% \begin{align}
% \norm{V^p \otimes V^c + V^c \otimes V^p}_{L^1} \leq 2 \norm{V^p}_{L^2} \norm{V^c}_{L^2} \leq C(\varepsilon) \eta^2(t) r(t)^{1 - \alpha - \varepsilon}.
% \end{align}
% Similarly,
% \begin{align}
% \norm{V^c \otimes V^c}_{L^1} \leq \norm{V^c}_{L^2} \norm{V^c}_{L^2} \leq C(\varepsilon) \eta^2(t) r(t)^{2 - 2 \alpha - 2 \varepsilon}.
% \end{align}
% More
% \begin{align}
% \norm{\eta^2 F_1}_{L^1} \leq \eta^2(t) r(t)^{2 - 2 \alpha - 2 \varepsilon}
% \end{align}
% We also note that
% \begin{align}
% r^\prime = (\xi \cdot \nabla r) \frac{\eta}{r}
% \end{align}
% which gives
% \begin{align}
% \norm{\eta r^\prime F_2}_{L^1} \leq | \nabla r| \frac{\eta^2}{r^\varepsilon}.
% \end{align}
% Estimate on 
% \begin{align}
% \norm{V}_{L^p} \text{ for } p > 1 \text{ is right away}.
% \end{align}
% Same applies for the curl.

% From the classical CZ theory and Morrey embedding theorem, we get
% \begin{align}
% \norm{\nabla V^c}_{C^0} \leq C \norm{\nabla^2 V^c}_{L^p} \leq C \norm{\div \nabla V^p}_{L^p} \leq C \eta \norm{\div \nabla W_r}_{L^p} \leq C \eta r^{1 - 2\alpha - \varepsilon} \quad \text{ for any } p > 2.
% \end{align}
% We also have
% \begin{align}
% \norm{\nabla V^p}_{L^\infty} \leq C \eta \norm{\nabla W_r}_{L^\infty} \leq C \frac{\eta}{r^2}
% \end{align}
% Now we estimates the time derivative. We again start by noticing
% \begin{align}
% \partial_t V^p = - \frac{\eta^2}{r} \xi \cdot \nabla W_r  + (\eta r)^\prime \frac{1}{r}W_r + \nabla (\eta r^\prime P_2) + \div (\eta r^\prime F_2)
% \end{align}






\end{proof}





\section{Iteration}
In this section, we set up the iteration of our convex integration scheme. We begin by introducing the relations between parameters. 

\begin{equation}\label{eq:parameters}
    \lambda_{q+1} = \lambda_q^{\sigma} \, ,
    \quad 
    \delta_q = \lambda_q^{-\beta} \, ,
    \quad
    r_{q+1} = \lambda_{q+1}^{-\mu} \, .
\end{equation}
At the $q$th step of the iteration, we construct solutions to the Reynolds-Euler system
\begin{equation}\label{eq:ER}
    \begin{cases}
        \partial_t u_q + \div(u_q \otimes u_q) + \nabla p_q = \div(R_q)
        \\
        \div u_q = 0 \, ,
    \end{cases}
\end{equation}
satisfying estimates:
\begin{equation}\label{eq:iterate1}
    \| R_q \|_{L^\infty_t L^1_x} \le \delta_{q+1} \, ,
    \quad
    \| D_{x,t} u_q \|_{L^\infty_t L^4_x} \le \lambda^N_q \, .
\end{equation}
 



\begin{proposition}[Iteration Step]\label{prop:iteration}
    There exists $p>1$, and parameters $\lambda_0>1$, $\sigma>1$, $\beta>0$, $\mu>0$, $N>0$, such that the following holds.
    Let $(u_q,p_q,R_q)$ be a smooth solution to \eqref{eq:ER} satisfying \eqref{eq:iterate1}. Then, there exists $(u_{q+1}, p_{q+1}, R_{q+1})$ solution to \eqref{eq:ER} such that
    \begin{itemize}
        \item[(i)] $\| R_{q+1} \|_{L^\infty_t L^1_x} \le \delta_{q+2}$,  
        and
        $\| D_{x,t} u_{q+1} \|_{L^\infty_t L^4_x} \le \lambda^N_{q+1}$,
        
        \item[(ii)] $\|u_{q+1}\|_{L^\infty_tL^2_x} \le \| u_q\|_{L^\infty_t L^2_x} + \delta_{q+1}^{1/5}$, and
        $\| D u_{q+1}\|_{L^\infty_t L^p_x}\le \| D u_q \|_{L^\infty_t L^p_x}
        + \delta_{q+1}^{1/5}$.
        
        
        
       
    \end{itemize}
\end{proposition}








\subsection{Convolution Step}
Let $\ell >0$ be a scale parameter that will be chosen later. We define 
\begin{equation}
    u_\ell = u_q \ast \rho_\ell \, ,
    \quad
    p_\ell = p_q \ast \rho_\ell\, ,
    \quad
    R_\ell = R_q \ast \rho_\ell + u_\ell \otimes u_\ell - (u\otimes u)\ast \rho_\ell \, ,
\end{equation}
where $\rho_\ell$ is a smooth mollifier in space and time, at length scale $\ell$.
It is immediate to check that $(u_\ell, p_\ell, R_\ell)$ solves the Euler-Reynold equation
\begin{equation}
    \partial_t u_\ell + \div(u_\ell \otimes u_\ell) + \nabla p_\ell = \div(R_\ell) \, .
\end{equation}
By Sobolev embedding we have
\begin{equation}\label{eq:u_q Sob}
    \| u_q \|_{C^{1/4}_{x,t}} \le C\|D_{x,t} u_q \|_{L^\infty_t L^4_x}
    \le C\lambda_q^N \, ,
\end{equation}
hence we can estimate 
\begin{equation}
    \begin{split}
        \| R_\ell \|_{L^\infty_t L^1_x} 
        &\le \| R_q \ast \rho_\ell \|_{L^\infty_t L^1_x} + \|u_\ell \otimes u_\ell - (u\otimes u)\ast \rho_\ell\|_{L^\infty_t L^1_x}
        \\&
        \le \delta_{q+1} + \ell^{1/4} \| u_q \|_{C^{1/4}_{x,t}} \| u_q \|_{L^\infty_{x,t}}
        \\& 
        \le \delta_{q+1}  + \ell^{1/4} \lambda_q^{2N}\, .
    \end{split}
\end{equation}
So, we can choose $\ell^{1/4} = \delta_{q+1}\lambda_q^{-2N}$ in order to get
\begin{equation}
    \| R_\ell \|_{L^\infty_t L^1_x} \le 2 \delta_{q+1}\, .
\end{equation}







\subsection{Error Decomposition}
Fix $\lambda_{q+1}\gg 1$. There exist $\xi_1, \xi_2, \xi_3, \xi_4$ unitary vectors of $\R^2$ with rationally dependent components satisfying the following properties.

\begin{itemize}
    \item[(i)] There exists $c_i\in [1,2]$ such that the time period of the curve $s \to s\xi_i$ in $\mathbb{T}^2$ is $c_i \lambda_{q+1}$.


    \item[(ii)] The following decomposition holds:
    \begin{align}\label{eq:error dec}
     - \div(R_\ell) = \div\left(\sum_{i=1}^4 a_i(x,t) \xi_i \otimes \xi_i\right) + \nabla P \, ,
     \end{align}
     where $a_i(x,t)$ are smooth functions satisfying
     \begin{equation}\label{eq:est_a}
         a_i(x,t) \ge \delta_{q+1} \, ,
         \quad 
         \| a_i \|_{L^\infty_t L^1_x} \le 10 \delta_{q+1} \, ,
         \quad
         \| a_i \|_{C^1_{x,t}}
         \le  \delta_{q+1}^{-11}\lambda_q^{24 N}\, .
     \end{equation}
     \end{itemize}


{\color{blue}[ADD A PROOF]}



\subsection{Time Series}

We introduce a small time scale $0 < \tau_{q+1} <1$, which will be expressed later as a negative power of $\lambda_{q+1}$. We partition $[0,+\infty)$ into time intervals $\mathcal{T}^k = [k\tau_{q+1}, (k+1)\tau_{q+1})$ of length $\tau_{q+1}$. Each of them will be divided further into four according to
\begin{equation}
    \mathcal{T}^k_i = \left[\tau_{q+1} \big(k +\frac{i-1}{4}\big),\, \tau_{q+1} \big(k+ \frac{i}{4}\big)\right) \, ,
    \quad i=1, 2, 3, 4\, , \quad  k\in \N \, .
\end{equation}
Notice that $\mathcal{T}^k= \bigcup_{i=1}^4 \mathcal{T}^k_i$.


\bigskip


Given a time-dependent function $g: \R_+ \to \R$, we introduce the time-average operator
\begin{equation}\label{eq:Ptau}
    P_{\tau}g(t) := \dashint_{\mathcal{T}^k} g(s)\, ds \, , \quad \quad t\in \mathcal{T}^k \, ,
\end{equation}
tailored for our time series.


\bigskip


We approximate the error $R_\ell$ with a constant-in-time tensor within each interval $\mathcal{T}^k$. To achieve this, we set
\begin{equation}
    a_i^k(x):= P_\tau a_i(x,t)
    =
    \dashint_{\mathcal{T}^k} a_i(x,t)\, dt \, ,
    \quad \text{for $t\in \mathcal{T}^k$}\, .
\end{equation}
Notice that
\begin{equation}\label{eq:a-aik}
    \| P_\tau a_i - a_i\|_{L^\infty_t L^1_x} 
    \le \tau_{q+1} 
    \| a_i \|_{C^1_{x,t}}
    \le \tau_{q+1} \delta_{q+1}^{-11}\lambda_q^{24N}\, ,
    \quad \text{ for every $t\in \mathcal{T}_i^k$} \, ,
\end{equation}
is going to be small provided $\tau_{q+1}$ is sufficiently small.




\subsection{Space-variable Scale}

The building blocks constructed in Proposition \ref{prop:build-block1} depend on a space-variable scale $r(x)$ and time cut-off $\eta(t)$. Both will depend on the indices $i,k$ referring to the time interval $\mathcal{T}_i^k$.


\bigskip

Fix $r_{q+1} \in (0,1)$ small enough so that 
\begin{equation}
    r_{q+1}^{1/2} \max_{i,k} \| a_i^k\|_{L^\infty} 
    \le 1 \, .
\end{equation}
We will express later $r_{q+1}$ as a negative power of $\lambda_{q+1}$. We define the space-dependent time scale as
\begin{equation}
    r^k_i(x) = r_{q+1} a^k_i(x) \, ,
    \quad i=1, 2, 3, 4\, , \quad k\in \N \, .
\end{equation}
Notice that, by construction
\begin{equation}
    r_i^k \ge r_{q+1} \delta_{q+1}\, ,
    \quad 
    \quad 
    \norm{ r_k^i }_{L^\infty} \le r_{q+1}^{1/2}(r_{q+1} \| a_i^k \|_{L^\infty}^2)^{1/2} 
    \le r_{q+1}^{1/2} \, .
\end{equation}




\subsection{Time cut-off}
Given $i\in \{1,2,3,4\}$ and $k\in \N$, we define a cut-off function $0 \le \zeta_i^k \le 1$ compactly supported in $\mathcal{T}_i^k$ satisfying the following properties:


\begin{itemize}
    \item[(i)] $\zeta_i^k(t) = 1$ for every $t$ whose distance from the end-points of $\mathcal{T}_i^k$ is bigger than $\tau_{q+1}/\lambda_{q+1}$.


    \item[(ii)] Bounds on the derivative:
    \begin{equation}
        \norm{\frac{d}{dt}\zeta_i^k}_{L^\infty} \le 10 \lambda_{q+1}^{-1}
    \end{equation}

\end{itemize}




\subsection{Trajectory of the Center}\label{sub:traj cent}

For each $k\in \N$ and $i=1,2,3,4$, we will construct a building block $V_i^k$ as in Proposition \ref{prop:build-block1} with scale function $r_i^k(x)$, and time cut-off $\eta(t) = \eta_i^k \zeta_i^k(t)$, where $\eta_i^k >0$ is given by 
\begin{equation}\label{eqn:choiceetamagic}
    (\eta_i^k )^2 =  4 \int_{\mathbb{T}^2}a_i^k(x) \, dx
    \in [4 \delta_{q+1}, 40 \delta_{q+1}]\, ,
\end{equation}
where the inclusion follows from \eqref{eq:est_a}.
This particular choice of $\eta_i^k$ is crucial to get the exact error cancellation and {\color{red} can be interpreted in two ways at this stage: we observe that it is natural under the simplifying assumption that the coefficient $a_i^k(x)$ is constant; on the other side, the reader may decide to leave it as a free parameter depending on $i$ and $k$ along this construction, and optimize it at the end of the proof of Proposition~\ref{prop:auxiliary}, finding back \eqref{eqn:choiceetamagic}. AK: this sentence does not make any sense}

\bigskip

The corresponding center of mass of the building block $V_i^k$ will be moving according to
\begin{equation}\label{eq:traj1}
        \frac{d}{dt} x^k_i(t) = \frac{ \eta_i^k \zeta_i^k(t)}{r_i^k(x^k_i(t))} \xi_i \, , \quad \quad
        \quad t \in \mathcal{T}_i^k \, .
\end{equation}
Let us denote $t_0 = \tau_{q+1}(k + \frac{i-1}{4} + \lambda_{q+1}^{-1})$. We fix $x_i^k(t_0)$ so that
\begin{equation}
    \dashint_0^{c_i\lambda_{q+1}} a_i^k(x_i^k(t_0) + s \xi_i) \, ds = \int_{\mathbb{T}^2}a_i^k(x)\, dx \, ,
\end{equation}
and we assume $\lambda_{q+1}^2 r_{q+1} \delta_{q+1}^{1/2} \le \frac{\tau_{q+1}}{100}$, so that 
\begin{equation}\label{eq:imp}
    \frac{c_i\lambda_{q+1} r_{q+1}}{\eta_i^k} \int_{\mathbb{T}^2}a_i^k(x)\, dx \le    {c_i\lambda_{q+1} r_{q+1}}\delta_{q+1}^{1/2} \le \frac{\tau_{q+1}}{10 \lambda_{q+1}}
\end{equation}
These two conditions imply that there exists $M_i^k\in \N$, $M_i^k \ge \lambda_{q+1}$ such that 
\begin{itemize}
    \item[(i)] $x_i^k(t_0 + m T_i^k) = x_i^k(t_0)$ for every $0 \le m \le M_i^k$,


    \item[(ii)] $t_0 + M_i^k T_i^k \le \tau_{q+1}(k + \frac{i}{4} - \lambda_{q+1}^{-1})$ and $t_0 + (M_i^k + 1) T_i^k > \tau_{q+1}(k + \frac{i}{4} - \lambda_{q+1}^{-1})$,
\end{itemize}
where
\begin{equation}
    T_i^k 
    = \int_0^{c_i\lambda_{q+1}} \frac{r_{q+1}}{\eta_i^k} a_i^k(x_i^k(t_0) + s\xi_i)\, ds
    = \frac{c_i\lambda_{q+1} r_{q+1}}{\eta_i^k} \int_{\mathbb{T}^2}a_i^k(x)\, dx
\end{equation}
is the time period. Notice that
\begin{equation}\label{eq:M}
    M_i^k = \Big\lfloor \frac{\tau_{q+1}(\frac{1}{4} - \frac{2}{\lambda_{q+1}})\eta_i^k}{c_i \lambda_{q+1}r_{q+1}\int_{\mathbb{T}^2}a_i^k(x)\, dx} \Big\rfloor \, .
\end{equation}


% \newpage

% %The initial time of the evolution is $t_0 = k \tau_{q+1} + (i-1) \frac{\tau_{q+1}}{4}$, the final time is $t_1 = k \tau_{q+1} + i \frac{\tau_{q+1}}{4}$. 
% We introduce a convenient constant-speed reparameterization of $x_i^k(t)$. Let $t(s)\in \mathcal{T}_i^k$ with $s\in [0, L(\eta)]$ such that $[t(0), t(L(\eta))] = \mathcal{T}_i^k$ and
% \begin{equation}\label{eq:change variables1}
%     x_i^k(t(s)) = x_i^k(t_0) + s \xi_i \, , \quad s\in [0, L(\eta)] \, ,
% \end{equation}
% It is easy to check that
% \begin{equation}\label{eq:change variables 2}
%     \frac{d}{ds} t(s) = \frac{r_{q+1}}{\eta \zeta_i^k(t(s))} a_i^k(x_i^k(t_0) + s \xi_i) \, ,
%     \quad \text{for every $s\in [0, L(\eta)]$} \, .
% \end{equation}
% The mapping $\eta \to L(\eta)$ is smooth, monotone and satisfies $\lim_{\eta\to 0} L(\eta)=0$ and $\lim_{\eta \to \infty} L(\eta)=\infty$. In particular, there exists $\eta_i^k>0$ such that
% \begin{equation}\label{z1}
%     \eta_i^k L(\eta_i^k) = \frac{\tau_{q+1}}{r_{q+1}} \, .
% \end{equation}
% Let $M_k^i \in \N$ be the number of times $t' \in (t_0,t_1]$ such that $x_i^k(t')=x_i^k(t_0)$. It is not hard to check that
% \begin{equation}\label{eq:MvsL}
%     c_i \lambda_{q+1} M_i^k \le L(\eta_i^k) \le c_i \lambda_{q+1} (M_i^k + 1) \, .
% \end{equation}



% The next step consists in estimating $\eta_i^k$. To this aim, it is convenient to select an initial condition $x_i^k(t_0)$ such that
% \begin{equation}\label{eq:initialtraj}
%     \int_0^{c_i\lambda_{q+1}} a_i^k(x_i^k(t_0) + s\xi_i) \, ds = c_i \lambda_{q+1} \int_{\mathbb{T}^2} a_i^k(x) \, dx \, .
% \end{equation}
% Such a choice can be made since the right-hand side of \eqref{eq:initialtraj} is the expectation of the term in the left-hand side when the initial condition is uniformly distributed on the torus. 

% \begin{proposition}
%     Assume that $10 \delta_{q+1}^{-2}\lambda_{q+1} r_{q+1} \le \tau_{q+1} \le 1/100$ and \eqref{eq:initialtraj}. Then
%     \begin{equation}
%         2\delta_{q+1}^{1/2} \le \eta_i^k \le 10 \delta_{q+1}^{1/2}
%     \end{equation}
% \end{proposition}



% \begin{proof}
% We begin by proving the lower bound on $\eta_i^k$. By \eqref{eq:change variables 2}, and the pointwise estimates 
% \begin{equation}
%     a_i(x,t) \ge \delta_{q+1} \, ,
%     \quad
%     \zeta_i^k(t) \le 1 \, ,
% \end{equation}
% we have
% \begin{align}
%     \frac{\tau_{q+1}}{4} 
%     = \int_0^{L(\eta_i^k)} \frac{d}{ds}t(s) \, ds
%     &= \int_0^{L(\eta_i^k)} \frac{r_{q+1}}{\eta_i^k \zeta_i^k(t(s))} a_i^k(x_i^k(t_0) + s\xi_i) \, ds 
%     \\& \ge \int_0^{L(\eta_i^k)} \frac{r_{q+1}}{\eta_i^k} \delta_{q+1}\, dt
%     \\& = \frac{\tau_{q+1} \delta_{q+1}}{(\eta_i^k)^2}\, ,
% \end{align}
% where we used the identity \eqref{z1}.



% % From the inequality $\zeta_i^k\le 1$, \eqref{eq:MvsL}, and the choice of the initial condition \eqref{eq:initialtraj}, we deduce
% % \begin{align}
% %     \int_0^{L(\eta_i^k)} \frac{r_{q+1}}{\eta_i^k \zeta_i^k(t(s))} a_i^k(x_i^k(t_0) + s\xi_i) \, ds 
% %     &\ge
% %     \frac{r_{q+1}}{\eta_i^k} \int_0^{c_i\lambda_{q+1} M_i^k} a_i^k(x_i^k(t_0) + s\xi_i) \, ds
% %     \\& = \frac{r_{q+1} c_i \lambda_{q+1} M_i^k}{\eta_i^k} \int_{\mathbb{T}^2} a_i^k(x) \, dx
% %     \\&
% %     \ge \frac{1}{2} \frac{r_{q+1}}{\eta_i^k} L(\eta_i^k) \int_{\mathbb{T}^2} a_i^k(x) \, dx
% %     \\&
% %     = \frac{1}{2} \frac{\tau_{q+1}}{(\eta_i^k)^2} \int_{\mathbb{T}^2} a_i^k(x) \, dx
% % \end{align}
% % Since $a_i \ge \delta_{q+1}$, we deduce the sought lower bound.
 
% \bigskip


% We now prove the converse inequality. We claim that there exists $t'\in (t_0, t_0 + \tau_{q+1}/9)$ and $t''\in (t_1 - \tau_{q+1}/9, t_1)$ such that $\eta_i^k =1$ in $[t',t'']$ and $x_i^k(t') = x_i^k(t'') = x_i^k(t_0)$.
    

% Let us first prove how to conclude the upper bound on $\eta_i^k$ from the claim. It is immediate to see that $t'=t(c_i\lambda_{q+1}A)$, $t''=t(c_i\lambda_{q+1}B)$ for some $0\le A < B \le M_i^k$.
% Then,
% \begin{align*}
%     \frac{\tau_{q+1}}{100}
%     &\le 
%     t'' - t'
%     \\& =
%     \int_{c_i\lambda_{q+1}A}^{c_i \lambda_{q+1}B} \frac{r_{q+1}}{\eta_i^k \zeta_i^k(t(s))} a_i^k(x_i^k(t_0) + s\xi_i) \, ds 
%     \\& =
%     \int_{c_i\lambda_{q+1}A}^{c_i \lambda_{q+1}B} \frac{r_{q+1}}{\eta_i^k} a_i^k(x_i^k(t_0) + s\xi_i) \, ds 
%     \\& \le 
%     \int_{0}^{c_i\lambda_{q+1}M_i^k} \frac{r_{q+1}}{\eta_i^k} a_i^k(x_i^k(t_0) + s\xi_i) \, ds 
%     \\& =\frac{r_{q+1}}{\eta_i^k} c_i \lambda_{q+1} M_i^k\int_{\mathbb{T}^2} a_i^k(x)\, dx
%     \\& \le \frac{\tau_{q+1}}{(\eta_i^k)^2} \delta_{q+1} \, .
% \end{align*}
% We finally verify the claim ..


% {\color{blue}ONLY PLACE WE USE ESTIMATE IN THE ASSUMPTION}

% \end{proof}





\subsection{Auxiliary Building Block}\label{sec:auxiliary}

We define
\begin{equation}\label{eq:U}
    U(x,t) := \frac{d}{dt} \left( \eta_i^k \zeta_i^k(t) r_i^k(t) \right) \wt{U}_i^k(x - x_i^k(t)) \xi_i \, ,
    \quad t\in \mathcal{T}_i^k
\end{equation}
where $\wt{U}_i^k(x) \ge 0$ is a scalar function supported on a ball of radius $10 \lambda_{q+1}^{-1}$. Moreover, we assume that: 
\begin{itemize}
    \item[(i)]  Space-average one:
    \begin{equation}\label{eqn:tildeu1}
        \dashint_{\mathbb{T}^2} \wt{U}_i^k(x)\, dx = 1 \, ,
    \end{equation}
    


    \item[(ii)] For every $x\in \mathbb{T}^2$, it holds
     \begin{equation}\label{eqn:tildeu2}
         \dashint_0^{c_i \lambda_{q+1}} \wt{U}_i^k(x - (x_i^k(t_0) + s \xi_i))\, ds
         = 1 \, .
     \end{equation}



     \item[(iii)] For every $p\in [1,\infty]$ it holds
     \begin{equation}\label{eq:est tildeU}
         \| \wt{U}_i^k \|_{L^p} \le C(p) \lambda_{q+1}^{2 - \frac{2}{p}}\, .
     \end{equation}
\end{itemize}
To build a scalar function $\wt{U}_i^k$ satisfying (i) and (ii) we argue as follows: first, we fix any $\Omega \ge 0$, supported on a ball of radius $10 \lambda_{q+1}^{-1}$ and bigger than $ \lambda_{q+1}^{-2}$ on half of such a ball. Next, we define 
\begin{equation}
    \overline \Omega  (x) := \dashint_0^{c_i \lambda_{q+1}} \Omega (x - (x_i^k(t_0) + s \xi_i))\, ds,
\end{equation}
which is a function invariant on the set $\{ x\in \mathbb{T}^2: x= x_i^k(t_0) + s\xi_i\}$ and bounded below by a constant $c>0$ independent of $\lambda_{q+1}$. We then set $\wt{U}^k_i = \Omega / \overline \Omega$ and observe that it satisfies \eqref{eqn:tildeu2}, which in turn implies \eqref{eqn:tildeu1} by further integrating with respect to the variable $x$.

\begin{proposition}\label{prop:auxiliary}
    Assume $\lambda_{q+1}^2 r_{q+1} \delta_{q+1}^{1/2} \le \frac{\tau_{q+1}}{100}$.
    Define $\eta_i^k \in [2\delta_{q+1}^{1/2}, 10\delta_{q+1}^{1/2}]$ as in \eqref{eqn:choiceetamagic}. Then,
    \begin{equation}
        \frac{1}{\tau_{q+1}}\int_{\mathcal{T}_i^k}U(x,t)\, dt
        = \div\left( a_i^k(x) \xi_i \otimes \xi_i
        + G_i^k(x)\right) \, ,
        \quad x\in \mathbb{T}^2 \, ,
    \end{equation}
    \begin{equation}\label{eq:Gik}
        \| G_i^k \|_{L^\infty_t L^1_x} 
        \le
       100 \tau_{q+1}\lambda_{q+1}^{-1} + 2 \lambda_{q+1}^{-1} \norm{a_i}_{C^1_{x,t}} \, .
    \end{equation}
\end{proposition}



\begin{proof}
As explained in Section \ref{sec:BB nonconstant speed}, the time average of $U(x,t)$ can be computed integrating by parts:
\begin{align}
\int_{\mathcal{T}_i^k}U(x,t)\, dt & = \int_{\mathcal{T}_i^k}\frac{d}{dt} \left( \eta_i^k \zeta_i^k(t) r_i^k(t) \right) \wt{U}_i^k(x - x_i^k(t)) \xi_i\, dt  \nonumber \\
& = - \int_{\mathcal{T}_i^k}  \eta_i^k \zeta_i^k(t) r_i^k(t)  \frac{d}{dt} \left( \wt{U}_i^k(x - x_i^k(t)) \right) \, \xi_i\, dt \nonumber \\
& = \int_{\mathcal{T}_i^k}  \left( \eta_i^k \zeta_i^k(t) \right)^2  \div \left( \wt{U}_i^k(x - x_i^k(t)) \xi_i \otimes \xi_i \right)\, dt \nonumber \\
& = \div \left( \int_{\mathcal{T}_i^k}  \left( \eta_i^k \zeta_i^k(t) \right)^2   \wt{U}_i^k(x - x_i^k(t)) \xi_i \otimes \xi_i \, dt \right)\, .
\end{align}


Notice that \eqref{eq:imp} is satisfied for $\lambda_{q+1}^2 r_{q+1} \delta_{q+1}^{1/2} \le \frac{\tau_{q+1}}{100}$ and $\eta_i^k \in [2\delta_{q+1}^{1/2}, 10\delta_{q+1}^{1/2}]$. Using the notation of Section \ref{sub:traj cent}, we set $\wt{\mathcal{T}_i^k} = [t_0, t_0 + M_i^k T_i^k]$, and recall that $\zeta_i^k(t)=1$ for every $t\in \wt{\mathcal{T}_i^k}$. 
We decompose
\begin{equation}
\begin{split}
    \int_{\mathcal{T}_i^k}&  \left( \eta_i^k \zeta_i^k(t) \right)^2   \wt{U}_i^k(x - x_i^k(t)) \xi_i \otimes \xi_i \, dt
    \\& =\left(\eta_i^k \right)^2\int_{\wt{\mathcal{T}_i^k}} \wt{U}_i^k(x - x_i^k(t)) \xi_i \otimes \xi_i \, dt
    +
    \int_{\mathcal{T}_i^k\setminus \wt{\mathcal{T}_i^k}}  \left( \eta_i^k \zeta_i^k(t) \right)^2  
    \wt{U}_i^k(x - x_i^k(t)) \xi_i \otimes \xi_i \, dt
    \\& = I + II \, .
\end{split}
\end{equation}
The second term, $II$, will be part of the error $F_i^k$. So, we estimate it in $L^1$ by
\begin{equation}
    \| II \|_{L^1} 
    \le 
    (\eta_i^k)^2 \| \wt{U}_i^k \|_{L^1} \int_{\mathcal{T}_i^k\setminus \wt{\mathcal{T}_i^k}}
    (\zeta_i^k(t))^2\, dt
    \le 
    80 \delta_{q+1} \tau_{q+1} \lambda_{q+1}^{-1} \, .
\end{equation}
Next, we study the main term $I$.
We change variables according to $t \to t(s) \in \wt{\mathcal{T}_i^k}$ such that $x_i^k(t(s)) = x_i^k(t_0) + s \xi_i$, where $t(0)=t_0$. Notice that
\begin{equation}
    \frac{d}{ds} t(s) = \frac{r_{q+1}}{\eta_i^k \zeta_i^k(t(s))} a_i^k(x_i^k(t_0) + s \xi_i)\, .
\end{equation}
We have,
\begin{align}
    I & 
    = \eta_i^k r_{q+1} \int_0^{c_i M_i^k \lambda_{q+1}} (a_i^k \wt{U}_i^k)(x - (x_i^k(t_0) + s\xi_i)) \, \xi_i \otimes \xi_i\,  ds
    \\& 
    =\eta_i^k r_{q+1} a_i^k(x) \int_0^{c_i M_i^k \lambda_{q+1}} \wt{U}_i^k(x - (x_i^k(t_0) + s\xi_i)) \, \xi_i \otimes \xi_i\,  ds
    \\& + \eta_i^k r_{q+1} \int_0^{c_i M_i^k \lambda_{q+1}} (a_i^k(x - (x_i^k(t_0) + s\xi_i) - a_i^k(x)) \wt{U}_i^k(x - (x_i^k(t_0) + s\xi_i)) \, \xi_i \otimes \xi_i\,  ds
    \\& = I' + II'
\end{align}
where, again $I'$ is the main term and $II''$ will be part of the error. So, we estimate
\begin{equation}
    \| II' \|_{L^1} \le \eta_i^k r_{q+1} c_i M_i^k \lambda_{q+1} \lambda_{q+1}^{-1} \| a_i^k \|_{C^1}
\end{equation}
Finally, we apply \eqref{eqn:tildeu2} to get
\begin{equation}
    \begin{split}
        I' & = \eta_i^k r_{q+1} a_i^k(x) \int_0^{c_i M_i^k \lambda_{q+1}} \wt{U}_i^k(x - (x_i^k(t_0) + s\xi_i))\, \xi_i \otimes \xi_i \, ds
        \\& = 
        \eta_i^k r_{q+1} c_i M_i^k \lambda_{q+1} a_i^k(x) \xi_i \otimes \xi_i \, .
    \end{split}
\end{equation}
Recalling \eqref{eqn:tildeu2}, we have 
\begin{equation}
    \begin{split}
        \eta_i^k r_{q+1} c_i M_i^k \lambda_{q+1} 
        & = 
        \eta_i^k r_{q+1} c_i 
        \Big\lfloor \frac{\tau_{q+1}(\frac{1}{4} - \frac{2}{\lambda_{q+1}})\eta_i^k}{c_i \lambda_{q+1}r_{q+1}\int_{\mathbb{T}^2}a_i^k(x)\, dx} \Big\rfloor \lambda_{q+1}
        \\& = \frac{\tau_{q+1} (\eta_i^k)^2(\frac{1}{4} - \frac{2}{\lambda_{q+1}})}{\int_{\mathbb{T}^2} a_i^k(x)\, dx} 
        -
        \eta_i^k r_{q+1} c_i \left\lbrace \frac{\tau_{q+1}(\frac{1}{4} - \frac{2}{\lambda_{q+1}})\eta_i^k}{c_i \lambda_{q+1}r_{q+1}\int_{\mathbb{T}^2}a_i^k(x)\, dx}  \right\rbrace\lambda_{q+1} \\& =
      {\color{red}  1  - 8 \frac{\tau_{q+1}}{\lambda_{q+1}} - \eta_i^k r_{q+1} c_i \left\lbrace \frac{\tau_{q+1}(\frac{1}{4} - \frac{2}{\lambda_{q+1}})\eta_i^k}{c_i \lambda_{q+1}r_{q+1}\int_{\mathbb{T}^2}a_i^k(x)\, dx}  \right\rbrace\lambda_{q+1} } \\
     {\color{red} \text{Division by } \tau_{q+1}. }\, ,
    \end{split}
\end{equation}
where we used \eqref{eqn:choiceetamagic}, and denote by $\left\lbrace x\right\rbrace$ the fractional part of $x\in \R$.
% We finally choose
% \begin{equation}
%     (\eta_i^k)^2 =  \frac{\int_{\mathbb{T}^2}a_i^k(x) \, dx}{\frac{1}{4} - \frac{2}{\lambda_{q+1}}}
%     \in [2 \delta_{q+1}, 4 \delta_{q+1}]\, ,
% \end{equation}
We add the term
\begin{equation}
    - \left(8 \frac{\tau_{q+1}}{\lambda_{q+1}} +
    \eta_i^k r_{q+1} c_i \left\lbrace \frac{\tau_{q+1}(\frac{1}{4} - \frac{2}{\lambda_{q+1}})\eta_i^k}{c_i \lambda_{q+1}r_{q+1}\int_{\mathbb{T}^2}a_i^k(x)\, dx}  \right\rbrace\lambda_{q+1}\right) \, a_i^k(x) \xi_i \otimes \xi_i
\end{equation}
to the error $F_i^k$. Notice that
\begin{equation}
   \eta_i^k r_{q+1} c_i \left\lbrace \frac{\tau_{q+1}(\frac{1}{4} - \frac{2}{\lambda_{q+1}})\eta_i^k}{c_i \lambda_{q+1}r_{q+1}\int_{\mathbb{T}^2}a_i^k(x)\, dx}  \right\rbrace\lambda_{q+1}
   \le 
   10 \delta_{q+1}^{1/2} r_{q+1} \lambda_{q+1} 
\end{equation}
So, in conclusion
\begin{equation}
\begin{split}
    \| G_i^k \|_{L^1} 
    & \le  80 \delta_{q+1} \tau_{q+1} \lambda_{q+1}^{-1} 
    + 2\lambda_{q+1}^{-1} \| a_i^k \|_{C^1}
    + 8 \tau_{q+1}\lambda_{q+1}^{-1}
    + 10 \delta_{q+1}^{1/2} r_{q+1}\lambda_{q+1} 
   \\& \le  100 \tau_{q+1}\lambda_{q+1}^{-1} + 2 \lambda_{q+1}^{-1} \norm{a_i^k}_{C^1}\, .
\end{split}  
\end{equation}







% {\color{red}


% \begin{align}
% \dashint_{\mathcal{T}_i^k}U(x,t)\, dt & = \div \left( \frac{4 r_{q+1}}{\tau_{q+1}} \int_0^{M_i^k c_i \lambda_{q+1}}   \eta_i^k(t(s)) \, a_i^k(x_i^k(t_0) + s \xi) \,   \wt{U}_i^k(x - (x_i^k(t_0) + s \xi_i)) \otimes \xi_i \, ds \right) \nonumber \\
% & = \div \left(  \frac{4 r_{q+1}a_i^k(x)}{\tau_{q+1}} \int_0^{M_i^k c_i \lambda_{q+1}}   \eta_i^k(t(s))  \,   \wt{U}_i^k(x - (x_i^k(t_0) + s \xi_i)) \otimes \xi_i \, ds + 4S^k_i\right)
% \end{align}
% where
% \begin{align}
% S^k_i = \frac{4}{\tau_{q+1}} \int_0^{M_i^k c_i \lambda_{q+1}}   \eta_i^k(t(s)) \, ( r(x_0 + s \xi) - r(x) ) \,   \wt{U}_i^k(x - (x_0 + s \xi_i)) \otimes \xi_i \, ds 
% \end{align}


% At this point we realize that we can essentially make two choice of $\eta^k_i$, one is that we choose $\eta^k_i$ with very sharp cutoff or require that $\tau_{q+1}$ is much bigger that one time period. Ideally, both should work but the one with sharp cutoff might be a bit easier. One should design a cutoff which goes from $0$
%  to $1$ on time interval $T_\xi$ (one time period corresponding to flat $\eta$) and then it stays constant on interval of size order $\tau_{q+1}$ and goes to zero again in $T_\xi$ time.  
% }

%\begin{align}
%    \dashint_{\mathcal{T}_i^k}U(x,t)\, dt
%    &=
%    \dashint_{\mathcal{T}_i^k}
%    \eta_i^k(t)^2\left(\frac{\nabla a_i^k(x_i^k(t))\cdot \xi_i}{a_i^k(x_i^k(t))} \right) \wt{U}_i^k(x - x_i^k(t)) \, dt
%    \\& =
%     r_{q+1}\dashint_{\mathcal{T}_i^k} \eta_i^k(t) \wt{U}_i^k(x - x_i^k(t))\frac{d}{d t} a_i^k(x_i^k(t)) \, dt
%     \\&=
%     - r_{q+1}\dashint_{\mathcal{T}_i^k} a_i^k(x_i^k(t)) \frac{d}{dt}(\eta_i^k(t) \wt{U}_i^k(x - x_i^k(t)))\, dt
%     \\&=
%     \dashint_{\mathcal{T}_i^k} \eta_i^k(t)^2 \div\left( \wt{U}_i^k(x-x_i^k(t)) \otimes \xi_i \right)\, dt
%     \\& \quad \quad
%     -r_{q+1} \dashint_{\mathcal{T}_i^k} a_i^k(x_i^k(t)) \wt{U}_i^k(x-x_i^k(t)) \frac{d}{dt} \eta_i^k(t)\, dt
%\end{align}


%\begin{equation}
%    \dashint_{\mathcal{T}_i^k}U(x,t)\, dt
%    =
%    \div\left( \dashint_{\mathcal{T}_i^k}   \eta_i^k(t)\wt{U}_i^k(x-x_i^k(t)) \otimes \xi_i \, dt\right)
%\end{equation}

%We focus on
%\begin{equation}
%    \int_{\mathcal{T}_i^k}   \eta_i^k(t)\wt{U}_i^k(x-x_i^k(t)) \otimes \xi_i \, dt
%\end{equation}
%and change variables according to $s\to t(s)$, where $t(0)=t_0$ and $x_i^k(t(s))= x_i^k(t_0) + s \xi_i$, it gives
%\begin{align}
%\dashint_{\mathcal{T}_i^k} &  \eta_i^k(t)\wt{U}_i^k(x-x_i^k(t)) \otimes \xi_i \, dt
%\\&=
%4\tau_{q+1}^{-1}r_{q+1}\int_0^{M_i^k c_i \lambda_{q+1}}
%    a_i^k(x_i^k(t_0) + s\xi_i) \wt{U}_i^k(x - (x_i^k(t_0) + s\xi_i))\otimes \xi_i \, ds
%\\& =
%4\tau_{q+1}^{-1}r_{q+1} a_i^k(x)\int_0^{M_i^k c_i \lambda_{q+1}}\wt{U}_i^k(x - (x_i^k(t_0) + s\xi_i))\otimes \xi_i \, ds 
%+ 4 S_i^k
%\\&=
%4\tau_{q+1}^{-1}r_{q+1}\lambda_{q+1}c_i M_i^k a_i^k(x) \xi_i \otimes \xi_i + 4 S_i^k
%\\& =
%4 a_i^k(x) \xi_i \otimes \xi_i + 4 S_i^k
%\end{align}
%where
%\begin{equation}
%    S_i^k = 
%\tau_{q+1}^{-1}r_{q+1}\int_0^{M_i^k c_i \lambda_{q+1}}
%    (a_i^k(x_i^k(t_0) + s\xi_i) - a_i^k(x))\wt{U}_i^k(x - (x_i^k(t_0) + s\xi_i))\otimes \xi_i \, ds
%\end{equation}
\end{proof}














\section{Perturbation and New Error}

The goal of this section is to define $(u_{q+1}, p_{q+1}, R_{q+1})$, the new solution to the Euler-Reynolds system \eqref{eq:ER}. We then check the relevant estimates to conclude the proof of Proposition \ref{prop:iteration}.


\subsection{Parameters}
We begin by choosing the parameters in Proposition \ref{prop:iteration}. We set
\begin{equation}\label{eq:cond2}
    \mu = 10\, , \quad
    \beta = 10^{-4}\, , \quad
    \sigma = 10^4 \mu \, , \quad
    N= 6 \mu \, .
\end{equation}
With this choice, it is immediate to verify that $r_{q+1}^{1/9} \le \lambda_q^{-24N} \delta_{q+1}^{11}$, hence
\begin{equation}
    r_{q+1} \delta_{q+1} \le r_i^k(x) \le r_{q+1}^{8/9} \, , \quad \text{for every $x\in \mathbb{T}^2$}\, .
\end{equation}
We then define the parameter $\tau_{q+1}$ as
\begin{equation}\label{eq:cond1}
    \frac{\tau_{q+1}}{100}
    =
    \lambda_{q+1}^2 r_{q+1} \delta_{q+1}^{1/2} \, ,
\end{equation}
notice that 
\begin{equation}
    \tau_{q+1} \le 100 r_{q+1}^{3/4} \, ,
\end{equation}
and Proposition \ref{prop:auxiliary} holds.



The value of $\lambda_0$ will depend on the universal constants appearing in our estimates, we will choose $\lambda_0$ big enough to absorb these constants.







\subsection{Principal Building Blocks}
For each $i=1,2,3,4$ and $k\in \N$, we let $V_i^k(x,t)$ be the solution to
\begin{equation}
\begin{cases}
\partial_t V_i^k + \div(V_i^k\otimes V_i^k) + \nabla P_i^k = 
 S_i^k {\frac{d}{dt} \left( \eta_i^k \zeta_i^k(t) r_i^k(t) \right)} +  \div(F_i^k)\, ,
 \quad t\in \mathcal{T}_i^k \, ,
 \\
 \div V_i^k =0 \, ,
 \end{cases}
\end{equation}
as in Proposition \ref{prop:build-block1},
with scale function $r_i^k(x)$, time cut-off $\eta_i^k \zeta_i^k(t)$, and $\eta_i^k \in [2\delta_{q+1}^{1/2}, 10\delta_{q+1}^{1/2}]$ chosen as in \ref{eqn:choiceetamagic}. The following estimates hold:

\begin{enumerate}[label = (\roman*)]



\item Estimate on the Reynolds stress tensor:
\begin{equation}\label{eq:Fik}
\begin{split}
\norm{F_i^k}_{L_t^\infty L_x^1} 
&\le 
C \delta_{q+1}^{1/2} (r_{q+1} \| a_i^k \|_{C^1})^{1/3} (1 + \| \log(a_i^k)\|_{C^1})
\\&
\le C r_{q+1}^{\frac{8}{27}}
\norm{a_i}_{C^1_{x,t}} 
\le C r_{q+1}^{\frac{8}{27}} \delta_{q+1}^{-11} \lambda_q^{24N}
 \\& \le C r_{q+1}^{1/6}\, ,
\end{split}
\end{equation}
thanks to our choice of parameters \eqref{eq:cond2}.


\item For every $p\in (1,\infty)$, it holds
\begin{align}\label{est:ki}
&\| V_i^k \|_{L^\infty_t L_x^p} + r_{q+1}^{1/2} \| D V_i^k\|_{L^\infty_t L^p_x} 
\leq 
C(p)  \delta_{q+1}^{1/2} r_{q+1}^{\frac{1}{p}-\frac{1}{2}} \, ,
\\
&\| S_i^k \|_{L^\infty_t L^p_x} \le C(p) r_{q+1}^{\frac{1}{p} - 1}\, .
\end{align}
Moreover, by using \eqref{eq:cond1} and \eqref{eq:cond2} we deduce
\begin{equation}\label{eq:time der est}
\begin{split}
\| \partial_t V_i^k \|_{L^\infty_t L^p_x} 
&\le C(p)(\delta_{q+1}^{-3}r_{q+1}^{-3}\|a_i^k\|_{C^1} + \delta_{q+1}^{-1/2}\lambda_{q+1}r_{q+1}^{-1}\tau_{q+1}^{-1})
\le C(p) r_{q+1}^{-4}\, .
\end{split}
\end{equation}

\item The source term $S_i^k$ is concentrated on a ball of radius $\lambda_{q+1}^{-1}$ and satisfies
\begin{align}\label{eq:S_i^k mean}
\supp S_i^k(\cdot, t) \subseteq B_{\lambda_{q+1}^{-1}}(x_i^k(t)), \qquad   \int_{\mathbb{T}^2} S_i^k(x,t)\, {\rm d} x =   \xi_i \, .
\end{align}
\end{enumerate}


\begin{remark}[Normalization of $S_i^k$]
   From Proposition \ref{prop:bb constant spead}, the average of $S_i^k$ should be $2\pi \xi_i$. However, for the sake of simplicity we normalize $V_i^k$, rescaling accordingly the time variable, so that \eqref{eq:S_i^k mean} holds. 
\end{remark}



\subsection{Auxiliary Building Block}
We consider the auxiliary building block 
\begin{equation}\label{eq:U1}
    U(x,t) := \frac{d}{dt} \left( \eta_i^k \zeta_i^k(t) r_i^k(t) \right) \wt{U}_i^k(x - x_i^k(t)) \xi_i \, ,
    \quad t\in \mathcal{T}_i^k
\end{equation}
as in Section~\ref{sec:auxiliary}.
From Proposition \ref{prop:auxiliary}, we deduce that
\begin{equation}
    P_\tau U(x,t) = \sum_{i=1}^4 \div\left(a_i^k(x) \xi_i \otimes \xi_i +  G_i^k(x,t) \right) \, ,
    \quad t\in \mathcal{T}^k\, ,
\end{equation}
where the operator $P_\tau$ has been introduced in \eqref{eq:Ptau}.


% We finally recall the estimate from 
% \begin{equation}\label{eq:est tildeU2}
%          \| \wt{U}_i^k \|_{L^p} \le C(p) \lambda_{q+1}^{2 - \frac{2}{p}}\, ,
%          \quad \text{for every $p\in [1,\infty]$ }\, ,
% \end{equation}
% form \eqref{eq:est tildeU}.


\subsection{Velocity Perturbation}
\label{sec:velocity perturbation}
We define the velocity field $u_{q+1}$ as
\begin{equation}
    u_{q+1}(x,t) = u_\ell(x,t) + v_{q+1}(x,t) + Q_{q+1}(x,t) \, ,
    \quad\quad 
    x\in \mathbb{T}^2\, , \, \, t\ge 0\, .
\end{equation}
The main perturbation is given by
\begin{equation}
    v_{q+1}(x,t) = \sum_{k\in \N} \sum_{i=1}^4 V_i^k(x,t) \, ,
\end{equation}
and the time correct is
\begin{equation}\label{eq:Q}
    - Q_{q+1}(x,t) = \mathbb{P}\left( \int_0^t (U(x,s) - P_\tau U(x,s))\, ds 
    %+  \xi_i \int_0^t r_i^k(s){\frac{d}{ds}\eta_i^k(s)}\, ds
    \right) \, .
\end{equation}






\subsection{New Error}
\label{sec:New error}
By plugging $u_{q+1}$ into \eqref{eq:ER}, we obtain the new error
\begin{equation}\label{eq:Rq+1 dec}
    R_{q+1} = 
    R_{q+1}^{(l)} 
    +
    R_{q+1}^{(c)}
    +
    R_{q+1}^{(t)}
    +
    R_{q+1}^{(s)}
    +
    \sum_k \sum_i (F_{i}^k + G_i^k)
\end{equation}
where $F_i^k$ satisfies \eqref{eq:Fik}, $G_i^k$ is given by Proposition \eqref{prop:auxiliary} and satisfies \eqref{eq:Gik}.
Then, 
\begin{equation}
    \begin{split}
        R_{q+1}^{(l)} 
        & = v_{q+1} \otimes u_\ell + u_\ell \otimes v_{q+1} \, ,
        \\
        R_{q+1}^{(c)} & = Q_{q+1} \otimes (u_\ell + v_{q+1}) + (u_\ell + v_{q+1}) \otimes Q_{q+1}  
        + Q_{q+1} \otimes Q_{q+1} \, ,      
    \end{split}
\end{equation}
where $R^{(l)}_{q+1}$ represents those terms that are linear in the perturbation, and $R_{q+1}^{(c)}$ is the collection of terms involving the time corrector $Q_{q+1}$. Finally, we define
\begin{equation}
    \begin{split}
    R_{q+1}^{(t)}(x,t) & = a_i(x,t) -  a_i^k(x)
        \\
    R_{q+1}^{(s)}(x,t) & = \mathcal{R}_0\left( S_i^k \frac{d}{dt}(\eta_i^k \zeta_i^k r_i^k ) - U_i^k\right)(x,t)
    \end{split}
    \quad \quad \text{for $t\in \mathcal{T}_i^k$} \, .
\end{equation}
From \eqref{eq:a-aik}, \eqref{eq:cond1}, and \eqref{eq:cond2} we deduce that
\begin{equation}\label{eq:Rt}
\begin{split}
    \| R_{q+1}^{(t)}\|_{L^\infty_t L^1_x} 
    &\le \tau_{q+1} 
    \| a_i \|_{C^1_{x,t}}
    \le \tau_{q+1} \delta_{q+1}^{-11}\lambda_q^{24N}
    \\&
    \le  100 r_{q+1} \lambda_{q+1}^{2} \delta_{q+1}^{-11}\lambda_q^{24N}
    \\& \le 100 r_{q+1}^{1/2}
    \, .
\end{split}
\end{equation}
Moreover, from Proposition \ref{prop:antidiv compact} and \eqref{eq:est tildeU}, we see that
\begin{equation}
\begin{split}
     \| R_{q+1}^{(s)}\|_{L^\infty_t L^p_x} 
     &\le C(p) \lambda_{q+1}^{-1}
     \left( \| S_i^k\|_{L^\infty_t L^p_x} + \| U_i^k\|_{L^\infty_tL^p_x}\right) 
     \sup_{i,k}\Big| \frac{d}{dt}(\eta_i^k \zeta_i^k r_i^k)\Big|
     \\&
     \le C(p) \lambda_{q+1}^{-1} r_{q+1}^{\frac{1}{p}-1} \sup_{i,k}\Big| \frac{d}{dt}(\eta_i^k \zeta_i^k r_i^k)\Big| \, ,
\end{split}
\end{equation}
for every $p\in (1,\infty)$.
Then, from \eqref{eq:traj1}, and \eqref{eq:cond1}
we see that
\begin{equation}\label{eq:der}
\begin{split}
    \Big| \frac{d}{dt}(\eta_i^k \zeta_i^k r_i^k)\Big|
    & \le
    \left( \delta_{q+1}^{1/2} \lambda_{q+1} \tau_{q+1}^{-1} r_{q+1} \| a_i^k\|_{L^\infty}  + \delta_{q+1} \| a_i^k \|_{C^1} \right)
    \\& \le 
    2 \delta_{q+1}^{1/2} \| a_i^k \|_{C^1}
    \le 
   2 \delta_{q+1}^{-11} \lambda_q^{24N}\, .
\end{split}
\end{equation}
So, we conclude
\begin{equation}
    \| R_{q+1}^{(s)}\|_{L^\infty_t L^1_x} 
     \le C(p) \lambda_{q+1}^{-1} r_{q+1}^{\frac{1}{p}-1} \delta_{q+1}^{-11} \lambda_q^{24N}\, ,
     \quad p\in (1,\infty)\, .
\end{equation}
Recalling that $r_{q+1}=\lambda_{q+1}^{-\mu}$ (see \eqref{eq:parameters}), we can choose $p>1$ depending on $\mu>0$ such that
\begin{equation}\label{eq:Rs}
    \| R_{q+1}^{(s)}\|_{L^\infty_t L^1_x} 
     \le C(\mu) \lambda_{q+1}^{-1/2}  \delta_{q+1}^{-11} \lambda_q^{24N}\, 
     \le C \lambda_{q+1}^{-1/4}\, .
\end{equation}





\subsection{Estimate on $Q_{q+1}$}
Fix $t\in \mathcal{T}^k$. By definition of $P_\tau$, we have
\begin{equation}
    -Q_{q+1}(x,t) = \mathbb P \int_{k \tau}^t \left(U(x,s) - \dashint_{\mathcal{T}^k} U(x, s')\, ds' \right)\, ds \,
\end{equation}
In view of \eqref{eq:U} and the estimate \eqref{eq:der}, we deduce
\begin{align}
    |Q_{q+1}(x,t)| & \le 2 \tau_{q+1} \dashint_{\mathcal{T}^k} \Big| \frac{d}{ds}(\eta_i^k \zeta_i^k(s) r_i^k(s))\Big|
    \Big| \left(\mathbb{P} \wt{U}_i^k \right)(x - x_i^k(s)) \Big|
    \, ds
    \\& \le 4 \tau_{q+1}\delta_{q+1}^{-11} \lambda_q^{24N}\dashint_{\mathcal{T}^k}
    \Big| \left(\mathbb{P} \wt{U}_i^k \right)(x - x_i^k(s)) \Big| \, ds \, .
\end{align}
Similarly,
\begin{align}
    |D Q_{q+1}(x,t)| & \le 4 \tau_{q+1}\delta_{q+1}^{-11} \lambda_q^{24N} \dashint_{\mathcal{T}^k} \Big| \left(D\mathbb P \wt{U}_i^k\right)(x - x_i^k(s)) \Big| \, ds \, .
\end{align}
In particular, for every $p\in (1,\infty)$ we have
\begin{equation}\label{eq:estQ}
\begin{split}
    \| Q_{q+1} \|_{L^\infty_t L^p_x} + & \lambda_{q+1}^{-1} \| D Q_{q+1} \|_{L^\infty_t L^p_x}
    \le C(p) \tau_{q+1} \delta_{q+1}^{-11} \lambda_{q+1}^{2 - \frac{2}{p}} \lambda_q^{24N}
    \\&
    \le C(p) r_{q+1} \delta_{q+1}^{-11} \lambda_{q+1}^{4-\frac{2}{p}} \lambda_q^{24N}
     \le C(p) \lambda_{q+1}^{-3}\, .
\end{split}
\end{equation}
where in the second line we used \eqref{eq:cond1} and \eqref{eq:cond2}.






\subsection{Estimate on $R^{(l)}_{q+1}$ and $R^{(c)}_{q+1}$}

Fix $t\in \mathcal{T}_i^k$. From \eqref{est:ki} and \eqref{eq:u_q Sob}, we deduce
\begin{align}
    \| R_{q+1}^{(l)}(\cdot, t)\|_{L^1} &
    \le 2 \| v_{q+1}(\cdot, t)\|_{L^{3/2}} \| u_\ell\|_{L^3}
     \le  \| V_i^k(\cdot, t)\|_{L^{3/2}}\| u_q \|_{L^\infty}
    \\& \le 
    C \delta_{q+1}^{1/2} r_{q+1}^{1/6} \| u_q\|_{L^\infty_t L^4_x}
    \le C \delta_{q+1}^{1/2} r_{q+1}^{1/6} \lambda_q^{N}\, .
\end{align}
Hence, using \eqref{eq:cond2} we deduce
\begin{equation}\label{eq:Rl}
    \| R^{(l)}_{q+1}\|_{L^\infty_t L^1_x} \le C \delta_{q+1}^{1/2} r_{q+1}^{1/6} \lambda_q^{N}
    \le C\lambda_{q+1}^{-1}\, .
\end{equation}
From \eqref{eq:estQ}, it follows
\begin{align}\label{eq:Rc}
    \| R_{q+1}^{(c)} \|_{L^\infty_t L^1_x}
    &\le \| Q_{q+1} \|_{L^\infty_t L_x^2} ( 2 \| u_\ell \|_{L^\infty_t L^2_x} + 2 \| v_{q+1} \|_{L^\infty_t L^2_x} + \| Q_{q+1} \|_{L^\infty_t L^2_x})
    \\&
    \le C \lambda_{q+1}^{-3}(\lambda_q^N + \lambda_{q+1}^{-3})
    \\&
    \le C \lambda_{q+1}^{-1}
    \, .
\end{align}



\subsection{Estimates on $u_{q+1}$}
We begin by estimating the $L^2$ norm of $u_{q+1}$. We rely on \eqref{eq:estQ}, \eqref{est:ki}, and \eqref{eq:cond1}:

\begin{equation}\label{eq:uq+1 estL2}
\begin{split}
    \| u_{q+1} \|_{L^\infty_t L^2_x}
    & \le \| u_\ell \|_{L^\infty_tL^2_x} + \sup_{i,k}\| V_i^k \|_{L^\infty_t L^2_x} + \| Q_{q+1}\|_{L^\infty_t L^2_x}
    \\&
    \le \| u_q \|_{L^\infty_t L^2_x} + C\delta_{q+1}^{1/2} + C \lambda_{q+1}^{-3}
    \\&
    \le \| u_q \|_{L^\infty_t L^2_x} + \delta_{q+1}^{1/5} \, ,
\end{split}
\end{equation}
provided $\lambda_0>0$ is big enough.


\bigskip


Let us now estimate the $L^p$ of $D u_{q+1}$. Once more, we rely on \eqref{eq:estQ}, \eqref{est:ki}, and \eqref{eq:cond1}. Fix any $p\in (1,\infty)$, it holds:
\begin{equation}
    \begin{split}
        \| D u_{q+1}\|_{L^\infty_t L^p_x} & 
        \le \| D u_\ell \|_{L^\infty_t L^p_x} + \sup_{ik} \| D V_i^k \|_{L^\infty_t L^p_x} + \| D Q_{q+1} \|_{L^\infty_t L^p_x}
        \\& \le \| D u_q \|_{L^\infty_t L^p_x} + C(p) \delta_{q+1}^{1/2} r_{q+1}^{\frac{1}{p} - 1} + C(p)\lambda_{q+1}^{-2} \, .
    \end{split}
\end{equation}
We then recall \eqref{eq:cond2}, and observe that
\begin{equation}
    \delta_{q+1}^{1/2} r_{q+1}^{\frac{1}{p} - 1}
    =
    \lambda_{q+1}^{- \beta/2 + \mu\frac{p-1}{p}}
    \le \frac{1}{2}\delta_{q+1}^{1/5}
\end{equation}
provided $1<p< \frac{1}{1-10^{-6}}$ and $\lambda_0>0$ is big enough. Under these assumptions, we have
\begin{equation}\label{eq:Duq+1 key}
     \| D u_{q+1}\|_{L^\infty_t L^p_x} \le  \| D u_{q}\|_{L^\infty_t L^p_x} + \delta_{q+1}^{1/5}\, .
\end{equation}
For $p=4$, recalling \eqref{eq:cond1}, we have
\begin{equation}\label{eq:Duq+1 est}
    \| D u_{q+1} \|_{L^\infty_t L^p_x} \le \lambda_q^N + C \delta_{q+1}^{1/2} r_{q+1}^{-3/4} + C \lambda_{q+1}^{-2}
    \le \frac{1}{2}\lambda_{q+1}^{N} \, .
\end{equation}


\bigskip


Finally, we estimate the time derivative of $u_{q+1}$. We use \eqref{eq:time der est}, and the identity
\begin{equation}
    \partial_t Q_{q+1}(x,t) 
    = - \mathbb{P}U(x,t) + \mathbb{P} \dashint_{\mathcal{T}^k} U(x,s)\, ds \, ,
    \quad t\in \mathcal{T}^k\, .
\end{equation}
Recalling our choice of parameters \eqref{eq:cond2}, we deduce
\begin{equation}\label{eq:partial t uq est}
    \begin{split}
        \| \partial_t u_{q+1} \|_{L^\infty_t L^4_x}
        &\le \| \partial_t u_\ell \|_{L^\infty_t L^4_x} + \sup_{ik} \| \partial_t V_i^k \|_{L^\infty_t L^4_x} + \| \partial_t Q_{q+1} \|_{L^\infty_t L^p_x}
        \\&
        \le \lambda_q^N + C r_{q+1}^{-4} + 2\| U \|_{L^\infty_t L^4_x}
        \\& \le 
        \lambda_q^N + C r_{q+1}^{-4} + C \delta_{q+1}^{-11} \lambda_q^{24N} \lambda_{q+1}^{3/2}
        \\& \le \frac{1}{2} \lambda_{q+1}^N \, ,
    \end{split}
\end{equation}
where we estimated $\| U \|_{L^\infty_t L^4_x}$ by means on \eqref{eq:est tildeU} and \eqref{eq:der}.




\subsection{Proof of Proposition \ref{prop:iteration}, Conclusion}

Let $(u_{q+1}, p_{q+1}, R_{q+1})$ as in Section \ref{sec:velocity perturbation} and Section \ref{sec:New error}.
By \eqref{eq:Rq+1 dec}, and estimates \eqref{eq:Rt}, \eqref{eq:Rs}, \eqref{eq:Rl}, \eqref{eq:Rc} we obtain
\begin{equation}
    \| R_{q+1} \|_{L^\infty_t L^p_x} \le C r_{q+1}^{1/2} + C\lambda_{q+1}^{-1/5} + \lambda_{q+1}^{-1} + \sup_{ik} (\| F_i^k\|_{L^\infty_t L^1_x} + \| G_i^k\|_{L^\infty_t L^1_x})
\end{equation}
From \eqref{eq:Fik} and \eqref{eq:Gik} we get
\begin{equation}
    \| F_i^k \|_{L^\infty_t L^1_x} \le C r_{q+1}^{1/6} \, ,
    \quad\quad
    \| G_i^k\|_{L^\infty_t L^1_x}
    \le C \delta_{q+1}^{1/2}\lambda{q+1} r_{q+1} + 2 \lambda_{q+1}^{-1} \delta_{q+1}^{-11} \lambda_q^{24N \, .}
\end{equation}
Recalling our choice of parameters \eqref{eq:cond2} and choosing $\lambda_0$ big enough, we deduce
\begin{equation}\label{eq:Rq+1 est}
    \| R_{q+1} \|_{L^\infty_t L^1_x} \le \delta_{q+2} \, .
\end{equation}
By combining \eqref{eq:Duq+1 est} and \eqref{eq:partial t uq est}, we deduce
\begin{equation}\label{eq:Dxtuq est}
    \| D_{x,t} u_{q+1} \|_{L^\infty_t L^4_x} \le \lambda_{q+1}^N \, .
\end{equation}
The proof of Proposition \ref{prop:iteration} (i) is complete.

\bigskip

The proof of Proposition \ref{prop:iteration} (ii) follows from \eqref{eq:uq+1 estL2} and \eqref{eq:Duq+1 key}.










==> Figures/Old_Material/Anuj_Notes/Def_Perturbation.tex <==
\section{Definition of Perturbation}
\label{section: def perturbation}
The defintion of the perturbation is
\begin{align}
w_{n+1} = u_{n+1} - u_{\ell} = w_{n+1}^{(p)} + w_{n+1}^{(c)} + \ol{w}_{n+1}^{(t)} + \wt{w}_{n+1}^{(c)}
\end{align}
\begin{enumerate}[label = (\roman*)]
    \item $w_{n+1}^{(p)} \to $ the principal part
    \item $w_{n+1}^{(c)} \to $ the correction part
    \item $\ol{w}_{n+1}^{(t)} \to $ the first time corrector
    \item $\wt{w}_{n+1}^{(t)} \to $ the second time corrector
\end{enumerate}

The different parts of the perturbation in the component form
\begin{align}
w_{n+1}^{(p)} = \sum_{i=1}^{4} W^{(p)}_i, \qquad w_{n+1}^{(c)} = \sum_{i=1}^{4} W^{(c)}_i,\qquad  \ol{w}_{n+1}^{(t)} = \sum_{i=1}^{4} \ol{Q}_i, \qquad \wt{w}_{n+1}^{(t)} = \sum_{i=1}^{4} \wt{Q}_i
\end{align}
\subsection{A few basic definitions}
\label{subsection: basic definitions}
Given a function $f$ defined on $[0, 1] \times \mathbb{T}^2$, we define the time average $P_\tau$ as
\begin{align}
\left[P_{\tau}(f)\right](x) = \frac{1}{\tau} \int_{k \tau}^{(k+1) \tau} f(t, x) \, {\rm d} t
\end{align}
We let
\begin{align}
- \div(R_n) = \div\left(\sum_{i=1}^4 a_i^2(t, x) e_i \otimes e_i\right) + \nabla P
\end{align}
where $a_i$ are smooth functions and obey
\begin{align}
\inf_{t, x} |a_i^2(t, x)| \geq \norm{R_n}_{L^\infty_t L^1_x}.
\end{align}
We denote $P_\tau$ applied to coefficients $a_i^2(t, x)$ as
\begin{align}
\ol{a}_i^2(x) = P_\tau(a_i^2(t, x)).
\end{align}
Next, we define the building block speed as
\begin{align}
\mu(x) \coloneqq \frac{\mu_0}{P_\tau(a_i^2(t, x))} = \frac{\mu_0}{\ol{a}_i^2(x)}.
\end{align}
The trajectory $p(t)$ of the particle solves
\begin{align}
\frac{d p(t)}{dt} = \mu(p(t)) e_i, \qquad p(0) = x_s.
\end{align}
It is clear that
\begin{align}
\dot{p}(t) = \mu(p(t)) e_i \quad \implies \quad \ddot{p}(t) = (e_i \cdot \nabla \mu (p(t))) \, \mu(p(t)) \,  e_i.
\end{align}
We define the size parameters for the building block as 
\begin{align}
r^{\perp}(x) \coloneqq r^{\perp}_0 \; \ol{a}_i^2(x), \qquad r^{\parallel}(x) \coloneqq r^{\parallel}_0 \; \ol{a}_i^2(x).
\end{align}



\subsection{The principal part of the perturbation}
Let $\Phi, \psi: \mathbb{R} \to \mathbb{R}$ be supported in $(-1/2, 1/2)$. We set $$\phi(x) = \Phi^{\prime \prime \prime \prime}(x).$$
These functions are such that
\begin{align}
\int \psi^2 \, {\rm d} x = 1, \qquad \text{and} \qquad \int \phi^2 \, {\rm d} x = 1.
\end{align}
Finally, also consider
\begin{align}
\ol{\zeta}(t) = \zeta\left(\frac{t - k \tau - \frac{(i-1)}{4} \tau}{\tau/4}\right).
\end{align}
The function $\zeta$ is supported in $(0, 1)$ and is such $$\int_0^1 \zeta^2(t^\prime) \, {\rm d} t^\prime = 1.$$
We define rescaled functions as
\begin{align}
\ol{\psi}(t, x) \coloneqq \left(\frac{1}{r^{\parallel}(p(t))}\right)^{\frac{1}{2}} \psi\left(\frac{\lambda (x - p(t)) \cdot e_i}{r^{\parallel}(p(t))}\right)
\end{align}
\begin{align}
\ol{\phi}(t, x) \coloneqq \left(\frac{1}{r^{\perp}(p(t))}\right)^{\frac{1}{2}} \phi\left(\frac{\lambda (x - x_s) \cdot e^\perp_i}{r^{\perp}(p(t))}\right)
\end{align}
We define the principal part of the perturbation as
\begin{align}
W^{(p)}_i(x) = U_0 \, \ol{\psi}(t, x) \, \ol{\phi}(t, x) \, \ol{\zeta}(t) e_i
\end{align}
We will later see that
\begin{align}
U_0 \leq 4 \lambda \norm{R_n}^{\frac{1}{2}}_{L^\infty_t L^1_x}.
\end{align}




\subsection{The correction part of the perturbation}
\begin{align}
W^{(c)}_i(x) = - U_0 \, \frac{r^\perp(p(t))}{r^\parallel(p(t))} \,
\left(\frac{1}{r^{\parallel}(p(t))}\right)^{\frac{1}{2}}\left(\frac{1}{r^{\perp}(p(t))}\right)^{\frac{1}{2}} \, \psi^\prime(\dots) \, \Phi^{\prime \prime \prime}(\dots) \, \ol{\zeta}(t) e^\perp_i,
\end{align}
with this one can check
\begin{align}
\div(W^{(p)}_i + W^{(c)}_i) = 0.
\end{align}




\subsection{The first time corrector}
\label{subsection: first time corrector}
We define the first time corrector as
\begin{align}
\ol{Q}_i(t, x) & \coloneqq \frac{U_0^2}{\mu(p(t))} \, \ol{\psi}^2(t, x) \, \ol{\phi}^2(t, x) \, \ol{\zeta}^2(t) \, e_i \nonumber \\
& = \frac{U_0^2}{\mu(p(t))} \frac{1}{r^{\perp}(p(t))}  \frac{1}{r^{\parallel}(p(t))} \psi^2\left(\frac{\lambda (x - p(t)) \cdot e_i}{r^{\parallel}(p(t))}\right) \phi^2\left(\frac{\lambda (x - x_s) \cdot e^\perp_i}{r^{\perp}(p(t))}\right) \, \ol{\zeta}^2(t) \, e_i \nonumber \\
& = \frac{U_0^2}{\mu_0} \frac{1}{r^{\perp}_0}  \frac{1}{r^{\parallel}_0} \frac{1}{\ol{a}_i^2(p(t))} \psi^2\left(\frac{\lambda (x - p(t)) \cdot e_i}{r^{\parallel}(p(t))}\right) \phi^2\left(\frac{\lambda (x - x_s) \cdot e^\perp_i}{r^{\perp}(p(t))}\right) \, \ol{\zeta}^2(t) \, e_i
\end{align}
Next, we calculate the time derivative of the corrector.
\begin{align}
\partial_t \ol{Q}_i(t, x) = I + II + III + IV + V,
\end{align}
where 
\begin{align}
I & \coloneq - U_0^2 \frac{1}{r^{\perp}(p(t))}  \frac{1}{r^{\parallel}(p(t))} \frac{2 \lambda}{r^{\parallel}(p(t))} \psi^\prime\left(\frac{\lambda (x - p(t)) \cdot e_i}{r^{\parallel}(p(t))}\right) \psi\left(\frac{\lambda (x - p(t)) \cdot e_i}{r^{\parallel}(p(t))}\right) \times \nonumber \\
& \qquad \qquad \qquad \qquad \qquad \qquad \qquad \qquad \qquad \qquad \qquad \phi^2\left(\frac{\lambda (x - x_s) \cdot e^\perp_i}{r^{\perp}(p(t))}\right) \, \ol{\zeta}^2(t) \, e_i \nonumber \\
& = - \div(W_i^{(p)} \otimes W_i^{(p)}),
\end{align}
\begin{align}
II \coloneqq \frac{U_0^2}{\mu_0} \frac{1}{r^{\perp}_0}  \frac{1}{r^{\parallel}_0} \left(\frac{- \nabla \ol{a}_i^2(p(t)) \cdot e_i}{\ol{a}_i^4(p(t))} \, \mu(p(t)) \right) \psi^2\left(\frac{\lambda (x - p(t)) \cdot e_i}{r^{\parallel}(p(t))}\right) \phi^2\left(\frac{\lambda (x - x_s) \cdot e^\perp_i}{r^{\perp}(p(t))}\right) \, \ol{\zeta}^2(t) \, e_i \nonumber \\
= - U_0^2 \frac{1}{r^{\perp}(p(t))}  \frac{1}{r^{\parallel}(p(t))} \left(\frac{\nabla \ol{a}_i^2(p(t)) \cdot e_i}{\ol{a}_i^2(p(t))}\right) \psi^2\left(\frac{\lambda (x - p(t)) \cdot e_i}{r^{\parallel}(p(t))}\right) \phi^2\left(\frac{\lambda (x - x_s) \cdot e^\perp_i}{r^{\perp}(p(t))}\right) \, \ol{\zeta}^2(t) \, e_i 
\end{align}
\begin{align}
III \coloneqq \frac{U_0^2}{\mu_0} \frac{1}{r^{\perp}_0}  \frac{1}{r^{\parallel}_0} \frac{1}{\ol{a}_i^2(p(t))} \left[ \frac{2 \lambda (x - p(t)) \cdot e_i}{r^{\parallel}_0}\right] \left(\frac{- \nabla \ol{a}_i^2(p(t)) \cdot e_i}{\ol{a}_i^4(p(t))} \, \mu(p(t)) \right) \psi^\prime\left(\frac{\lambda (x - p(t)) \cdot e_i}{r^{\parallel}(p(t))}\right) \times & \nonumber \\
\psi\left(\frac{\lambda (x - p(t)) \cdot e_i}{r^{\parallel}(p(t))}\right) \, \phi^2\left(\frac{\lambda (x - x_s) \cdot e^\perp_i}{r^{\perp}(p(t))}\right) \, \ol{\zeta}^2(t) \, e_i & \nonumber \\
= - U_0^2 \left(\frac{\nabla \ol{a}_i^2(p(t)) \cdot e_i}{\ol{a}_i^2(p(t))}\right) \left[ (x - p(t)) \cdot e_i \right] \div\left[\ol{\psi}^2(t, x) \, \ol{\phi}^2(t, x) \, e_i \otimes e_i\right] \ol{\zeta}^2(t)
\end{align}
\begin{align}
IV \coloneqq \frac{U_0^2}{\mu_0} \frac{1}{r^{\perp}_0}  \frac{1}{r^{\parallel}_0} \frac{1}{\ol{a}_i^2(p(t))} \left[ \frac{2 \lambda (x - x_s) \cdot e^\perp_i}{r^{\perp}_0}\right] \left(\frac{- \nabla \ol{a}_i^2(p(t)) \cdot e_i}{\ol{a}_i^4(p(t))} \, \mu(p(t)) \right) \psi^2\left(\frac{\lambda (x - p(t)) \cdot e_i}{r^{\parallel}(p(t))}\right) \times & \nonumber \\
\phi^\prime\left(\frac{\lambda (x - x_s) \cdot e^\perp_i}{r^{\perp}(p(t))}\right) \, \phi\left(\frac{\lambda (x - x_s) \cdot e^\perp_i}{r^{\perp}(p(t))}\right) \, \ol{\zeta}^2(t) \, e_i & \nonumber \\
= - U_0^2 \left(\frac{\nabla \ol{a}_i^2(p(t)) \cdot e_i}{\ol{a}_i^2(p(t))}\right) \left[ (x - x_s) \cdot e^\perp_i \right] \div\left[\ol{\psi}^2(t, x) \, \ol{\phi}^2(t, x) \, e_i \otimes e_i^\perp\right] \ol{\zeta}^2(t)
\end{align}
\begin{align}
V \coloneqq  \frac{U_0^2}{\mu(p(t))} \, \ol{\psi}^2(t, x) \, \ol{\phi}^2(t, x) \, \left(\frac{2}{\tau/4}\right) \dot{\ol{\zeta}}(t) \ol{\zeta} \, e_i
\end{align}
Using integration by parts we, observe that
\begin{align}
\int_{\mathbb{T}^2} III \, {\rm d} x = - \int_{\mathbb{T}^2} II \, {\rm d} x 
\end{align}
and 
\begin{align}
\int_{\mathbb{T}^2} IV \, {\rm d} x = - \int_{\mathbb{T}^2} II \, {\rm d} x 
\end{align}
Therefore,
\begin{align}
\int_{\mathbb{T}^2} \left( II + III + IV \right) \, {\rm d} x = - \int_{\mathbb{T}^2} II \, {\rm d} x =  \int_{\mathbb{T}^2} \ol{II} \, {\rm d} x 
\end{align}
where we define the negative of the second term as
\begin{align}
\ol{II} & \coloneqq  U_0^2 \frac{1}{r^{\perp}(p(t))}  \frac{1}{r^{\parallel}(p(t))} \left(\frac{\nabla \ol{a}_i^2(p(t)) \cdot e_i}{\ol{a}_i^2(p(t))}\right) \psi^2\left(\frac{\lambda (x - p(t)) \cdot e_i}{r^{\parallel}(p(t))}\right) \phi^2\left(\frac{\lambda (x - x_s) \cdot e^\perp_i}{r^{\perp}(p(t))}\right) \, \ol{\zeta}^2(t) \, e_i \nonumber \\
& = U_0^2  \left(\frac{\nabla \ol{a}_i^2(p(t)) \cdot e_i}{\ol{a}_i^2(p(t))}\right) \ol{\psi}^2(t, x) \, \ol{\phi}^2(t, x) \, \ol{\zeta}^2(t) \, e_i.
\end{align}
Next, we define a sixth term
\begin{align}
VI = U_0^2  \left(\frac{\nabla \ol{a}_i^2(p(t)) \cdot e_i}{\ol{a}_i^2(p(t))}\right) \wt{\psi}^2(t, x) \, \wt{\phi}^2( x) \, \ol{\zeta}^2(t) \, e_i, 
\end{align}
where
\begin{align}
\wt{\psi}(t, x) \coloneqq \left(\frac{1}{K}\right)^{\frac{1}{2}} \psi\left(\frac{\lambda (x - p(t)) \cdot e_i}{K}\right)
\end{align}
\begin{align}
\wt{\phi}( x) \coloneqq \left(\frac{1}{K}\right)^{\frac{1}{2}} \phi\left(\frac{\lambda (x - x_s) \cdot e^\perp_i}{K}\right)
\end{align}
where $K$ is constant number smaller than $1$, to be chosen later based on convenience. The important thing to note is that
\begin{align}
\int_{\mathbb{T}^2} \left(\ol{II} - VI\right) \, {\rm d} x = 0.
\end{align}
Finally, we define a slightly altered version of the sixth term.
\begin{align}
VI^\prime = U_0^2  \left(\frac{\nabla \ol{a}_i^2(x) \cdot e_i}{\ol{a}_i^2(x)}\right) \wt{\psi}^2(t, x) \, \wt{\phi}^2(x) \, \ol{\zeta}^2(t) \, e_i, 
\end{align}

\subsection{The terms that go into the error}
\label{subsection: corrector 1 eqn error terms}
We will send the following terms into the next error
\begin{enumerate}[label = (\roman*)]
    \item The term $V$
    \item The term $II + III + IV - VI$
    \item The term $VI - VI^\prime$
\end{enumerate}
As a result we will have,
\begin{align}
\partial_t \ol{Q}_i(t, x) + \div(W_i^{(p)} \otimes W_i^{(p)}) = \text{ errors } + VI^\prime,
\end{align}
Let's quickly estimate these errors.
\begin{align}
\norm{ \div^{-1} V }_{L^\infty_t L^1_x} \leq \frac{32 \norm{ R_n }_{L^\infty_t L^\infty_x} \norm{ R_n }_{L^\infty_t L^1_x}}{\mu_0 \, \tau}.
\end{align}
\begin{align}
\norm{ \div^{-1} (II + III + IV - VI) }_{L^\infty_t L^1_x} \leq  \frac{4 \norm{ R_n }_{C^1_{t, x}}}{\lambda}
\end{align}
\begin{align}
\norm{ \div^{-1} (VI - VI^\prime) }_{L^\infty_t L^1_x} \leq  \left( \norm{ R_n }_{C^2_{t, x}} + \frac{ \norm{ R_n }^2_{C^1_{t, x}}} {\norm{ R_n }_{L^\infty_t L^1_x}}\right)\frac{1}{\lambda}
\end{align}



\subsection{The second time corrector}
\label{subsection: second time corrector}
We define the second time corrector to be
\begin{align}
\wt{Q}(t, x) & \coloneqq \int_0^t \left[ VI^\prime - P_{\tau}(VI^\prime)\right] \, {\rm d} t^\prime, \nonumber \\
& = \int_{k \tau}^t \left[ VI^\prime - P_{\tau}(VI^\prime)\right] \, {\rm d} t^\prime.
\end{align}
From here we see that the magnitude of the second corrector can be bounded as
\begin{align}
|\wt{Q}(t, x)| \leq 2 \tau P_{\tau}(|VI^\prime|). 
\end{align}
Furthermore, the $\mathscr{L}^2$ measure of the support of $\wt{Q}$ is $$\sim \lambda \times \frac{1}{\lambda} \sim 1.$$

\subsection{The leading order term in $P_{\tau}(VI^\prime)$}
\label{subsection: leading order term in P tau}
Using the time average lemma stated in the hand-written notes, we can estimate the leading order timer in $P_{\tau}(VI^\prime)$ upto certain errors. I plan to add this lemma sometime soon.
\begin{align}
P_{\tau}(VI^\prime) = L + errors,
\end{align}
where 
\begin{align}
L & \coloneqq U_0^2  \left(\frac{\nabla \ol{a}_i^2(x) \cdot e_i}{\ol{a}_i^2(x)}\right) \frac{1}{4 \lambda} \frac{1}{t_p} \frac{1}{\mu(x)} \, \wt{\phi}^2(x) \, e_i, \nonumber \\
& =  U_0^2  \left(\nabla \ol{a}_i^2(x) \cdot (e_i \otimes e_i)\right) \frac{1}{4 \lambda} \frac{1}{t_p} \frac{1}{\mu_0} \, \wt{\phi}^2(x) ,
\end{align}
where $t_p$ is the time period given by
\begin{align}
t_p = \int_0^{c \lambda} \frac{d s}{\mu(x_s + s e_i)}.
\end{align}
Here, $1 \leq c \leq \sqrt{5}$ is a constant and depends on the slope of the direction $e_i$. An estimate on $t_p$ gives
\begin{align}
t_p \leq \frac{2 c \lambda}{\mu_0} \left(\norm{ R_n }_{L^\infty_t L^1_x} + \frac{\norm{ R_n }_{C^1_{t, x}}}{\lambda} \right).
\end{align}

\subsection{Cancelling the error}
To cancel the error, we want the following condition
\begin{align}
\int_{\mathbb{T}^2} U_0^2  \frac{1}{4 \lambda} \frac{1}{t_p} \frac{1}{\mu_0} \, \wt{\phi}^2(x) \, {\rm d} x = 1,
\end{align}
which gives
\begin{align}
U_0 \lesssim \lambda \left(\norm{ R_n }_{L^\infty_t L^1_x} + \frac{\norm{ R_n }_{C^1_{t, x}}}{\lambda}\right)^{\frac{1}{2}}.
\end{align}
Finally, we will be putting the residue in the error which gives
\begin{align}
\norm{\div^{-1} \left[L - \div(a_i^2(x) e_i \otimes e_i)\right]}_{L^\infty_t L^1_x} \leq \frac{\norm{ R_n }_{C^1_{t, x}}}{\lambda}.
\end{align}





\subsection{The time derivative of the principal part}
\label{subsection: time derivative principal part}
In this subsection, $\mu$, $r^\perp$ and $r^\parallel$ would automatically mean $\mu(p(t))$, $r^\perp(p(t))$ and $r^\parallel(p(t))$, unless we specifically add `$0$' in the subscript. We first recall,
\begin{align}
W^{(p)}_i(x) = U_0 \, \ol{\psi}(t, x) \, \ol{\phi}(t, x) \, \ol{\zeta}(t) e_i = U_0 \left(\frac{1}{r^{\perp} \, r^{\parallel}}\right)^{\frac{1}{2}} \psi\left(\frac{\lambda (x - p(t)) \cdot e_i}{r^{\parallel}}\right) \phi\left(\frac{\lambda (x - x_s) \cdot e^\perp_i}{r^{\perp}}\right) \ol{\zeta}(t) e_i \nonumber
\end{align}
Then the time derivative is given by
\begin{align}
\partial_t W^{(p)}_i(x) = T_1 + T_2 + T_3 + T_4 + T_5.
\end{align}
Next, we list all of these five terms one-by-one. 

The first term is
\begin{align}
T_1 = U_0  \left(\frac{1}{r^{\perp} \, r^{\parallel}}\right)^{\frac{1}{2}} \left(-\frac{\lambda \mu(p(t))}{r^\parallel}\right) \psi^\prime(\dots) \phi(\dots) \ol{\zeta} e_i = \div(A_1),
\end{align}
where 
\begin{align}
A_1 = U_0  \left(\frac{1}{r^{\perp} \, r^{\parallel}}\right)^{\frac{1}{2}} \left(-\frac{\lambda \mu(p(t))}{r^\parallel}\right) M_1
\end{align}
and the matrix $M_1$ is given by
\begin{align}
M_1 = 
\begin{bmatrix}
0 && \frac{r^\perp}{\lambda} \psi^\prime(\dots) \Phi^{\prime \prime \prime}(\dots) \, e_i \otimes e^\perp_i \\[10pt]
\frac{r^\perp}{\lambda} \psi^{\prime}(\dots) \Phi^{\prime \prime \prime}(\dots) \, e^\perp_i \otimes e_i && -\frac{(r^\perp)^2}{\lambda r^\parallel} \psi^{\prime \prime}(\dots) \Phi^{ \prime \prime}(\dots) \, e^\perp_i \otimes e^\perp_i
\end{bmatrix}.
\end{align}


The second term is
\begin{align}
T_2 = U_0 \mu \left(\frac{1}{r^{\perp} \, r^{\parallel}}\right)^{\frac{1}{2}} \left(-\frac{\nabla \ol{a}_i^2(p(t)) \cdot e_i}{\ol{a}_i^2(p(t))}\right) \psi(\dots) \phi(\dots) \ol{\zeta} e_i = \div(A_2),
\end{align}
where 
\begin{align}
A_2 = U_0 \mu \left(\frac{1}{r^{\perp} \, r^{\parallel}}\right)^{\frac{1}{2}} \left(-\frac{\nabla \ol{a}_i^2(p(t)) \cdot e_i}{\ol{a}_i^2(p(t))}\right) \ol{\zeta} M_2
\end{align}
and the matrix $M_2$ is given by
\begin{align}
M_2 = 
\begin{bmatrix}
0 && \frac{r^\perp}{\lambda} \psi(\dots) \Phi^{\prime \prime \prime}(\dots) \, e_i \otimes e^\perp_i \\[10pt]
\frac{r^\perp}{\lambda} \psi(\dots) \Phi^{\prime \prime \prime}(\dots) \, e^\perp_i \otimes e_i && -\frac{(r^\perp)^2}{\lambda r^\parallel} \psi^\prime(\dots) \Phi^{ \prime \prime}(\dots) \, e^\perp_i \otimes e^\perp_i
\end{bmatrix}.
\end{align}


The third term is
\begin{align}
T_3 = U_0 \mu \left(\frac{1}{r^{\perp} \, r^{\parallel}}\right)^{\frac{1}{2}} \left[\frac{\lambda (x - p(t)) \cdot e_i}{r^{\parallel}}\right] \left(-\frac{\nabla \ol{a}_i^2(p(t)) \cdot e_i}{\ol{a}_i^2(p(t))}\right) \psi^\prime(\dots) \phi(\dots) \ol{\zeta} e_i = \div(A_3),
\end{align}
where 
\begin{align}
A_3 = U_0 \mu \left(\frac{1}{r^{\perp} \, r^{\parallel}}\right)^{\frac{1}{2}} \left(-\frac{\nabla \ol{a}_i^2(p(t)) \cdot e_i}{\ol{a}_i^2(p(t))}\right) \ol{\zeta} M_3
\end{align}
and the matrix $M_3$ is given by
\begin{align}
M_3 = 
\begin{bmatrix}
0 && \frac{r^\perp}{\lambda} (x \psi)(\dots) \Phi^{\prime \prime \prime}(\dots) \, e_i \otimes e^\perp_i \\[10pt]
\frac{r^\perp}{\lambda} ( x \psi)(\dots) \Phi^{\prime \prime \prime}(\dots) \, e^\perp_i \otimes e_i && -\frac{(r^\perp)^2}{\lambda r^\parallel} (x \psi)^\prime(\dots) \Phi^{ \prime \prime}(\dots) \, e^\perp_i \otimes e^\perp_i
\end{bmatrix}.
\end{align}
Here, $(x \psi) (\dots)$ mean to represent $$\left[\frac{\lambda (x - p(t)) \cdot e_i}{r^{\parallel}}\right] \psi \left(\frac{\lambda (x - p(t)) \cdot e_i}{r^{\parallel}}\right).$$





The fourth term is given by
\begin{align}
T_4 = U_0 \mu \left(\frac{1}{r^{\perp} \, r^{\parallel}}\right)^{\frac{1}{2}} \left[\frac{\lambda (x - x_s) \cdot e^\perp_i}{r^{\perp}}\right] \left(-\frac{\nabla \ol{a}_i^2(p(t)) \cdot e_i}{\ol{a}_i^2(p(t))}\right) \psi(\dots) \phi^\prime(\dots) \ol{\zeta} e_i = \div(A_4),
\end{align}
where 
\begin{align}
A_4 = U_0 \mu \left(\frac{1}{r^{\perp} \, r^{\parallel}}\right)^{\frac{1}{2}} \left(-\frac{\nabla \ol{a}_i^2(p(t)) \cdot e_i}{\ol{a}_i^2(p(t))}\right) \ol{\zeta} M_4
\end{align}
and the matrix $M_4$ is given by
\begin{align}
M_4 = 
\begin{bmatrix}
0 && \frac{r^\perp}{\lambda} \psi(\dots) (x \phi - \Phi^{\prime \prime \prime})(\dots) \, e_i \otimes e^\perp_i \\[10pt]
\frac{r^\perp}{\lambda} \psi(\dots) (x \phi - \Phi^{\prime \prime \prime})(\dots) \, e^\perp_i \otimes e_i && -\frac{(r^\perp)^2}{\lambda r^\parallel} \psi^\prime(\dots) (x \Phi^{\prime \prime \prime} - \Phi^{\prime \prime \prime} - \Phi^{\prime \prime})(\dots) \, e^\perp_i \otimes e^\perp_i
\end{bmatrix}.
\end{align}




The fifth term is
\begin{align}
T_5 = U_0 \left(\frac{1}{r^{\perp} \, r^{\parallel}}\right)^{\frac{1}{2}} \left(\frac{1}{\tau/4}\right) \psi(\dots) \phi(\dots) \dot{\ol{\zeta}} e_i = \div(A_2),
\end{align}
where 
\begin{align}
A_5 = U_0 \left(\frac{1}{r^{\perp} \, r^{\parallel}}\right)^{\frac{1}{2}} \left(\frac{1}{\tau/4}\right) \dot{\ol{\zeta}} M_5
\end{align}
and the matrix $M_5$ is given by
\begin{align}
M_5 = 
\begin{bmatrix}
0 && \frac{r^\perp}{\lambda} \psi(\dots) \Phi^{\prime \prime \prime}(\dots) \, e_i \otimes e^\perp_i \\[10pt]
\frac{r^\perp}{\lambda} \psi(\dots) \Phi^{\prime \prime \prime}(\dots) \, e^\perp_i \otimes e_i && -\frac{(r^\perp)^2}{\lambda r^\parallel} \psi^\prime(\dots) \Phi^{ \prime \prime}(\dots) \, e^\perp_i \otimes e^\perp_i
\end{bmatrix}.
\end{align}

\subsection{$L^1$-norm of term A}
We define our term $A$ to be
\begin{align}
A = A_1 + A_2 + A_3 + A_4 + A_5.
\end{align}
A straightforward computation shows
\begin{align}
\norm{A}_{L^\infty_t L^1_x} \leq \norm{R_n}_{L^\infty_t L^1_x}^{\frac{1}{2}} \frac{\mu_0}{\lambda} \frac{(r^\perp_0)^{3/2}}{(r^\parallel)^{1/2}} \; + \; 
\frac{\norm{R_n}_{C^1_{t, x}} \norm{R_n}_{L^\infty_t L^\infty_x}}{\norm{R_n}_{L^\infty_t L^1_x}^{\frac{1}{2}}}
\frac{\mu_0}{\lambda^2} (r^\perp_0)^{3/2}(r^\parallel)^{1/2} + \nonumber \\ \norm{R_n}_{L^\infty_t L^1_x}^{\frac{1}{2}} \norm{R_n}^2_{L^\infty_t L^\infty_x} \frac{1}{\tau \lambda^2} (r^\perp_0)^{3/2}(r^\parallel)^{1/2}. 
\end{align}
In this expression the dominating term is supposed to be only the first term on the right hand side.

==> Figures/Old_Material/Anuj_Notes/Putting_everything_togather.tex <==
\section{Putting everything to gather}

\subsection{List of Parameters}

\begin{enumerate}[label = (\roman*)]
\item $\lambda \to$ Frequency parameter
\item $\ell \to$ Mollification parameter
\item $\delta \to$ Parameter for the error magnitude
\item $r^\Par_\Naught \to$ Length of the building block
\item $r^\Per_\Naught \to$ Width of the building block
\item $\tau \to$ Time parameter
\item $\mu_0 \to$ Speed Parameter
\end{enumerate} 

At the $n$th iteration, we assume the following relation
\begin{align}
\ell = \frac{1}{\lambda_{n+1}^\gamma}, \qquad \delta_{n} = \frac{1}{\lambda_n^\beta}, \qquad r^\Par_{\Naught, n} = \frac{1}{\lambda_n^a}, \qquad  r^\Per_{\Naught, n} = \frac{1}{\lambda_n^b}, \qquad \tau = \frac{1}{\lambda_n^c}, \qquad \mu_{0, n} = \lambda_n^d, \qquad \lambda_{n+1} = \lambda_n^\sigma 
\end{align}

At every iteration, we will require
\begin{align}
&\norm{ R_n }_{L^\infty_t L^1_x} \leq \delta_{n+1} = \frac{1}{\lambda_{n+1}^\beta}. \\[5pt]
&\norm{ u_n }_{C^1_{t, x}} \leq \lambda_{n+1}^{\alpha_1}. \\[5pt]
&\norm{ u_n }_{C^2_{t, x}} \leq \lambda_{n+1}^{\alpha_2}. 
\end{align}

\subsection{Magnitude of various norms}
\begin{enumerate}[label = (\roman*)]
\item \underline{$L^2$-norm of the principal part of perturbation}
\begin{align}
\norm{w^{(p)}_{n+1}}_{L^\infty_t L^2_x} \lesssim \norm{ R_n }_{L^\infty_t L^1_x}^{\frac{1}{2}} \leq \delta_{n+1}^{1/2} = \frac{1}{\lambda_{n+1}^{\beta/2}}.
\end{align}
Requirement:
\begin{align}
\beta > 0.
\end{align}
\item \underline{$L^2$-norm of the divergence correction}
\begin{align}
\norm{w^{(p)}_{n+1}}_{L^\infty_t L^2_x} \lesssim \frac{r^\Per_{\Naught, n+1}}{r^\Par_{\Naught, n+1}} \norm{ R_n }_{L^\infty_t L^1_x}^{\frac{1}{2}} \leq \frac{r^\Per_{\Naught, n+1}}{r^\Par_{\Naught, n+1}} \delta_{n+1}^{1/2} = \frac{1}{\lambda_{n+1}^{\beta/2 + b - a}}.
\end{align}
Requirement:
\begin{align}
\beta + 2b > a.
\end{align}
\item \underline{$L^2$-norm of the first corrector}
\begin{align}
\norm{\ol{w}^{(t)}_{n+1}}_{L^\infty_t L^2_x} \lesssim \norm{ R_n }_{L^\infty_t L^1_x} \frac{1}{\mu_{0, n+1}} \left(\frac{1}{r^\Par_{\Naught, n+1}} \frac{1}{r^\Per_{\Naught, n+1}}\right)^{\frac{1}{2}} \lesssim \frac{1}{\lambda_{n+1}^{\beta + d - a/2 - b/2}}.
\end{align}
Requirement:
\begin{align}
2 \beta + 2 d > a + b.
\end{align}
\item \underline{$L^2$-norm of the second corrector}
\begin{align}
\norm{\wt{w}^{(t)}_{n+1}}_{L^\infty_t L^2_x} \lesssim \norm{ R_{\ell} }_{C^1_{t, x}} \tau_{n+1} \lesssim \frac{\tau_{n+1}}{\ell^3} \lesssim \frac{1}{\lambda_{n+1}^{c - 3 \gamma}}.
\end{align}
Requirement:
\begin{align}
c > 3 \gamma.
\end{align}

\item \underline{$L^2$-norm of the velocity from mollification}
\begin{align}
\norm{u_n - u_{\ell}}_{L^\infty_t L^2_x} \leq \ell \norm{u_n}_{C^1_{t, x}} \leq \frac{1}{\lambda_{n+1}^{\gamma - \alpha_1}}
\end{align}
Requirement:
\begin{align}
\gamma > \alpha_1.
\end{align}


\item \underline{$L^p$-norm of the principal part of vorticity}
\begin{align}
\norm{D w^{(p)}_{n+1}}_{L^\infty_t L^2_x} & \lesssim \frac{\norm{ R_n }_{L^\infty_t L^1_x}^{\frac{1}{2}}}{{\delta_{n+1}}^{(2-2/p)}} \;  \frac{1}{(r^\Per_{\Naught, n+1})^{(3/2-1/p)}} \frac{1}{(r^\Par_{\Naught, n+1})^{(1/2-1/p)}} \nonumber \\
& \lesssim \frac{1}{\lambda_{n+1}^{\beta(2/p - 3/2) - b(3/2 - 1/p) - a (1/2 - 1/p)}}.
\end{align}
Requirement:
\begin{align}
& \beta \left(\frac{2}{p} - \frac{3}{2}\right) - b \left( \frac{3}{2} - \frac{1}{p}\right) - a \left( \frac{1}{2} - \frac{1}{p}\right) > 0 \nonumber \\
& \implies p < \frac{2 (2 \beta + b + a)}{3 \beta + 3b + a}.
\end{align}

\item \underline{$L^p$-norm of the divergence correction}
Same as above but only a bit smaller.


\item \underline{$L^p$-norm of the first corrector vorticity}
\begin{align}
\norm{D \ol{w}^{(t)}_{n+1}}_{L^\infty_t L^2_x} & \lesssim \frac{\norm{ R_n }_{L^\infty_t L^1_x}}{{\delta_{n+1}}^{(2-2/p)}} \; \frac{1}{\mu_{0, n+1}} \frac{1}{(r^\Per_{\Naught, n+1})^{(2-1/p)}} \frac{1}{(r^\Par_{\Naught, n+1})^{(1-1/p)}} \nonumber \\
& \lesssim \frac{1}{\lambda_{n+1}^{\beta(2/p - 1) + d + b(  1/p - 2) + a (1/p - 1)}}.
\end{align}
Requirement:
\begin{align}
& \beta \left(\frac{2}{p} - 1\right) + d + b \left( \frac{1}{p} - 2\right) + a \left(  \frac{1}{p} - 1\right) > 0 \nonumber \\
& \implies p < \frac{ 2 \beta + b + a}{\beta + 2b + a - d}.
\end{align}

\item \underline{$L^p$-norm of the second corrector vorticity}
\begin{align}
\norm{\wt{w}^{(t)}_{n+1}}_{L^\infty_t L^2_x} \lesssim \norm{ R_{\ell} }_{C^1_{t, x}} \tau_{n+1} \lambda_{n+1} \lesssim \frac{\tau_{n+1} \lambda_{n+1}}{\ell^3} \lesssim \frac{1}{\lambda_{n+1}^{c - 3 \gamma - 1}}.
\end{align}
Requirement:
\begin{align}
c > 3 \gamma + 1.
\end{align}


\item \underline{$L^p$-norm of the vorticity from mollification}
\begin{align}
\norm{D u_n - D u_{\ell}}_{L^\infty_t L^p_x} \leq \ell \norm{u_n}_{C^2_{t, x}} \leq \frac{1}{\lambda_{n+1}^{\gamma - \alpha_2}}
\end{align}
Requirement:
\begin{align}
\gamma > \alpha_2.
\end{align}
\end{enumerate} 




\subsection{Error estimates}

\begin{enumerate}[label = (\roman*)]
\item \underline{Error from mollification}
\begin{align}
\frac{1}{\delta_{n+2}}\norm{u_{\ell} \otimes u_{\ell} - (u_n \otimes u_n)_{\ell}}_{L^\infty_t L^1_x} & \leq \frac{1}{\delta_{n+2}} \ell \norm{u_n}^2_{C^1_{t, x}} \nonumber \\
& \leq \lambda_{n+1}^{\beta \sigma} \frac{1}{\lambda_{n+1}^\gamma} \lambda_{n+1}^{2 \alpha_1}
\end{align}
Requirement:
\begin{align}
\gamma > \beta \sigma + 2 \alpha_1.
\end{align}



\item \underline{Error when the time derivative hits cutoff in first corrector}
\begin{align}
\frac{1}{\delta_{n+2}} \norm{ \div^{-1} V }_{L^\infty_t L^1_x} & \leq \frac{1}{\delta_{n+2}} \frac{\norm{ R_n }_{L^\infty_{t, x} } \norm{ R_n }_{L^\infty_t L^1_x}}{\mu_{0, n+1} \, \tau_{n+1}}. \nonumber \\
& \leq \lambda_{n+1}^{\beta \sigma} \frac{\delta_{n+1}^2}{\ell^2} \frac{1}{\lambda_{n+1}^d} \lambda_{n+1}^{c} \nonumber \\
& \leq \lambda_{n+1}^{\beta \sigma} \frac{\lambda_{n+1}^{2 \gamma}}{\lambda_{n+1}^{2 \beta}} \frac{1}{\lambda_{n+1}^d} \lambda_{n+1}^{c}
\end{align}
Requirement:
\begin{align}
d + 2 \beta > c + \beta \sigma + 2 \gamma.
\end{align}


\item \underline{Average of three terms in first corrector when time derivative hits $r^\Per$ and $r^\Par$ minus the buidling} \underline{block term of length $1/\lambda$}
\begin{align}
\frac{1}{\delta_{n+2}} \norm{ \div^{-1} (II + III + IV - VI) }_{L^\infty_t L^1_x} & \leq \frac{1}{\delta_{n+2}} \frac{\norm{ R_n }_{C^1_{t, x}}}{\lambda_{n+1}} \nonumber \\
& \leq \lambda_{n+1}^{\beta \sigma} \frac{\delta_{n+1}}{\ell^3} \frac{1}{\lambda_{n+1}}  \nonumber \\
& \leq \lambda_{n+1}^{\beta \sigma} \frac{\lambda_{n+1}^{3 \gamma}}{\lambda_{n+1}^{ \beta}} \frac{1}{\lambda_{n+1}} 
\end{align}
Requirement:
\begin{align}
1 + \beta > \beta \sigma + 3 \gamma.
\end{align}


\item \underline{$P_\tau$ minus leading order term: Error 1}
\begin{align}
\frac{1}{\delta_{n+2}} \norm{ P_\tau - L }_{L^\infty_t L^1_x} & \leq \frac{1}{\delta_{n+2}} \frac{\norm{ R_n }_{C^1_{t, x}} \norm{ R_n }_{L^\infty_{t, x}} }{\delta_{n+1}} \frac{\lambda_{n+1}}{\mu_{0, n+1}}\nonumber \\
& \leq \frac{1}{\delta_{n+2}} \frac{\delta_{n+1} }{\ell^5} \frac{\lambda_{n+1}}{\lambda_{n+1}^d}  \nonumber \\
& \leq \lambda_{n+1}^{\beta \sigma} \frac{\lambda_{n+1}^{5 \gamma}}{\lambda_{n+1}^{ \beta}} \frac{\lambda_{n+1}}{\lambda_{n+1}^d} 
\end{align}
Requirement:
\begin{align}
d + \beta > 1 + \beta \sigma + 5 \gamma.
\end{align}



\item \underline{$P_\tau$ minus leading order term: Error 2}
\begin{align}
\frac{1}{\delta_{n+2}} \norm{ P_\tau - L }_{L^\infty_t L^1_x} & \leq \frac{1}{\delta_{n+2}} \norm{ R_n }_{C^2_{t, x}}  \frac{1}{\delta_{n+1}}\frac{1}{\lambda_{n+1}}\nonumber \\
& \leq \frac{1}{\delta_{n+2}} \frac{1}{\ell^4} \frac{1}{\lambda_{n+1}}  \nonumber \\
& \leq \lambda_{n+1}^{\beta \sigma} \lambda_{n+1}^{4 \gamma}  \frac{1}{\lambda_{n+1}}
\end{align}
Requirement:
\begin{align}
1 > 4 \gamma + \beta \sigma.
\end{align}


\item \underline{Extra Condition: $P_\tau$ minus leading order term: Error 2}
The last requirement holds under the condition
\begin{align}
\frac{ \norm{ R_n }_{C^1_{t, x}} }{\lambda_{n+1}} \leq  \norm{ R_n }_{L^\infty_t L^1_{x}}
 \end{align}
which is satisfied if the last requirement is satisfied.


\item \underline{$\norm{A}_{L^\infty_t L^1_x}$: Error 1} \\
Requirement:
\begin{align}
\frac{3}{2} b + \frac{\beta}{2} > d + \frac{a}{2} + \beta \sigma
\end{align}

\item \underline{$\norm{A}_{L^\infty_t L^1_x}$: Error 2} \\
Requirement:
\begin{align}
\frac{3}{2} b + \frac{a}{2} + \frac{3 \beta}{2} > d + 5 \gamma + \beta \sigma
\end{align}


\item \underline{$\norm{A}_{L^\infty_t L^1_x}$: Error 3} \\
Requirement:
\begin{align}
\frac{3}{2} b + \frac{a}{2} + \frac{3 \beta}{2} > c + 4 \gamma + \beta \sigma
\end{align}


\item \underline{Linear terms: Error 1} \\
Requirement:
\begin{align}
\frac{b}{2} + \frac{a}{2} + \beta  > 2 \gamma + \beta \sigma
\end{align}


\item \underline{Linear terms: Error 2} \\
Requirement:
\begin{align}
c + \beta  > 3 \gamma + \beta \sigma
\end{align}


\item \underline{Quadratic terms: Error 1} \\
Requirement:
\begin{align}
b + \beta  > a + \beta \sigma
\end{align}

\item \underline{Quadratic terms: Error 2} \\
Requirement:
\begin{align}
d + \frac{3}{2}\beta  > \frac{a}{2} + \frac{b}{2} + \beta \sigma
\end{align}

\item \underline{Quadratic terms: Error 3} \\
Requirement:
\begin{align}
c + \frac{3}{2}\beta  > 3 \gamma + \beta \sigma
\end{align}


\item \underline{Quadratic terms: Error 4} \\
Requirement:
\begin{align}
2d + 2\beta  > a + b  + \beta \sigma
\end{align}

\item \underline{Quadratic terms: Error 5} \\
Requirement:
\begin{align}
c + d + 2\beta  > \frac{a}{2} + \frac{b}{2} + 3 \gamma + \beta \sigma
\end{align}

\item \underline{Quadratic terms: Error 6} \\
Requirement:
\begin{align}
2c + 2\beta  > 6 \gamma  + \beta \sigma
\end{align}
\end{enumerate} 





\subsection{Higher derivatives}
\begin{enumerate}[label = (\roman*)]
\item \underline{First derivative: from principal part} \\
Requirement:
\begin{align}
\alpha_1 \sigma > a + b + 2 \beta
\end{align}

\item \underline{First derivative: First corrector} \\
Requirement:
\begin{align}
\alpha_1 \sigma > a + 2b -d + \beta
\end{align}


\item \underline{First derivative: Second corrector} \\
Requirement:
\begin{align}
\alpha_1 \sigma > 1 + 3\gamma - c - \beta
\end{align}

\item \underline{Second derivative: from principal part} \\
Requirement:
\begin{align}
\alpha_2 \sigma > a + 2 b + 3 \beta
\end{align}

\item \underline{Second derivative: First corrector} \\
Requirement:
\begin{align}
\alpha_2 \sigma > a + 3b -d + 2\beta
\end{align}


\item \underline{Second derivative: Second corrector} \\
Requirement:
\begin{align}
\alpha_2 \sigma > 2 + 3\gamma - c - \beta
\end{align}
\end{enumerate}



\subsection{Other requirements}
\begin{enumerate}[label = (\roman*)]
\item \underline{} \\
Requirement:
\begin{align}
0 < \gamma < 1.
\end{align}

\item \underline{} \\
Requirement:
\begin{align}
0 < \beta
\end{align}

\item \underline{$r^\Par < 1/\lambda$ all time} \\
Requirement:
\begin{align}
a + \beta > 2 \gamma + 1
\end{align}

\item \underline{$r^\Per < 1/\lambda$ all time} \\
Requirement:
\begin{align}
b + \beta > 2 \gamma + 1
\end{align}

\item \underline{} \\
Requirement:
\begin{align}
0 < c
\end{align}


\item \underline{} \\
Requirement:
\begin{align}
0 < d
\end{align}

\item \underline{} \\
Requirement:
\begin{align}
1 < \sigma
\end{align}

\end{enumerate}





\section{Maria's notes - proof of Elia's prop 2.1
}

Setting: 
$$V= \nabla^\perp \psi = \nabla \phi$$ 
$$\psi = \frac{x_2}{x_1^2+x_2^2} = \partial_2 G, \qquad \phi = \frac{x_2}{x_1^2+x_2^2} = \partial_2 G,$$
$$EQ FOR V$$
We first rescale
$$V_\eps= \frac 1 \eps V\left(\frac x \eps\right)$$
$$\varphi_\eps = $$

Let $\xi_\alpha$ be a cutoff at scale $\eps^\alpha$. 
Define
$$\tilde p_ \eps (x) = (1-\xi_\alpha)\phi_\eps  = $$

Don't talk about support of pressure.
Later, since all other terms of the equation are compactly supported, the pressure will come compactly supported.

Moral: $Q$ is as in the previous paper, namely it is not divergence free (but small divergence). This allows to avoid the computation of Constantin which sets the average in an unuseful way for CI, and instead have ... .

==> Figures/Old_Material/Anuj_Notes/error_estimates.tex <==
\section{Error estimates}
\label{section: error estimates}
We have already obtain error estimates in \S \ref{section: def perturbation} on some of the important terms. Now, we obtain estimates some of the remaining terms.
\subsection{Linear terms}
\label{subsectino: error linear terms}
In this subsection, we are concerned with the terms
\begin{align}
\div(u_{\ell} \otimes w_{n+1}) \qquad \text{and} \qquad \div(w_{n+1} \otimes u_{\ell}).
\end{align}
As these terms will contribute to the new error, all we need to make sure is that
\begin{align}
\norm{u_{\ell} \, w_{n+1}}_{L^\infty_t L^1_x}
\end{align}
is small. We have,
\begin{align}
\norm{u_{\ell} \, w_{n+1}}_{L^\infty_t L^1_x} \leq \norm{u_{\ell} \, w^{(p)}_{n+1}}_{L^\infty_t L^1_x} + \norm{u_{\ell} \, w^{(c)}_{n+1}}_{L^\infty_t L^1_x} +
\norm{u_{\ell} \, \ol{w}^{(t)}_{n+1}}_{L^\infty_t L^1_x} +
\norm{u_{\ell} \, \wt{w}^{(p)}_{n+1}}_{L^\infty_t L^1_x}.
\end{align}
The estimates of the first three terms are similar, so only estimate the first term and the fourth term.
\begin{align}
\norm{u_{\ell} \, w^{(p)}_{n+1}}_{L^\infty_t L^1_x} & \leq \norm{u_{\ell} }_{L^\infty_t L^\infty_x} \norm{ w^{(p)}_{n+1}}_{L^\infty_t L^1_x} \nonumber \\
& \leq \sup_t \left(\frac{r^\perp(p(t)) r^\parallel(p(t))}{\lambda^2}\right)^{\frac{1}{2}}\norm{u_{\ell} }_{L^\infty_t L^\infty_x} \norm{ w^{(p)}_{n+1}}_{L^\infty_t L^2_x} \nonumber \\
& \leq \norm{R_n}_{L^\infty_t L^1_x} \norm{u_{\ell} }_{L^\infty_t L^\infty_x} \norm{ w_{n+1}}_{L^\infty_t L^2_x} \frac{\left(r^\perp_0 r^\parallel_0\right)^{\frac{1}{2}}}{\lambda}.
\end{align}
For the fourth term, we have
\begin{align}
\norm{u_{\ell} \, \wt{w}^{(p)}_{n+1}}_{L^\infty_t L^1_x} & \leq \norm{u_{\ell} }_{L^\infty_t L^2_x} \norm{ \wt{w}^{(p)}_{n+1}}_{L^\infty_t L^\infty_x} \nonumber \\
& \leq \norm{ \wt{w}^{(p)}_{n+1}}_{L^\infty_t L^\infty_x}  \nonumber \\
& \leq \norm{R_n}_{C^1_{t, x}} \, \tau.
\end{align}

\subsection{Quadratic terms}
We have already completed the analysis of
\begin{align}
\div(w^{(p)}_{n+1} \otimes w^{(p)}_{n+1}) + \div(R_l).
\end{align}
Next, we deal with the terms
\begin{enumerate}[label = (\roman*)]
    \item $\div(w^{(p)}_{n+1} \otimes w^{(c)}_{n+1}) $ 
    \item $\div(w^{(p)}_{n+1} \otimes \ol{w}^{(t)}_{n+1}) $ 
    \item $\div(w^{(p)}_{n+1} \otimes \wt{w}^{(t)}_{n+1}) $ 
    \item $\div(w^{(c)}_{n+1} \otimes w^{(c)}_{n+1}) $ 
    \item $\div(w^{(c)}_{n+1} \otimes \ol{w}^{(t)}_{n+1}) $ 
    \item $\div(w^{(c)}_{n+1} \otimes \wt{w}^{(t)}_{n+1}) $ 
    \item $\div(\ol{w}^{(t)}_{n+1} \otimes \ol{w}^{(t)}_{n+1}) $
    \item $\div(\ol{w}^{(t)}_{n+1} \otimes \wt{w}^{(t)}_{n+1}) $
    \item $\div(\wt{w}^{(t)}_{n+1} \otimes \wt{w}^{(t)}_{n+1}) $
\end{enumerate}
plus six more similar terms (therefore omitted). We see that
\begin{align}
\norm{w^{(p)}_{n+1} \otimes w^{(c)}_{n+1}}_{L^\infty_t L^1_x} & \leq \norm{w^{(p)}_{n+1} }_{L^\infty_t L^2_x} \norm{w^{(c)}_{n+1}}_{L^\infty_t L^2_x}, \nonumber \\
& \leq \frac{r^\perp_0}{r^\parallel_0} \norm{w^{(p)}_{n+1} }^2_{L^\infty_t L^2_x}, \nonumber \\
& \leq \norm{R_n}_{L^\infty_t L^1_x} \, \frac{r^\perp_0}{r^\parallel_0}
\end{align}

\begin{align}
\norm{w^{(p)}_{n+1} \otimes \ol{w}^{(t)}_{n+1}}_{L^\infty_t L^1_x} & \leq \norm{w^{(p)}_{n+1} }_{L^\infty_t L^2_x} \norm{\ol{w}^{(t)}_{n+1}}_{L^\infty_t L^2_x}, \nonumber \\
& \leq \norm{ R_n }^{\frac{3}{2}}_{L^\infty_t L^1_x} \frac{\lambda}{\mu_0} \left(\frac{1}{r^\parallel_0} \frac{1}{r^\perp_0}\right)^{\frac{1}{2}}
\end{align}

\begin{align}
\norm{w^{(p)}_{n+1} \otimes \wt{w}^{(t)}_{n+1}}_{L^\infty_t L^1_x} & \leq \norm{w^{(p)}_{n+1} }_{L^\infty_t L^2_x} \norm{\wt{w}^{(t)}_{n+1}}_{L^\infty_t L^2_x}, \nonumber \\
& \leq \norm{ R_n }^{\frac{1}{2}}_{L^\infty_t L^1_x} \, \norm{ R_n }_{C^1_{t, x}} \, \tau
\end{align}
Since the $L^2$-norm of $w^{(c)}_{n+1}$ is smaller than $w^{(p)}_{n+1}$, we do not compute rest of the terms involving $w^{(c)}_{n+1}$.


\begin{align}
\norm{\ol{w}^{(t)}_{n+1} \otimes \ol{w}^{(t)}_{n+1}}_{L^\infty_t L^1_x} & \leq \norm{\ol{w}^{(t)}_{n+1} }^2_{L^\infty_t L^2_x}, \nonumber \\
& \leq \norm{ R_n }^{2}_{L^\infty_t L^1_x} \left(\frac{\lambda}{\mu_0} \right)^2 \left(\frac{1}{r^\parallel_0} \frac{1}{r^\perp_0}\right)
\end{align}

\begin{align}
\norm{\ol{w}^{(t)}_{n+1} \otimes \wt{w}^{(t)}_{n+1}}_{L^\infty_t L^1_x} & \leq \norm{\ol{w}^{(t)}_{n+1} }_{L^\infty_t L^2_x} \norm{\wt{w}^{(t)}_{n+1}}_{L^\infty_t L^2_x}, \nonumber \\
& \leq \norm{ R_n }_{L^\infty_t L^1_x} \norm{ R_n }_{C^1_{t, x}} \frac{\lambda}{\mu_0} \left(\frac{1}{r^\parallel_0} \frac{1}{r^\perp_0}\right)^{\frac{1}{2}} \, \tau
\end{align}

The final term is 
\begin{align}
\norm{\wt{w}^{(t)}_{n+1} \otimes \wt{w}^{(t)}_{n+1}}_{L^\infty_t L^1_x} & \leq \norm{\wt{w}^{(t)}_{n+1} }^2_{L^\infty_t L^2_x}, \nonumber \\
& \leq \norm{ R_n }^{2}_{C^1_{t,x}} \tau^2
\end{align}

==> Figures/Old_Material/Anuj_Notes/issue.tex <==
\section{A New Issue: January 20}
A scale separation needs to be less than two, $\sigma < 2$ because of $W^c \otimes W^c$, where $W^c$ is the divergence corrector to the principal part of the perturbation.
\begin{align}
\norm{W^{(c)}_{n+1} \otimes W^{(c)}_{n+1}}_{L^\infty_t L^1_x} & \leq \norm{R_n}_{L^\infty_t L^1_x} \, \frac{r^\perp_0}{r^\parallel_0}.
\end{align}
We want this term to be smaller than $\delta_{n+2}$, which means
\begin{align}
\delta_{n+1} \frac{r^\perp_0}{r^\parallel_0} < \delta_{n+2}.
\end{align}
From the vorticity estimate, we get
\begin{align}
\delta^2_{n+1} < \delta_{n+2}.
\end{align}
This implies that the scale separation needs to be less than 2.

\section{A Main Issue}
We out line the main issue regarding the scale separation. Suppose, we require
$$\norm{R_n}_{L^\infty_t L^1_x} \leq \delta_{n+1}.$$

Let us consider the three dominating term that we have been talking about for a while. The estimate on the vorticity in the principal part of perturbation measured in $L^1$ is given by
\begin{align}
\norm{D W_i^{(p)}}_{L^\infty_t L^1_x} \leq \norm{ R_n }_{L^\infty_t L^1_x}^{\frac{1}{2}}  \left(\frac{r^\parallel_0}{r^\perp_0}\right)^{\frac{1}{2}} < 1.
\end{align}
The estimate on the vorticity in the first corrector  measured in $L^1$ is given by
\begin{align}
\norm{D \ol{Q}_i}_{L^\infty_t L^1_x} \leq \norm{ R_n }_{L^\infty_t L^1_x} \; \frac{1}{\mu_0} \frac{1}{r^\perp_0} < 1
\end{align}
Finally, the error contribution from term $A$ is given by
\begin{align}
\norm{A}_{L^\infty_t L^1_x} \leq \norm{R_n}_{L^\infty_t L^1_x}^{\frac{1}{2}} \mu_0\frac{(r^\perp_0)^{3/2}}{(r^\parallel)^{1/2}}  < \delta_{n+2}.
\end{align}
Multiplying all three gives us that for the convex integration scheme to close, we need
\begin{align}
\norm{R_n}_{L^\infty_t L^1_x}^2 \leq \delta_{n+2} 
\end{align}
or we can rewrite it as
\begin{align}
\delta_{n+1}^2 \leq \delta_{n+2}. 
\end{align}
This is something reasonable to expect. Therefore, the convex integration scheme closes when $p = 1$. But the issue arise when we want to go beyond $p = 1$. Since, it is the error in the vorticity that will be helping us to go beyond $p = 1$, we need to have something like
\begin{align}
\delta_n = \frac{1}{\lambda_n^\beta.}
\end{align}
If the error decreases, slower than the power-law of the length scale ($1/\lambda_n$), we will not be able to go beyond $p = 1$. Next, assume that the $\sigma$ is the parameter governing the scale separation, i.e.,
\begin{align}
\lambda_{n+1} = \lambda_n^\sigma.
\end{align}
Therefore, the condition
\begin{align}
\delta_{n+1}^2 \leq \delta_{n+2}. 
\end{align}
implies that 
\begin{align}
\sigma < 2,
\end{align}
i.e., we cannot have large scale separation. This causes problems in controlling the error terms containing derivatives. Consider, for example, the leading order term from $P_\tau$ of building block (of size $\frac{1}{20 \lambda_{n+1}}$)
\begin{align}
L =  \left(\nabla \ol{a}_i^2(x) \cdot (e_i \otimes e_i)\right)  \wt{\phi}^2(x) ,
\end{align}
This term is used in canceling the error of the form
\begin{align}
- \div(R_n) = \left(\sum_{i=1}^4 \nabla a_i^2(t, x)  e_i\right) + \nabla P
\end{align}
 which gives
\begin{align}
\norm{\div^{-1} \left[L + \div(R_n)\right]}_{L^\infty_t L^1_x} \leq \frac{\norm{ R_n }_{C^2_{t, x}}}{\lambda_{n+1}}.
\end{align}
Next, we want 
\begin{align}
\frac{\norm{ R_n }_{C^2_{t, x}}}{\lambda_{n+1}} \leq \delta_{n+2} 
\end{align}
A crude, estimate 
\begin{align}
\norm{ R_n }_{C^2_{t, x}} \leq \lambda_{n}^2 \norm{ R_n }_{C^0_{t, x}} 
 \leq \lambda_{n}^4 \norm{ R_n }_{L^\infty_{t} L^1_x} 
\end{align}
Therefore, we want 
\begin{align}
\delta_{n+1} \lambda_{n}^4  \frac{1}{\lambda_{n+1}} \leq \delta_{n+2},
\end{align}
which after relaxing a bit 
\begin{align}
\lambda_{n}^4  \frac{1}{\lambda_{n+1}} \leq 1,
\end{align}
This implies
\begin{align}
\sigma > 4.
\end{align}
This condition is at odds with the requirement $\sigma < 2$.

Even if somehow had an improve estimate
\begin{align}
\norm{ R_n }_{C^2_{t, x}} \leq  
  \lambda_{n}^2 \norm{ R_n }_{L^\infty_{t} L^1_x}, 
\end{align}
even then it is a problem. 
In conclusion, we can ask to the error to decrease at a slow pace, for example, a logarithmic decrease
\begin{align}
\delta_{n} = \frac{1}{\log (\lambda_n)}
\end{align}
but not as a power-law
\begin{align}
\delta_n = \frac{1}{\lambda_n^\beta},
\end{align}
which then creates problem going beyond $p = 1$.

==> Figures/Old_Material/Anuj_Notes/modified_def_pert.tex <==

\section{Maria's notes}
For introduction:

Novelties in CI: 

No periodicity of BB. Corresponds to a gain in $L^p$ norms, $p<\infty$.

New BB, relation with old $Q$






\section{Definition of Perturbation}
\label{section: def perturbation}
The defintion of the perturbation is
\begin{align}
w_{n+1} = u_{n+1} - u_{\ell} = w_{n+1}^{(p)} + w_{n+1}^{(c)} + \ol{w}_{n+1}^{(t)} + \wt{w}_{n+1}^{(c)}
\end{align}
\begin{enumerate}[label = (\roman*)]
    \item $w_{n+1}^{(p)} \to $ the principal part
    \item $w_{n+1}^{(c)} \to $ the correction part
    \item $\ol{w}_{n+1}^{(t)} \to $ the first time corrector
    \item $\wt{w}_{n+1}^{(t)} \to $ the second time corrector
\end{enumerate}

The different parts of the perturbation in the component form
\begin{align}
w_{n+1}^{(p)} = \sum_{i=1}^{4} W^{(p)}_i, \qquad w_{n+1}^{(c)} = \sum_{i=1}^{4} W^{(c)}_i,\qquad  \ol{w}_{n+1}^{(t)} = \sum_{i=1}^{4} \ol{Q}_i, \qquad \wt{w}_{n+1}^{(t)} = \sum_{i=1}^{4} \wt{Q}_i
\end{align}
\subsection{A few basic definitions}
\label{subsection: basic definitions}
Given a function $f$ defined on $[0, 1] \times \mathbb{T}^2$, we define the time average $P_\tau$ as
\begin{align}
\left[P_{\tau}(f)\right](x) = \frac{1}{\tau} \int_{k \tau}^{(k+1) \tau} f(t, x) \, {\rm d} t
\end{align}
We let
\begin{align}
- \div(R_n) = \div\left(\sum_{i=1}^4 a_i^2(t, x) e_i \otimes e_i\right) + \nabla P
\end{align}
where $a_i$ are smooth functions and obey
\begin{align}
\inf_{t, x} |a_i^2(t, x)| \geq \norm{R_n}_{L^\infty_t L^1_x}.
\end{align}
We denote $P_\tau$ applied to coefficients $a_i^2(t, x)$ as
\begin{align}
\ol{a}_i^2(x) = P_\tau(a_i^2(t, x)).
\end{align}
Next, we define the building block speed as
\begin{align}
\mu(x) \coloneqq \frac{\mu_0}{P_\tau(a_i^2(t, x))} = \frac{\mu_0}{\ol{a}_i^2(x)}.
\end{align}

\subsection{Notation}
%\begin{align}
%\rho_\varepsilon \coloneqq \frac{1}{\varepsilon^{1/2}} \rho \left(\frac{x}{\varepsilon}\right).
%\end{align}


\subsection{The static jet}
We begin by building the profile of the jet. Let us fix parameters $r^\Per \ll r^\Par\ll 1$ and $\xi \in \mathbb{R}^2$ unitary with rationally dependent components.








Consider smooth functions $\Phi, \psi: \RR\to \RR$ supported in $(-1/2,1/2)$ are such $\int \psi^2 \, {\rm d} x = \int \phi^2 \, {\rm d}x =1$, where we set $\phi := \Phi^{\prime \prime \prime \prime}$.  We define the {\it static jet} centered at the origin $x=0$ as
\begin{align}
	W_{\xi, \, r^\Per, \, r^\Par}^p (x) := \psi_{r^\Par}(x) \, \phi_{r^\Per}(x) \, \xi \, , 
\end{align}
where $\xi^\perp:= (-\xi_2,\xi_1)$ and we use the notation
\begin{align}
	\psi_{r^\Par}(x)
	:= 
	\frac{1}{(r^{\Par})^{1/2}} \psi\left( \frac{x\cdot \xi}{r^\Par}\right)\, ,
	\quad
	\phi_{r^\Per}(x)
	:=
	\frac{1}{(r^\Per)^{1/2}}
	\phi\left( \frac{x\cdot \xi^\perp}{r^\Per}\right) \, . 
\end{align}
With a slight abuse of notation, $W^p_{\xi,r^\Per,r^\Par}(x)$ denote its $1$-periodic extension when $x\in \mathbb{T}^2$.



\subsection{Correction of the divergence}


The static jet $W_{\xi,r^\Per,r^\Par}^p$ is not divergence free:

\begin{align}
	\div(W_{\xi,r^\Per,r^\Par}^p)(x) 
	=
    \frac{1}{r^\Par} \, \psi^{\prime}_{r^\Par}(x) \, \phi_{r^\Per}(x) \, \xi
\end{align}
With the obvious notation, we define the {\it divergence corrector} as
\begin{equation}
	W_{\xi,r^\Per,r^\Par}^c(x) :=  - \frac {r^\Per}{r^\Par} \,
	\psi^{\prime}_{r^\Par} 
	 \Phi^{\prime \prime \prime}_{r^\Per}\, \xi^\perp \, .
\end{equation}
Notice that
\begin{equation}
	\div(W_{\xi,r^\Per,r^\Par}^p + W_{\xi,r^\Per,r^\Par}^c) = 0 \, .
\end{equation}

\subsection{Trajectory of the center of the building block}
The position $p(t)$ of the center of the building block solves
\begin{align}
\frac{d p(t)}{dt} = \mu(p(t)) \xi, \qquad p(0) = p_0.
\end{align}
It is clear that
\begin{align}
\dot{p}(t) = \mu(p(t)) \xi \quad \implies \quad \ddot{p}(t) = (\xi \cdot \nabla \mu (p(t))) \, \mu(p(t)) \,  \xi.
\end{align}
The orbit $p(t)$ is periodic, with period
\begin{align}
	T_\xi \coloneqq \int_0^{\wt T_\xi} \frac{1}{\mu(p(s))} \, ds = \frac{1}{\mu_0}\int_0^{\wt T_\xi} \ol{a}_i^2(p(s))\, ds
 \label{def: time period Txi}
\end{align}
where $\tilde T_\xi$ is the period associated with constant velocity $\xi$ and initial position $p_0$. We have to decide which of the following two lemmas we will be using in the end.


\begin{lemma}
	\begin{align}
		\Big| T_\xi - \wt{T}_\xi \int_{\mathbb{T}^2} \frac{1}{\mu(x)}\, dx \Big|
		\le \frac{\| \nabla a \|_{L^\infty}}{\mu_0} \, .
	\end{align}
\end{lemma}

\begin{proof}
	The trajectory $t\xi$ is $1/\tilde T_\xi$-dense...
\end{proof}


\begin{lemma}
There exists an initial condition $p_0 \in \TT^2$ such that
\begin{align}
 T_\xi = \wt{T}_\xi \int_{\mathbb{T}^2} \frac{1}{\mu(x)}\, dx  \leq \frac{\lambda}{\mu_0} \norm{R_n}_{L^\infty_t L^1_x}.
\end{align}
\end{lemma}

\begin{proof}
From the definition of $T_\xi$ in (\ref{def: time period Txi}), an integration over the torus with respect to the initial condition $p_0$ leads to
\begin{align}
\int_{\TT^2} T_\xi \, {\rm d} p_0 = \wt{T}_\xi \int_{\mathbb{T}^2} \frac{1}{\mu(x)}\, dx.
\end{align}
Therefore, there must be a desired initial condition $p_0$.
\end{proof}


\subsection{Moving Jet}
We define the time-dependent size parameters for the building block as 
\begin{align}
r^{\Per}(t) \coloneqq r^{\Per}_\Naught \; \ol{a}_i^2(p(t)), \qquad r^{\Par}(t) \coloneqq r^{\Par}_\Naught \; \ol{a}_i^2(p(t)),
\end{align}
where $r^\Per_\Naught$ and $r^\Par_\Naught$ are constants to be chosen later such that $r^\Per(t) < r^\Par(t) < 1$ for all time. Notice that 
\begin{align}
	\frac{r^\Per(t)}{r^\Par(t)} = \frac{r^\Per_\Naught}{r^\Par_\Naught} < 1 \, ,
\end{align}
is independent of time.

{\color{blue} An issue: We need to require $r^\Par(t) \leq \frac{1}{\lambda}$ at all time. This means 
\begin{align}
r^\Par_0 \leq \frac{1}{\norm{R_n}_{L^\infty_t L^\infty_x}}\frac{1}{\lambda}
\end{align}
which can be very small and may cause problems (not sure) with the scale separation.
}


\bigskip

The {\it moving jet} and its potential matrix is defined according to
\begin{align}
	&W^p_\xi(x,t):= W_{\xi, r^\Per(t), r^\Par(t)}^p(x-p(t)) \, ,
	\\
	&W^c_\xi(x,t):= W_{\xi, r^\Per(t), r^\Par(t)}^c(x-p(t)).
\end{align}






\subsection{The first time corrector}
\label{subsection: first time corrector}
We first note that
\begin{align}
\div(W^p_\xi \otimes W^p_\xi) = \frac{2}{r^\Par(t)}  \psi^\prime_{r^\Par(t)}(x-p(t)) \, \psi_{r^\Par(t)}(x-p(t)) \, \phi^2_{r^\Per(t)}(x - p(t))
\end{align}
We use overline to denote the first time corrector. We define the first time corrector as
\begin{align}
\ol{Q}_i(t, x) & \coloneqq \frac{1}{\mu(p(t))} \, \psi^2_{r^\Par(t)}(x-p(t)) \, \phi^2_{r^\Per(t)}(x - p(t)) \, \xi \nonumber \\
& = \frac{1}{\mu(p(t))} \, \frac{1}{r^\Par(t)} \psi^2\left(\frac{(x-p(t)) \cdot \xi}{r^\Par(t)}\right) \, \frac{1}{r^\Per(t)} \phi^2\left(\frac{(x-p(t)) \cdot \xi^\perp}{r^\Par(t)}\right) \, \xi \nonumber \\
& = \frac{1}{\ol{a}_i^2(p(t))}\frac{1}{\mu_0} \, \frac{1}{r^\Par_\Naught} \psi^2\left(\frac{(x-p(t)) \cdot \xi}{r^\Par_\Naught \, \ol{a}_i^2(p(t))}\right) \, \frac{1}{r^\Per_\Naught} \phi^2\left(\frac{(x-p(t)) \cdot \xi^\perp}{r^\Per_\Naught \, \ol{a}_i^2(p(t))}\right) \, \xi \nonumber 
\end{align}
A simple computation shows
\begin{align}
\partial_t \ol{Q}_i + \div(W^p_\xi \otimes W^p_\xi) =  - \frac{\nabla \ol{a}^2_i(p(t))}{\ol{a}^2_i(p(t))} \left[\psi^2_{r^\Par(t)}(y) \, \phi^2_{r^\Per(t)}(y) \xi + (y \cdot \xi) \div\left(\psi^2_{r^\Par(t)}(y) \, \phi^2_{r^\Per(t)}(y) \xi \otimes \xi \right) \right. \nonumber \\  \left. + (y \cdot \xi^\perp) \div\left(\psi^2_{r^\Par(t)}(y) \, \phi^2_{r^\Per(t)}(y) \xi \otimes \xi^\perp \right) \right]_{y = x - p(t)} \eqcolon I &
\end{align}
Next, we define a second term

\begin{align}
II = \frac{\nabla \ol{a}^2_i(p(t))}{\ol{a}^2_i(p(t))} \left[\psi^2_{\nu}(y) \, \phi^2_{\nu}(y) \xi \right]_{y = x - p(t)},
\end{align}
where $$\nu = \frac{K}{\lambda} \qquad \text{and} \quad K < 1$$
is a constant.
A simple integration by parts shows that
\begin{align}
\int_{\mathbb{T}^d} (I - II) \, {\rm d} x = 0.
\end{align}
Moreover, 
\begin{align}
\supp I \subseteq \supp II \subseteq B_{2 \nu}(x - p(t))
\end{align}
Therefore, we will put $I - II$ in the error.
\begin{align}
\norm{\div^{-1}(I - II)}_{L^\infty_t L^1_x} \leq \frac{2 K}{\lambda} \norm{\nabla \log |\ol{a}^2_i| }_{L^\infty_x}
\end{align}

\begin{lemma}
The following estimate holds
\begin{align}
\left|\int_{t=0}^{T_\xi} II \, {\rm d}t \right| \lesssim E \coloneqq \norm{\nabla \log |\ol{a}^2_i| }_{L^\infty_x}  \norm{ \ol{a}^2_i }_{L^\infty_x}  \frac{1}{\mu_0 \nu}
\end{align}
\end{lemma}
\begin{proof}
We have the following computation
\begin{align}
\left|\int_{t=0}^{T_\xi} II \, {\rm d}t \right| & \leq \norm{\nabla \log |\ol{a}^2_i| }_{L^\infty_x} \int_{t=0}^{T_\xi} \left[\psi^2_{\nu}(y) \, \phi^2_{\nu}(y)  \right]_{y = x - p(t)}, \, {\rm d}t 
\end{align}
Using the change of variables $$s = p(t) \cdot \xi,$$
we get
\begin{align}
\left|\int_{t=0}^{T_\xi} II \, {\rm d}t \right| & \leq \norm{\nabla \log |\ol{a}^2_i| }_{L^\infty_x} \int_{t=0}^{\wt{T}_\xi} \frac{1}{\mu(\xi s)} \frac{1}{\nu^2} \psi^2 \left(\frac{x \cdot \xi - s}{\nu}\right) \phi^2 \left(\frac{(x - x_s) \cdot \xi^\perp}{\nu}\right) \, {\rm d} s \nonumber \\
& \leq \norm{\nabla \log |\ol{a}^2_i| }_{L^\infty_x}  \norm{ \ol{a}^2_i }_{L^\infty_x} \int_{t=0}^{\wt{T}_\xi} \frac{1}{\mu_0} \frac{1}{\nu^2} \psi^2 \left(\frac{x \cdot \xi - s}{\nu}\right) \phi^2 \left(\frac{(x - x_s) \cdot \xi^\perp}{\nu}\right) \, {\rm d} s \nonumber \\
& \lesssim \norm{\nabla \log |\ol{a}^2_i| }_{L^\infty_x}  \norm{ \ol{a}^2_i }_{L^\infty_x}  \frac{1}{\mu_0 \nu}
\end{align}
\end{proof}
We have the following definition of the time cutoff that we will use in rest of this section.
\begin{align}
\ol{\zeta}(t) = 2 \zeta\left(\frac{t - k \tau - \frac{(i-1)}{4} \tau}{\tau/4}\right), \qquad \text{for} \quad i \in \{1, 2, 3, 4\}.
\end{align}
where we have
\begin{align}
\int_{0}^{1} \zeta^2(t) \, {\rm d} t = 1.
\end{align}
As a result,
\begin{align}
\frac{1}{\tau}\int_{k \tau}^{(k+1)\tau} \ol{\zeta}^2(t^\prime) \, {\rm d} t^\prime = 1.
\end{align}

\begin{lemma}
The following estimate holds
\begin{align}
\left|\frac{1}{\tau} \int_{k \tau}^{(k+1)\tau} II \, \ol{\zeta}^2(t) \, {\rm d}t - \frac{1}{T_\xi} \int_{t=0}^{T_\xi} \frac{\nabla \ol{a}^2_i(p(t))}{\ol{a}^2_i(p(t))} \left[\psi^2_{\delta}(y) \, \phi^2_{\delta}(y) \xi \right]_{y = x - p(t)}  \, {\rm d}t  \right|  \lesssim \frac{1}{\tau} E
\end{align}
\end{lemma}
\begin{proof}
We let 
\begin{align}
m = \left\lfloor \frac{\tau}{T_\xi} \right\rfloor
\end{align}
\begin{align}
\frac{1}{\tau} \int_{k \tau}^{(k+1) \tau} II \, \ol{\zeta}^2(t) \, {\rm d}t = \sum_{i = 0}^{m} \frac{1}{\tau} \int_{k \tau + i T_\xi}^{k \tau + (i+1) T_\xi} II \, \ol{\zeta}^2(t) \, {\rm d}t + \frac{1}{\tau} \int_{k \tau + m T_\xi}^{(k+1)\tau} II \, \ol{\zeta}^2(t) \, {\rm d}t 
\end{align}
Next, we note that
\begin{align}
\left|\ol{\zeta}^2(t) - \frac{1}{T_\xi} \int_{i T_\xi}^{(i+1) T_\xi} \ol{\zeta}^2(t^\prime) \, {\rm d} t^\prime \right| \leq \norm{\ol{\zeta}^2}_{C^1} T_\xi \lesssim \frac{T_\xi}{\tau}
\end{align}
and 
\begin{align}
\left|\frac{1}{\tau} \int_{k \tau + m T_\xi}^{(k+1)\tau} II \, \ol{\zeta}^2(t^\prime) \, {\rm d} t^\prime \right| \leq \frac{E}{\tau}. 
\end{align}
Finally, we recall
\begin{align}
\frac{1}{\tau}\int_{k \tau}^{(k+1)\tau} \ol{\zeta}^2(t^\prime) \, {\rm d} t^\prime = 1.
\end{align}
\end{proof}



\begin{lemma}
The following estimate holds
\begin{align}
\left|\div^{-1} \left(\frac{1}{T_\xi} \int_{t=0}^{T_\xi} \frac{\nabla \ol{a}^2_i(p(t)) \cdot \xi}{\ol{a}^2_i(p(t))} \left[\psi^2_{\delta}(y) \, \phi^2_{\delta}(y) \right]_{y = x - p(t)} \, {\rm d}t -   \frac{1}{\nu \mu_0 T_\xi}\nabla \ol{a}^2_i(x) \cdot \xi \phi^2_{\nu}(x) \right) \right| \lesssim \norm{\nabla R_{n}}_{L^\infty_t L^1_{x}} \frac{1}{\mu_0 T_\xi}.
\end{align}
\label{lemma: leading order term}
\end{lemma}
\begin{proof}
In the integral 
\begin{align}
\frac{1}{T_\xi} \int_{t=0}^{T_\xi} \frac{\nabla \ol{a}^2_i(p(t)) \cdot \xi}{\ol{a}^2_i(p(t))} \left[\psi^2_{\delta}(y) \, \phi^2_{\delta}(y) \right]_{y = x - p(t)} \, {\rm d}t
\end{align}
we consider the change of variables $$s = p(t) \cdot \xi,$$
which gives
\begin{align}
\frac{1}{T_\xi} \int_{t=0}^{T_\xi} \frac{\nabla \ol{a}^2_i(s \xi) \cdot \xi }{\mu_0} \frac{1}{\nu^2} \psi^2 \left( \frac{x \cdot \xi - s}{\nu}\right) \phi^2 \left( \frac{x \cdot \xi^\perp}{\nu}\right) \, {\rm d}s 
\end{align}
after an integration-by-parts it leads to
\begin{align}
- \frac{1}{T_\xi} \int_{t=0}^{T_\xi} \frac{ \ol{a}^2_i(s \xi) }{\mu_0} \div \left[\psi^2_\nu(x - s \xi) \phi^2_\nu(x - s\xi) \xi \right] \, {\rm d}s \nonumber \\
= - \div\left( \frac{1}{T_\xi} \int_{t=0}^{T_\xi} \frac{ \ol{a}^2_i(s \xi) }{\mu_0} \psi^2_\nu(x - s \xi) \phi^2_\nu(x - s\xi) \xi  \, {\rm d}s\right)
\end{align}
On the other hand, we also have
\begin{align}
 \nabla \ol{a}^2_i(x) \cdot \xi \phi^2_{\nu}(x) & = \div \left(\ol{a}^2_i(x)  \phi^2_{\nu}(x) \xi \right) \nonumber \\
 & = \div \left( \frac{1}{T_\xi} \int_{0}^{T_\xi} \ol{a}^2_i(x) \psi^2_\nu(x - s \xi) \phi^2_{\nu}(x) \xi \, {\rm d} s\right)
\end{align}
Complete the computations here.
%Next, we note that 
%\begin{align}
%\left|\frac{1}{T_\xi} \int_{t=0}^{T_\xi} \frac{(\nabla \ol{a}^2_i(s \xi) - \nabla \ol{a}^2_i(x) )}{\mu_0}  \frac{1}{\nu^2} \psi^2 \left( \frac{x \cdot \xi - s}{\nu}\right) \phi^2 \left( \frac{x \cdot \xi^\perp}{\nu}\right) \, {\rm d}s \right| & \lesssim \norm{\nabla \ol{a}^2_i}_{C^1_{t, x}} \frac{1}{\mu_0 T_\xi} \nonumber \\
%& \lesssim \norm{\nabla R_{\ell}}_{C^1_{t, x}} \frac{1}{\mu_0 T_\xi}
%\end{align}
\end{proof}







\subsection{The second time corrector}
\label{subsection: second time corrector}
We define the second time corrector to be
\begin{align}
\wt{Q}(t, x) & \coloneqq \int_0^t \left[ II \, \ol{\zeta}^2 - P_{\tau}(II \, \ol{\zeta}^2)\right] \, {\rm d} t^\prime, \nonumber \\
& = \int_{k \tau}^t \left[ II \, \ol{\zeta}^2 - P_{\tau}(II \, \ol{\zeta}^2)\right] \, {\rm d} t^\prime.
\end{align}
From here we see that the magnitude of the second corrector can be bounded as
\begin{align}
|\wt{Q}(t, x)| & \leq 2 \tau P_{\tau}(|II \, \ol{\zeta}^2|) \nonumber \\
& \leq \tau (\text{Leading order term } + \text{ errors}), \nonumber \\
& \leq \tau \left(\frac{E}{T_\xi} + \frac{E}{\tau}\right) \nonumber \\
& \leq \tau \norm{\nabla \log |\ol{a}^2_i| }_{L^\infty_x}  \norm{ \ol{a}^2_i }_{L^\infty_x}  \frac{1}{\nu \mu_0 T_\xi}.
\end{align}
Furthermore, the $\mathscr{L}^2$ measure of the support of $\wt{Q}$ is $$\sim \lambda \times \frac{1}{\lambda} \sim 1.$$
From here we see that 
\begin{align}
\norm{\wt{Q}_i}_{L^\infty_t L^2_x} \leq \tau \norm{\nabla \log |\ol{a}^2_i| }_{L^\infty_x}  \norm{ \ol{a}^2_i }_{L^\infty_x}  \frac{1}{\nu \mu_0 T_\xi}.
\end{align}
and 
\begin{align}
\norm{D \wt{Q}_i}_{L^\infty_t L^p_x} \leq \tau \lambda \norm{\nabla \log |\ol{a}^2_i| }_{L^\infty_x}  \norm{ \ol{a}^2_i }_{L^\infty_x}  \frac{1}{\nu \mu_0 T_\xi}.
\end{align}

{\color{blue}
The set where the derivative of $\tilde Q$ is of size $\lambda$ is actually small (like a strip of thickness $1/\lambda$).



\bigskip

Morally,
\begin{equation}
    \tilde Q \sim \tau \div(R_n)
\end{equation}
It cannot be smaller than that.

}

\subsection{Cancelling the error}
Finally, we come to the part of cancelling the error. The leading order term we got in Lemma \ref{lemma: leading order term} is
\begin{align}
\div (\ol{a}_i^2 \xi \otimes \xi) = \div( P_\tau(a_i^2(t, x)) \xi \otimes \xi).
\end{align}
We want to use this term to cancel
\begin{align}
\div (a_i^2(t, x) \xi \otimes \xi)
\end{align}
Therefore, the contribution towards the error is
\begin{align}
\tau \norm{\partial_t R_n}_{L^\infty_t L^1_x}.
\end{align}






\subsection{The time derivative of the principal part}
\label{subsection: time derivative principal part}
In this subsection, $\mu$, $r^\Per$ and $r^\Par$ would automatically mean $\mu(p(t))$, $r^\Per(p(t))$ and $r^\Par(p(t))$, unless we specifically add `$0$' in the subscript. We first recall,
\begin{align}
W^{(p)}_i(x) =  \left(\frac{1}{r^{\Per} \, r^{\Par}}\right)^{\frac{1}{2}} \psi\left(\frac{(x - p(t)) \cdot \xi}{r^{\Par}}\right) \phi\left(\frac{(x - p_0) \cdot \xi^\perp_i}{r^{\perp}}\right) \ol{\zeta}(t) \xi_i \nonumber
\end{align}
Then the time derivative is given by
\begin{align}
\partial_t W^{(p)}_i(x) = T_1 + T_2 + T_3 + T_4 + T_5.
\end{align}
Next, we list all of these five terms one-by-one. 

The first term is
\begin{align}
T_1 = \left(\frac{1}{r^{\Per} \, r^{\Par}}\right)^{\frac{1}{2}} \left(-\frac{\mu(p(t))}{r^\Par}\right) \psi^\prime(\dots) \phi(\dots) \ol{\zeta} e_i = \div(A_1),
\end{align}
where 
\begin{align}
A_1 = \left(\frac{1}{r^{\Per} \, r^{\Par}}\right)^{\frac{1}{2}} \left(-\frac{\mu(p(t))}{r^\Par}\right) \ol{\zeta} M_1
\end{align}
and the matrix $M_1$ is given by
\begin{align}
M_1 = 
\begin{bmatrix}
0 && r^\Per \psi^\prime(\dots) \Phi^{\prime \prime \prime}(\dots) \, \xi \otimes \xi^\perp \\[10pt]
r^\Per \psi^{\prime}(\dots) \Phi^{\prime \prime \prime}(\dots) \, \xi^\perp \otimes \xi && -\frac{(r^\Per)^2}{r^\Par} \psi^{\prime \prime}(\dots) \Phi^{ \prime \prime}(\dots) \, \xi^\perp \otimes \xi^\perp
\end{bmatrix}.
\end{align}


The second term is
\begin{align}
T_2 = \mu \left(\frac{1}{r^{\Per} \, r^{\Par}}\right)^{\frac{1}{2}} \left(-\frac{\nabla \ol{a}_i^2(p(t)) \cdot \xi}{\ol{a}_i^2(p(t))}\right) \psi(\dots) \phi(\dots) \ol{\zeta} \xi = \div(A_2),
\end{align}
where 
\begin{align}
A_2 = \mu \left(\frac{1}{r^{\Per} \, r^{\Par}}\right)^{\frac{1}{2}} \left(-\frac{\nabla \ol{a}_i^2(p(t)) \cdot \xi}{\ol{a}_i^2(p(t))}\right) \ol{\zeta} M_2
\end{align}
and the matrix $M_2$ is given by
\begin{align}
M_2 = 
\begin{bmatrix}
0 && r^\Per \psi(\dots) \Phi^{\prime \prime \prime}(\dots) \, \xi \otimes \xi^\perp \\[10pt]
r^\Per \psi(\dots) \Phi^{\prime \prime \prime}(\dots) \, \xi^\perp \otimes \xi && -\frac{(r^\Per)^2}{r^\Par} \psi^{\prime}(\dots) \Phi^{ \prime \prime}(\dots) \, \xi^\perp \otimes \xi^\perp
\end{bmatrix}.
\end{align}


The third term is
\begin{align}
T_3 = \mu \left(\frac{1}{r^{\Per} \, r^{\Par}}\right)^{\frac{1}{2}} \left[\frac{ (x - p(t)) \cdot \xi}{r^{\Par}}\right] \left(-\frac{\nabla \ol{a}_i^2(p(t)) \cdot \xi}{\ol{a}_i^2(p(t))}\right) \psi^\prime(\dots) \phi(\dots) \ol{\zeta} \xi = \div(A_3),
\end{align}
where 
\begin{align}
A_3 = \mu \left(\frac{1}{r^{\Per} \, r^{\Par}}\right)^{\frac{1}{2}} \left(-\frac{\nabla \ol{a}_i^2(p(t)) \cdot \xi}{\ol{a}_i^2(p(t))}\right) \ol{\zeta}  M_3
\end{align}
and the matrix $M_3$ is given by
\begin{align}
M_3 = 
\begin{bmatrix}
0 && r^\Per (x \psi)(\dots) \Phi^{\prime \prime \prime}(\dots) \, \xi \otimes \xi^\perp \\[10pt]
r^\Per (x \psi)(\dots) \Phi^{\prime \prime \prime}(\dots) \, \xi^\perp \otimes \xi && -\frac{(r^\Per)^2}{r^\Par} ( x \psi)^{\prime}(\dots) \Phi^{ \prime \prime}(\dots) \, \xi^\perp \otimes \xi^\perp
\end{bmatrix}.
\end{align}
Here, $(x \psi) (\dots)$ mean to represent $$\left[\frac{ (x - p(t)) \cdot \xi}{r^{\Par}}\right] \psi \left(\frac{(x - p(t)) \cdot \xi}{r^{\Par}}\right).$$





The fourth term is given by
\begin{align}
T_4 = \mu \left(\frac{1}{r^{\Per} \, r^{\Par}}\right)^{\frac{1}{2}} \left[\frac{(x - p_0) \cdot \xi^\perp}{r^{\Per}}\right] \left(-\frac{\nabla \ol{a}_i^2(p(t)) \cdot \xi}{\ol{a}_i^2(p(t))}\right) \psi(\dots) \phi^\prime(\dots) \ol{\zeta} e_i = \div(A_4),
\end{align}
where 
\begin{align}
A_4 = \mu \left(\frac{1}{r^{\Per} \, r^{\Par}}\right)^{\frac{1}{2}} \left(-\frac{\nabla \ol{a}_i^2(p(t)) \cdot \xi}{\ol{a}_i^2(p(t))}\right) \ol{\zeta} M_4
\end{align}
and the matrix $M_4$ is given by
\begin{align}
M_4 = 
\begin{bmatrix}
0 && r^\Per \psi(\dots) (x \phi - \Phi^{\prime \prime \prime})(\dots) \, \xi \otimes \xi^\perp \\[10pt]
r^\Per \psi(\dots) (x \phi - \Phi^{\prime \prime \prime})(\dots) \, \xi^\perp \otimes \xi && -\frac{(r^\Per)^2}{ r^\Par} \psi^\prime(\dots) (x \Phi^{\prime \prime \prime} - \Phi^{\prime \prime \prime} - \Phi^{\prime \prime})(\dots) \, \xi^\perp \otimes \xi^\perp
\end{bmatrix}.
\end{align}




The fifth term is
\begin{align}
T_5 = \left(\frac{1}{r^{\Per} \, r^{\Par}}\right)^{\frac{1}{2}} \left(\frac{1}{\tau/4}\right) \psi(\dots) \phi(\dots) \dot{\ol{\zeta}} e_i = \div(A_5),
\end{align}
where 
\begin{align}
A_5 = \left(\frac{1}{r^{\Per} \, r^{\Par}}\right)^{\frac{1}{2}} \left(\frac{1}{\tau/4}\right) \dot{\ol{\zeta}} M_5
\end{align}
and the matrix $M_5$ is given by
\begin{align}
M_5 = 
\begin{bmatrix}
0 && r^\Per \psi(\dots) \Phi^{\prime \prime \prime}(\dots) \, \xi \otimes \xi^\perp \\[10pt]
r^\Per \psi(\dots) \Phi^{\prime \prime \prime}(\dots) \, \xi^\perp \otimes \xi && -\frac{(r^\Per)^2}{r^\Par} \psi^{\prime}(\dots) \Phi^{ \prime \prime}(\dots) \, \xi^\perp \otimes \xi^\perp
\end{bmatrix}.
\end{align}

\subsection{$L^1$-norm of term A}
We define our term $A$ to be
\begin{align}
A = A_1 + A_2 + A_3 + A_4 + A_5.
\end{align}
A straightforward computation shows
\begin{align}
\norm{A}_{L^\infty_t L^1_x} \leq \norm{R_n}_{L^\infty_t L^1_x}^{\frac{1}{2}} \mu_0\frac{(r^\Per_\Naught)^{3/2}}{(r^\Par)^{1/2}} \; + \; 
\norm{\nabla \log (|R_n|)}_{L^\infty_t L^\infty_x} \norm{R_n}_{L^\infty_t L^\infty_x}
\mu_0 (r^\Per_\Naught)^{3/2}(r^\Par_\Naught)^{1/2}  \nonumber \\ + \norm{R_n}_{L^\infty_t L^1_x}^{\frac{1}{2}} \norm{R_n}^2_{L^\infty_t L^\infty_x} \frac{1}{\tau} (r^\Per_\Naught)^{3/2}(r^\Par_\Naught)^{1/2}. 
\end{align}
The first term in this estimate comes from $A_1$, the second term comes from $A_2$, $A_3$ and $A_5$ and the last term comes from $A_5$.
In this estimate the dominating term is supposed to be only the first term on the right hand side.

==> Figures/Old_Material/Anuj_Notes/mollification.tex <==
\section{Mollification}
\label{section: mollification}
The equations at the $n$th iteration are
\begin{align}
\partial_t u_n + \div(u_n \otimes u_n) = - \nabla p_n + \div(R_n)
\end{align}
We consider the space time mollification
\begin{align}
 u_{\ell} = u_n \ast \varphi_{\ell}, \qquad p_{\ell} = p_n \ast \varphi_{\ell}, \qquad R_{\ell} = R_n \ast \varphi_{\ell}
\end{align}
Definition of the iodicturbation
\begin{align}
w_{n+1} = u_{n+1}  - u_{\ell}
\end{align}
Equation of the perturbation
\begin{align}
\partial_t w_{n+1} + \div(u_{\ell} \otimes w_{n+1}) + \div(w_{n+1} \otimes u_{\ell}) + \left[\div(w_{n+1} \otimes w_{n+1}) + \div(R_{\ell})\right] & \nonumber \\
+ \div(u_{\ell} \otimes u_{\ell} - (u_n \otimes u_n)_{\ell}) = - \nabla (p_{n+1} - p_n) + \div(R_{n+1}) &
\end{align}
\subsection{Estimates at the level of mollification}
\label{subsection: estimates mollification}
\begin{align}
\norm{R_{\ell}}_{L^\infty_t L^1_x} \leq \norm{R_n}_{L^\infty_t L^1_x}
\end{align}
\begin{align}
\norm{u_n - u_{\ell}}_{L^\infty_t L^2_x} \leq \ell \norm{u_n}_{C^1_{t, x}}
\end{align}
\begin{align}
\norm{D u_n - D u_{\ell}}_{L^\infty_t L^p_x} \leq \ell \norm{u_n}_{C^2_{t, x}}
\end{align}
\begin{align}
\norm{u_{\ell} \otimes u_{\ell} - (u_n \otimes u_n)_{\ell}}_{L^\infty_t L^1_x} \leq \ell \norm{u_n}^2_{C^1_{t, x}}
\end{align}
\begin{align}
\norm{u_n - u_{\ell}}_{C^N_{t, x}} \lesssim \ell^{1-N} \norm{u_n}_{C^1_{t, x}}
\end{align}
\begin{align}
\norm{u_n - u_{\ell}}_{C^N_{t, x}} \lesssim \ell^{2-N} \norm{u_n}_{C^2_{t, x}}
\end{align}

==> Figures/Old_Material/Anuj_Notes/norm_estimates.tex <==
\section{Estimates on the $L^2$-norm of the velocity and $L^p$ norm of the vorticity}
\label{section: norm estimates}
\subsection{$L^2$-norm of velocities}
\label{subsection: L2 norm velocity}
\begin{align}
\norm{u^{(p)}_{n+1}}_{L^\infty_t L^2_x} \leq \norm{W_i^{(p)}}_{L^\infty_t L^2_x} \leq \norm{ R_n }_{L^\infty_t L^1_x}^{\frac{1}{2}}.
\end{align}
\begin{align}
\norm{\ol{u}^{(t)}_{n+1}}_{L^\infty_t L^2_x} \leq \norm{\ol{Q}_i}_{L^\infty_t L^2_x}.
\end{align}
We note that
\begin{align}
|\ol{Q}_i(t, x)| & \leq \frac{U_0^2}{\mu(p(t))} \frac{1}{r^{\Per}(p(t))} \frac{1}{r^{\Par}(p(t))}\psi^2\left(\frac{(x - p(t)) \cdot \xi}{r^{\Par}(p(t))}\right) \phi^2\left(\frac{(x - p_0) \cdot \xi^\perp}{r^{\Per}(p(t))}\right)
\end{align}
and has a support of area
\begin{align}
r^{\Par}(p(t)) r^{\Per}(p(t))
\end{align}
Therefore,
\begin{align}
\norm{\ol{Q}_i}_{L^\infty_t L^2_x} \leq \norm{ R_n }_{L^\infty_t L^1_x} \frac{1}{\mu_0} \left(\frac{1}{r^\Par_\Naught} \frac{1}{r^\Per_\Naught}\right)^{\frac{1}{2}} 
\end{align}
\begin{align}
\norm{\wt{u}^{(t)}_{n+1}}_{L^\infty_t L^2_x} \leq \norm{\wt{Q}_i}_{L^\infty_t L^2_x}.
\end{align}
Now referring to \S \ref{subsection: second time corrector}, we get
\begin{align}
|\wt{Q}_i(t, x)| \leq  \tau \norm{\nabla \log |\ol{a}^2_i| }_{L^\infty_x}  \norm{ \ol{a}^2_i }_{L^\infty_x}  \frac{1}{\nu \mu_0 T_\xi}.
\end{align}
and 
\begin{align}
\norm{\wt{Q}_i}_{L^\infty_t L^2_x} \leq \tau \norm{\nabla \log |\ol{a}^2_i| }_{L^\infty_x}  \norm{ \ol{a}^2_i }_{L^\infty_x}  \frac{1}{\nu \mu_0 T_\xi}.
\end{align}









\subsection{$L^1$-norm of vorticity}
\label{subsection: L1 norm vorticity}
For convenience, we rewrite $L^1$-norm of the vorticity separately. We substitute $p = 1$ in above expressions and obtain
\begin{align}
\norm{D W_i^{(p)}}_{L^\infty_t L^1_x} \leq \norm{ R_n }_{L^\infty_t L^1_x}^{\frac{1}{2}}  \left(\frac{r^\parallel_0}{r^\perp_0}\right)^{\frac{1}{2}}.
\end{align}
\begin{align}
\norm{D \ol{Q}_i}_{L^\infty_t L^1_x} \leq \norm{ R_n }_{L^\infty_t L^1_x} \; \frac{\lambda}{\mu_0} \frac{1}{r^\perp_0} 
\end{align}
\begin{align}
\norm{D \wt{Q}_i}_{L^\infty_t L^1_x} \leq \tau \lambda \norm{\nabla \log |\ol{a}^2_i| }_{L^\infty_x}  \norm{ \ol{a}^2_i }_{L^\infty_x}  \frac{1}{\nu \mu_0 T_\xi}.
\end{align}





%\subsection{$L^p$-norm of vorticity}
%\label{subsection: Lp norm vorticity}
%We see that
%\begin{align}
%|D W_i^{(p)} (t, x)| \leq U_0 \left(\frac{1}{r^\parallel(p(t))}\right)^{\frac{1}{2}} \left(\frac{1}{r^\perp(p(t))}\right)^{\frac{1}{2}} \; \frac{\lambda}{r^\perp(p(t))}.
%\end{align}
%Therefore, we get the $L^p$-norm to be
%\begin{align}
%\norm{D W_i^{(p)}(t)}_{L^p_x} \leq U_0 \left(\frac{1}{r^\parallel(p(t))}\right)^{\frac{1}{2}} \left(\frac{1}{r^\perp(p(t))}\right)^{\frac{1}{2}} \; \frac{\lambda}{r^\perp(p(t))} \left(\frac{r^\perp(p(t)) r^\parallel(p(t))}{\lambda^2}\right)^{\frac{1}{p}}
%\end{align}
%which simplifies to
%\begin{align}
%\norm{D W_i^{(p)}}_{L^\infty_t L^p_x} \leq \frac{\norm{ R_n }_{L^\infty_t L^1_x}^{\frac{1}{2}}}{\norm{ R_n }_{L^\infty_t L^\infty_x}^{(2-2/p)}} \; \lambda^{(2-2/p)} \frac{1}{(r^\perp_0)^{(3/2-1/p)}} \frac{1}{(r^\parallel_0)^{(1/2-1/p)}}.
%\end{align}
%We move to vorticity in the first corrector.
%\begin{align}
%|D \ol{Q}_i(t, x)| & \leq \frac{U_0^2}{\mu(p(t))} \frac{1}{r^{\perp}(p(t))} \frac{1}{r^{\parallel}(p(t))} \frac{\lambda}{r^{\perp}(p(t))}.
%\end{align}
%The estimate on the $L^p$ norm therefore is
%\begin{align}
%\norm{D \ol{Q}_i(t)}_{ L^p_x} \leq \frac{U_0^2}{\mu(p(t))} \frac{1}{r^{\perp}(p(t))} \frac{1}{r^{\parallel}(p(t))} \frac{\lambda}{r^{\perp}(p(t))} \left(\frac{r^{\perp}(p(t)) r^{\parallel}(p(t))}{\lambda^2}\right)^{\frac{1}{p}}
%\end{align}
%which simplifies to
%\begin{align}
%\norm{D \ol{Q}_i}_{L^\infty_t L^p_x} \leq \frac{\norm{ R_n }_{L^\infty_t L^1_x}}{\norm{ R_n }_{L^\infty_t L^\infty_x}^{(2-2/p)}} \; \frac{\lambda^{(3-2/p)}}{\mu_0} \frac{1}{(r^\perp_0)^{(2-1/p)}} \frac{1}{(r^\parallel_0)^{(1-1/p)}}
%\end{align}
%The $L^p$-norm of the second corrector is straightforward. We get,
%\begin{align}
%\norm{D \wt{Q}_i}_{L^\infty_t L^p_x} \leq \norm{ R_n }_{C^1_{t, x}} \frac{\tau}{\lambda}
%\end{align}

==> Figures/Old_Material/Anuj_Notes/old_new_bb.tex <==
%Date March 24, 2024
%Date March 24, 2024
%Date March 24, 2024
%Date March 24, 2024
%Date March 24, 2024
%Date March 24, 2024
%Date March24, 2024
%Date March 24, 2024

\section{Principal building block}
\label{sec: principal bb}
In this section, we construct principal building block velocity field for our convex integration scheme. One of the main ingredient of our construction is the Lamb--Chaplygin dipole, which is an exact solution of the 2D Euler equation on $\mathbb{R}^2$. The main advantage of the Lamb--Chaplygin dipole is that it translates with a constant velocity without deforming. The Lamb--Chaplygin dipole consists of two regions: a circular inner core of some fixed radius where the vorticity of opposite signs concentrate and out this core the velocity field is irrotational. Therefore, outside in inner core the flow is potential and is given by the doublet flow. The Lamb--Chaplygin dipole can also be understood as the desingularization of the doublet, which has a singularity at the origin. The Lamb--Chaplygin dipole in exact solution defined on $\mathbb{R}^2$. We find an approximate solution corresponding to this dipole on $\mathbb{T}^2$ through a patching argument. We first define a periodic analog of the doublet flow with the help of a Weierstrass $\wp$ function. The idea is that the periodic doublet in the leading order is the same as the doublet flow close to the singularity at the origin. Therefore, in the outside region of the Lamb--Chaplygin dipole, we patch it with the periodic doublet with the help of a cutoff function. We show that the errors generated in the process of patching are quite small. In the next few subsection, we carry out this construction process.


\subsection{A few preliminaries}
Let $v$ be a smooth velocity field given by a smooth streamfunction
\begin{align}
v = \nabla^\perp \phi.
\end{align}
Suppose that $\Omega \in \mathbb{R}^2$ is a connected domain whose boundary $\partial \Omega$ is a rectifiable curve. Then, we see that the integration of $v$ over $\Omega$ can be evaluated as
\begin{align}
\int_{\Omega} v dx = \int_{\Omega} \nabla^\perp \psi \, {\rm d} x = \int_{\partial \Omega} \psi \, n^\perp \, {\rm d} s,
\end{align}
which is a simple consequence of the divergence theorem. The integral on the right hand side make sense even if the velocity field $v$ is singular. Now we state a way to evaluate this integral in situations which are useful to us.
\begin{lemma}
Let $f(z) = \phi(x_1, x_2) + i \psi(x_1, x_2)$ be a complex function such that $\psi(x_1, x_2) = - \phi(x_2, x_1)$. If $\Omega = \left[-\frac{1}{2}, \frac{1}{2}\right]^2$ then
\begin{align}
\int_{\partial \Omega} \psi \, n^\perp \, {\rm d} s = \left( - \frac{1}{2} \operatorname{Im} \oint_{\partial \Omega} f(z) \, {\rm d}z,  \; \frac{1}{2} \operatorname{Re} \oint_{\partial \Omega} f(z) \, {\rm d}z \right)
\end{align}
\end{lemma}
The complex functions we will be using fall under this category.
 \begin{proof}
 Let $z(t) : [0, \ell] \to \mathbb{C}$ be the parameterization of $\gamma$ with arc length. 
 Writing $z(t) = x_1(t) + i x_2(t)$, we have
 \begin{align}
 \operatorname{Im} \oint_{\gamma} f(z) \, {\rm d}z & = \operatorname{Im} \int_0^\ell f(z(t)) z^\prime(t) \, {\rm d}t \nonumber \\
 & = \operatorname{Im} \int_0^\ell \left( \; \phi(x_1(t), x_2(t)) \, + \, i \psi(x_1(t), x_2(t)) \; \right) \; (x_1^\prime(t) + i x_2^\prime(t)) \; {\rm d}t \nonumber \\
 & = \int_0^\ell \phi(x_1(t), x_2(t)) \; x_2^\prime(t) \; {\rm d}t + \int_0^\ell \psi(x_1(t), x_2(t)) \; x_1^\prime(t) \; {\rm d}t \nonumber \\
 & = \int_0^\ell \psi(x_1(t), x_2(t)) \; ( x_1^\prime(t) - x_2^\prime(t) ) \; {\rm d}t
 \end{align}
 Similarly, we can also get
 \begin{align}
 \operatorname{Re} \oint_{\gamma} f(z) \, {\rm d}z 
 & = - \int_0^\ell \psi(x_1(t), x_2(t)) \; ( x_1^\prime(t) + x_2^\prime(t) ) \; {\rm d}t
 \end{align}
 \end{proof}

\subsection{A doublet on $\mathbb{R}^2$}
\label{subsec: doublet}
A doublet flow is a divergence-free potential flow on $\mathbb{R}^2 \setminus \{0\}$. The potential $\wt{\Phi}$ and the streamfunction $\wt{\Psi}$ are given by a complex function as
\begin{align}
\wt{F}(z) \coloneqq \wt{\Phi}(x_1, x_2) + i \wt{\Psi}(x_1, x_2) \coloneqq - \frac{1}{z}, \quad \text{where} \quad z = x_1 + i x_2.
\end{align}
We define the velocity field $\wt{V} = (\wt{V}_1, \wt{V}_2)$ using the derivative of the function $F$ as
\begin{align}
\wt{f}(z) \coloneqq \wt{V}_1(x_1, x_2) - i \wt{V}_2(x_1, x_2) \coloneqq  \frac{1}{z^2}.
\end{align}
From our definition, it is clear that
\begin{align}
\wt{V} = \nabla^\perp \wt{\Psi} = \nabla \wt{\Phi}.
\end{align}
Next, we define a pressure field
\begin{align}
\wt{P} = \partial_1 \wt{\Phi} - \frac{|\nabla \wt{\Phi}|^2}{2}.
\end{align}
For a given $r > 0$, we define our scaled variables as
\begin{align}
\wt{\Phi}_{r} = \wt{\Phi}\left(\frac{x}{r}\right), \quad 
\wt{\Psi}_{r} = \wt{\Psi}\left(\frac{x}{r}\right), \quad 
\wt{V}_{r} = \frac{1}{r}\wt{V}\left(\frac{x}{r}\right), \quad
\wt{P}_{r} = \frac{1}{r^2}\wt{P}\left(\frac{x}{r}\right).
\end{align}
A simple computation shows that for $\bs{x} \in \mathbb{R}^2 \setminus \{0\}$, we have
\begin{align}
- \frac{1}{r} \partial_1 \wt{V}_{r} + \wt{V}_{r} \cdot \nabla \wt{V}_{r} = - \nabla \wt{P}_{r}.
\end{align}






\subsection{A periodic doublet on $\mathbb{R}^2$}
\label{subsec: periodic doublet}
Next, we define a periodic version of the doublet flow on $\mathbb{R}^2$, with period $1$ both in $x_1$ and $x_2$ directions. We again define the potential $\wh{\Phi}$ and streamfunction $\wh{\Psi}$ of the required flow field through a complex function.
\begin{align}
\wh{F}(z) \coloneqq \wh{\Phi}(x_1, x_2) + i \wh{\Psi}(x_1, x_2) \coloneqq - \frac{1}{z} - \sum_{\substack{\omega = m + i n \\ (m, n) \in \mathbb{Z}^2 \\ (m, n) \neq (0, 0)}} \frac{z^2}{(z+\omega) \omega^2}.
\label{principal bb: period doublet stream pot}
\end{align}
The function on the right hand side is known as the Weierstrass zeta function, which is not a doubly periodic function. We define the velocity field using the derivative function of the function $\wh{F}$ as
\begin{align}
\wh{f}(z) \coloneqq  \wh{V}_1(x_1, x_2) - i \wh{V}_2(x_1, x_2) \coloneqq \frac{1}{z^2} + \sum_{\substack{\omega = m + i n \\ (m, n) \in \mathbb{Z}^2 \\ (m, n) \neq (0, 0)}} \left(\frac{1}{(z+\omega)^2} - \frac{1}{\omega^2}\right).
\end{align}
The function on the right hand side in the above expression is known as Weierstrass $\wp$-function, which is a doubly periodic function. 
From our definition, it is clear that
\begin{align}
\wh{V} = \nabla^\perp \wh{\Psi} = \nabla \wh{\Phi}.
\end{align}
Next, we define a pressure field
\begin{align}
\wt{P} = \partial_1 \wh{\Phi} - \frac{|\nabla \wh{\Phi}|^2}{2}.
\end{align}
For a given $r > 0$, we define our scaled variables as
\begin{align}
\wh{\Phi}_{r} = r \wh{\Phi}, \quad 
\wh{\Psi}_{r} = r \wh{\Psi}, \quad 
\wh{V}_{r} = \nabla^\perp \wh{\Psi}_{r}, \quad
\wh{P}_{r} = \frac{1}{r} \partial_1 \wh{\Phi}_{r} - \frac{|\nabla \wh{\Phi}_r|^2}{2}.
\label{principal bb: period doublet scaled}
\end{align}
A simple computation shows that for $x \in \mathbb{R}^2 \setminus \mathbb{Z}^2$, we have
\begin{align}
- \frac{1}{r} \partial_1 \wt{V}_{r} + \wt{V}_{r} \cdot \nabla \wt{V}_{r} = - \nabla \wt{P}_{r}.
\label{principal bb: scaled period doublet eqn}
\end{align}







\subsection{Desingularization of doublet on $\mathbb{R}^2$: The Lamb--Chaplygin dipole}
For the description of the velocity field in this section, we use polar coordinates $\rho$ and $\theta$, where $x_1 = \rho \cos\theta$ and $x_2 = \rho \sin \theta$. The Lamb--Chaplygin dipole is a desingularization of the doublet flow. It consists of two regions: (i) $\rho \leq 1$ the desingularized region, where the vorticity is nonzero, (ii) $\rho \geq 1$, where the flow is potential given in section \ref{subsec: doublet}. We define the streamfunction $\ol{\Psi}$ for this flow as
\begin{align}
\ol{\Psi} \coloneqq 
\begin{cases}
\rho \sin \theta - \frac{2 J_1(b\rho)}{b J_0(b)} \sin \theta \qquad & \text{when} \quad \rho \leq 1, \\
\frac{\sin \theta}{\rho} \qquad & \text{when} \quad \rho \geq 1. 
\end{cases}
\end{align}
Here, $J_0$ and $J_1$ are the Bessel functions of first kind of zero and first order respectively. The number $b \approx 3.831705970\dots$ is the first non-trivial zero of $J_1$. It is clear that for $\rho \geq 1$
\begin{align}
\ol{\Psi} = \wt{\Psi}.
\end{align}
Using this streamfunction, we define the velocity field as
\begin{align}
\ol{V} = \nabla^\perp \ol{\Psi}.
\end{align}
The velocity field defined in such a way belongs to $C^{1, 1}$, i.e., the derivative is Lipschitz. We define the pressure field in the two regions separately as well. 
\begin{align}
\ol{P} = \ol{V}_1 - \frac{b^2}{2} (\ol{\Psi} - x_2)^2 - \frac{\ol{V}_1^2 + \ol{V}_2^2}{2} \quad \text{for} \quad \rho \leq 1, \qquad \qquad \ol{P} = \ol{V}_1 - \frac{\ol{V}_1^2 + \ol{V}_2^2}{2} \quad \text{for} \quad \rho \geq 1.
\end{align}
Finally, we define the rescaled variables for a given $r > 0$ as
\begin{align}
\ol{\Psi}_{r} = \ol{\Psi}\left(\frac{x}{r}\right), \quad 
\ol{V}_{r} = \frac{1}{r}\ol{V}\left(\frac{x}{r}\right), \quad
\ol{P}_{r} = \frac{1}{r^2}\ol{P}\left(\frac{x}{r}\right).
\end{align}
A simple computation shows
\begin{align}
- \frac{1}{r} \partial_1 \ol{V}_{r} + \ol{V}_{r} \cdot \nabla \ol{V}_{r} = - \nabla \ol{P}_{r}.
\label{principal bb: scaled lamb chaplygin eqn}
\end{align}






\subsection{Patching up}
The purpose of this section is to patch the Lamb--Chaplygin dipole with the periodic doublet to produce an approximate solution that is periodic on $\mathbb{R}^2$.
We start of with a few definitions. We define a domain of interest $\mathcal{D} \subseteq \mathbb{R}^2$ as
\begin{align}
\mathcal{D} = \left[-\frac{1}{2}, \frac{1}{2}\right]^2.
\end{align}
Next, given a function $f$ whose domain is $\mathbb{R}^2$ and $\supp f \subseteq \mathcal{D}$, we denote the periodized version of $f$ using $f^p$, which is defined as
\begin{align}
f^p(x_1, x_2) = \sum_{(m, n) \in \mathbb{Z}^2} f(x_1 + i, x_2 + j).
\end{align}
We let $\rchi: \mathbb{R}^2 \to \mathbb{R}$ to be a radial cutoff function such that $\rchi$ is $1$ in $B_2(0)$ and $0$ in $\mathbb{R}^2 \setminus B_3(0)$. We define a rescaled version of this cutoff function as 
\begin{align}
\rchi_r \coloneqq \rchi \left(\frac{x}{r}\right).
\end{align}
For the convenience of computations carried out in this section, we define
\begin{align}
\Gamma_r = \wh{\Psi}_r - \wt{\Psi}_r, \qquad \Lambda_r = \wh{\Phi}_r - \wt{\Phi}_r.
\end{align}
From the definitions (\ref{principal bb: period doublet stream pot}) and (\ref{principal bb: period doublet scaled}), it is clear that $|\Gamma_r|, |\Lambda_r| \lesssim r^3$ and $|\nabla \Gamma_r|, |\nabla \Lambda_r| \lesssim r^2$ when $x \in B_{3r}(0)$. We finally define our patched up velocity field $V^\ast$ as 
\begin{align}
V^\ast_r = (\ol{V}_r \rchi_r)^p + \wh{V}_r (1 - \rchi_r^p) \; -  (\Gamma_r \nabla^\perp \rchi_r)^p.
\label{principal bb: V star}
\end{align}
and a pressure
\begin{align}
P^\ast_r = (\ol{P}_r \rchi_r)^p  + \wh{P}_r (1 - \rchi_r^p).
\label{principal bb: P star}
\end{align}
The velocity field $V^\ast_r$ and pressure $P^\ast_r$ are periodic. Moreover, a simple calculation shows that $V^\ast_r$ is divergence-free.
\begin{proposition}[Patched solution]
For every $0 < r < \frac{1}{12}$, let $V^\ast_r$ and $P^\ast_r$ be as defined in (\ref{principal bb: V star}) and (\ref{principal bb: P star}) respectively. Then the velocity field $V_r^\ast \in C^{1, 1} (\mathbb{R}^2; \mathbb{R}^2)$ and the pressure $P_r^\ast \in C^{1, 1} ( \mathbb{R}^2; \mathbb{R})$ are doubly periodic in the directions $x_1$ and $x_2$ with period $1$ and obey
\begin{align}
- \frac{1}{r} \partial_1 V_r^\ast + V_r^\ast \cdot \nabla V_r^\ast = - \nabla P_r^\ast + \div(F_1), \\
\nabla \cdot V_r^\ast = 0, \qquad \qquad \qquad \qquad \qquad \qquad
\end{align}
where $F_1: \mathbb{R}^2 \to \mathbb{R}^2 \times \mathbb{R}^2$ is a symmetric tensor and is doubly periodic. Moreover, we have:
\begin{enumerate}[label = (\roman*)]
\item $\norm{F_1}_{L^1(\mathcal{D})} \leq C r^2$,
\item $\supp F_1 \subseteq B_{3 r}(0)$,
\item $\norm{V_r^\ast}_{L^1(\mathcal{D})} \leq C r |\log r|, \qquad \norm{V_r^\ast}_{L^p(\mathcal{D})} \leq C(p) r^{\frac{2}{p} - 1} \text{ for } p \in (1, \infty]$,
\item $\norm{\nabla \times V_r^\ast}_{L^p(\mathcal{D})} \leq C(p) r^{\frac{2}{p} - 2} \,$.
\end{enumerate}
\end{proposition}


% \begin{proposition}[Patching up]
% For every $0 < r < \frac{1}{12}$, there exist a vector field $V^\ast \in C^{1, 1} (\mathbb{T}^2; \mathbb{R}^2)$ and a pressure $P^\ast \in C^{1, 1} ( \mathbb{T}^2; \mathbb{R})$ such that
% \begin{align}
% \nabla \cdot V^\ast = 0, \\
% - \frac{1}{r} \partial_1 V^\ast + V^\ast \cdot \nabla V^\ast = - \nabla P^\ast + E^\ast,
% \end{align}
% where $E^\ast: \mathbb{T}^2 \to \mathbb{R}^2$ satisfies the following properties:
% \begin{enumerate}[label = (\roman*)]
% \item $E^\ast \in C^\infty(\mathbb{T}^2; \mathbb{R}^2)$,
% \item $\norm{E^\ast}_{L^\infty} \lesssim 1$,
% \item $\supp E^\ast \subseteq B_{3 r}(0,0)$,
% \item $\int_{\mathbb{T}^2} E^\ast \, {\rm d}x = 0$.
% \end{enumerate}
% In particular, we have
% \begin{align}
% \norm{\div^{-1} E^\ast}_{L^1} \lesssim r^3.
% \end{align}
% \end{proposition}





\begin{proof}
We set
\begin{align}
E^\ast \coloneqq - \frac{1}{r} \partial_1 V^\ast + V^\ast \cdot \nabla V^\ast + \nabla P^\ast.
\end{align}
From the periodicity of $V^\ast$ and $P^\ast$, it is clear that $E^\ast$ is periodic. Therefore, it sufficient to characterize $E^\ast$ on $\mathcal{D}$. We begin by noticing that the average of $E^\ast$ on $\mathcal{D}$ is zero. Next, we note that
\begin{align}
V^\ast = \ol{V}_r, \; P^\ast = \ol{P}_r  \text{ when } \; x \in B_{2 r}(0) \quad \text{and} \quad V^\ast = \wh{V}_r, \; P^\ast = \wh{P}_r  \text{ when }  x \in \mathcal{D} \setminus B_{3 r}(0). 
\end{align}
Therefore, from (\ref{principal bb: scaled period doublet eqn}) and (\ref{principal bb: scaled lamb chaplygin eqn}), we see that $E^\ast = 0$ in the complement of the annulus $B_{3 r}(0) \setminus B_{2r}(0)$. To estimate $E^\ast$ inside the annulus, we implicitly assume
that $x \in B_{3 r}(0) \setminus B_{2 r}(0)$ in rest of the calculation. Inside the annulus, we can write our velocity field and pressure as
\begin{align}
V^\ast = \wh{V}_r - \nabla^\perp \Gamma_r \rchi_r - \Gamma_r \nabla^\perp \rchi_r, \qquad P^\ast = \wh{P}_r + (\wt{P}_r - \wh{P}_r) \rchi_r.
\end{align}
From this we see that when $x \in B_{3 r}(0) \setminus B_{2 r}(0)$ the $E^\ast = \div F$,
%\begin{align}
%E^\ast = \div F = \div F_1 + \div F_2 + \div F_3,
%\end{align}
where
\begin{align}
F = - \frac{1}{r} \rchi_r \nabla^\perp \Gamma_r \otimes e_1  - \frac{1}{r}  \Gamma_r \nabla^\perp \rchi_r \otimes e_1 - 2 \, \text{Sym}(\wh{V}_r \otimes (\nabla^\perp \Gamma_r \rchi_r + \Gamma_r \nabla^\perp \rchi_r) ) + (\wt{P}_r - \wh{P}_r) \rchi_r \, \text{I}_{2 \times 2}.
\end{align}
%where
%\begin{align}
%F_1 \coloneqq - \frac{1}{r} \rchi \nabla^\perp \Gamma_r \otimes e_1  - \frac{1}{r}  \Gamma_r \nabla^\perp \rchi \otimes e_1,
%\end{align}
%\begin{align}
%F_2 \coloneqq - 2 \, \text{Sym}(\wh{V}_r \otimes (\nabla^\perp \Gamma_r \rchi + \Gamma_r \nabla^\perp \rchi) ),
%\end{align}
%\begin{align}
%F_3 \coloneqq (\wt{P}_r - \wh{P}_r) \rchi \, \text{I}_{2 \times 2}.
%\end{align}
Finally, from the definition of $\wh{V}_r$, $\wt{P}_r$ and $\wh{P}_r$ along with the following estimate
\begin{align}
\Gamma_{r} \lesssim r |x|^2, \qquad |\nabla \Gamma_{r}| \lesssim r |x| \qquad \text{when} \quad x \in B_{3 r}(0) \setminus B_{2 r}(0),
\end{align}
we obtain
\begin{align}
E^\ast \lesssim 1
\end{align}
inside the annulus. Finally, using the fact $E^\ast$ is periodic and  zero average on $\mathcal{D}$, we invert the divergence using lemma XX to conclude
\begin{align}
\norm{\div^{-1} E^\ast}_{L^1} \leq r^2.
\end{align}
Finally, we note that the estimates $(iii)$ and $(iv)$ are straightforward estimates.
%which gives
%\begin{align}
%\norm{F_1}_{L^\infty} \lesssim r \qquad \implies \qquad \norm{F_1}_{L^1} \lesssim r^3.
%\end{align}
%The $L^1$ norm is calculated in $\left[-\frac{1}{2}, \frac{1}{2}\right]^2$.
%Next, noting that 
%\begin{align}
%\wt{V}_r \lesssim \frac{1}{r} \qquad \text{when} \quad x \in B_{3 r}(0) \setminus B_{2 r}(0),
%\end{align}
%we obtain same estimates for the second term
%\begin{align}
%\norm{F_2}_{L^\infty} \lesssim r \qquad \implies \qquad \norm{F_2}_{L^1} \lesssim r^3.
%\end{align}
%Finally, we now calculate estimates on $F_3$. We note that
%\begin{align}
%\wh{P}_r - \wt{P}_r = \wh{P}^t_r - \wt{P}^t_r + \wh{P}^s_r - \wt{P}^s_r
%\end{align}
%We have that
%\begin{align}
%\wh{P}^t_r - \wt{P}^t_r = \frac{1}{r} \partial_1 (\wh{\Phi}^t_r - \wt{\Phi}^t_r) = \frac{1}{r} \partial \Lambda_r \qquad \implies \qquad \norm{\wh{P}^t_r - \wt{P}^t_r}_{L^\infty} \lesssim r.
%\end{align}
%We also have
%\begin{align}
%\wh{P}^s_r - \wt{P}^s_r = \frac{1}{2} \left[|\nabla \wh{\Phi}_r|^2 - |\nabla \wt{\Phi}_r|^2\right] = \nabla \wt{\Phi}_r \cdot \nabla \Gamma_r + \frac{1}{2} |\nabla \Gamma_r|^2 \qquad \implies \qquad \norm{\wh{P}^s_r - \wt{P}^s_r}_{L^\infty} \lesssim r.
%\end{align}
%In total we have
%\begin{align}
%\norm{F_3}_{L^\infty} \lesssim r \qquad \implies \qquad \norm{F_3}_{L^1} \lesssim r^3.
%\end{align}
%Finally, associating the periodic functions $V^\ast$, $P^\ast$ and $E^\ast$ with functions on torus, which we continue to call $V^\ast$, $P^\ast$ and $E^\ast$ completes the proof of the proposition.
\end{proof}




\begin{lemma}
Let $V_r^\ast \in C^{1, 1} (\mathbb{T}^2; \mathbb{R}^2)$ be as defined in (\ref{principal bb: V star}). Then
\begin{align}
\partial_r V^\ast_r = \frac{1}{r} V^\ast_r + \div(F_2),
\end{align}
where $F_2: \mathbb{T}^2 \to \mathbb{R}^2$ obeys:
\begin{align}
\norm{F_2}_{L^1} \lesssim r.
\end{align}
\end{lemma}
\begin{proof}
We work with the periodic version of $V^\ast$ defined on $\mathbb{R}^2$. We first note that on the domain $\mathcal{D}$, we have a few simple computations:
\begin{align}
\partial_r \ol{V}_r = - \frac{1}{r} \ol{V}_r - \frac{x}{r^2} \cdot \nabla \ol{V}_r = \frac{1}{r} \ol{V}_r - \div\left(\ol{V}_r \otimes \frac{x}{r}\right), \qquad 
\partial_r \wh{V}_r =  \frac{1}{r} \wh{V}_r, 
\qquad 
\partial_r \rchi_r =  -  \frac{x}{r} \cdot \nabla \rchi_r.
\end{align}
%To see this, we have the following simple computation
%\begin{align}
%\partial_r \ol{V}_r & = \partial_r \left(\frac{1}{r} \ol{V}\left(\frac{x}{r}\right)\right) \nonumber \\
%& = - \frac{1}{r^2} \ol{V} \left(\frac{x}{r}\right) - \frac{x}{r^3} \cdot \nabla \ol{V}\left(\frac{x}{r}\right) \nonumber \\
%& = - \frac{1}{r} \ol{V}_r - \frac{x}{r^2} \cdot \nabla \ol{V}_r \nonumber \\
%& = \frac{1}{r} \ol{V}_r - \div\left(\ol{V}_r \otimes \frac{x}{r}\right).
%\end{align}
%We also see that 
%\begin{align}
%\partial_r \wh{V}_r = \partial_r \left(r \wh{V}(x) \right) =  \frac{1}{r} \wh{V}_r,
%\end{align}
%and that
%\begin{align}
%\partial_r \rchi_r = - \frac{x}{r^2} \cdot (\nabla \rchi) \left(\frac{x}{r}\right) = -  \frac{x}{r} \cdot \nabla \rchi_r.
%\end{align}
Next, we define
\begin{align}
E_2 \coloneq \partial_r V^\ast_r - \frac{1}{r} V^\ast_r.
\end{align}
By construction, $E_2$ is periodic. Therefore, it is sufficient to analyze its behavior on $\mathcal{D}$.
%We note that when $x \in \mathcal{D}$ then
%\begin{align}
%V^\ast = \ol{V}_r \rchi_r + \wh{V}_r (1 - \rchi_r) + (\ol{\Psi}_r - \wh{\Psi}_r) \nabla^\perp \rchi.
%\end{align}
Therefore,
\begin{align}
E_2 & = - \rchi_r \div\left(\ol{V}_r \otimes \frac{x}{r}\right) - \nabla^\perp \Gamma_r \, \partial_r \rchi_r - \partial_r (\Gamma_r \nabla^\perp \rchi) + \frac{\Gamma_r}{r} \nabla^\perp \rchi \nonumber \\
& = - \div\left(\rchi_r \ol{V}_r \otimes \frac{x}{r}\right) + \ol{V}_r \left(\frac{|x|}{r} \frac{\partial \rchi_r}{\partial \rho}  \right) - \nabla^\perp (\Gamma_r \partial_r \rchi_r)  \eqcolon E_2^1 + E_2^2 + E_2^3.
\end{align}
First and last term are clearly zero average. From lemma ZZ, we also note that the second term is zero average as our cutoff function is radial. Furthermore, the support of all these lie in $B_{3 r}(0)$. Finally, we note that the magnitude of all these terms lead to 
\begin{align}
\norm{E^1_2}_{L^1} \lesssim 1, \qquad \norm{E^2_2}_{L^1} \lesssim 1, \qquad
\norm{E^3_2}_{L^1} \lesssim r^3.
\end{align}
Therefore, using lemma ZZ inverting the divergence leads to
the required result.
%\begin{align}
%E_2 = - \rchi_r \div\left(\ol{V}_r \otimes \frac{x}{r}\right) + (\ol{V}_r - \wh{V}_r) \partial_r \rchi_r + \partial_r [(\ol{\Psi}_r - \wh{\Psi}_r) \nabla^\perp \rchi] - \frac{(\ol{\Psi}_r - \wh{\Psi}_r)}{r} \nabla^\perp \rchi.
%\end{align}
%We first focus on the last three terms in the expression.
%\begin{align}
%\partial_r [\Gamma_r \nabla^\perp \rchi] = \frac{\Gamma_r}{r} \nabla^\perp \rchi + \Gamma_r \nabla^\perp \partial_r \rchi_r.
%\end{align}
%Therefore, we have
%\begin{align}
%(\ol{V}_r - \wh{V}_r) \partial_r \rchi_r + \partial_r [(\ol{\Psi}_r - \wh{\Psi}_r) \nabla^\perp \rchi] - \frac{(\ol{\Psi}_r - \wh{\Psi}_r)}{r} \nabla^\perp \rchi = \nabla^\perp [(\ol{\Psi}_r - \wh{\Psi}_r)  \partial_r \rchi_r]
%\end{align}
%We notice that
%\begin{align}
%\norm{(\ol{\Psi}_r - \wh{\Psi}_r)  \partial_r \rchi_r}_{L^\infty} \lesssim r^2.
%\end{align}
%Therefore,
%\begin{align}
%\norm{(\ol{\Psi}_r - \wh{\Psi}_r)  \partial_r \rchi_r}_{L^1} \lesssim r^4.
%\end{align}
%Now, we analyze the first term in the expression of $E_2$.
%\begin{align}
%- \rchi_r \div\left(\ol{V}_r \otimes \frac{x}{r}\right) = - \div \left(\rchi_r \ol{V}_r \otimes \frac{x}{r}\right) + \ol{V}_r \left[\frac{x}{r} \cdot \nabla \rchi_r \right]
%\end{align}
%We have the following estimate on the first term on RHS
%\begin{align}
%\norm{\rchi_r \ol{V}_r \otimes \frac{x}{r}}_{L^\infty} \lesssim \frac{1}{r}.
%\end{align}
%Therefore,
%\begin{align}
%\norm{\rchi_r \ol{V}_r \otimes \frac{x}{r}}_{L^1} \lesssim r.
%\end{align}
%For the last term, we see that
%\begin{align}
%\norm{\ol{V}_r \left[\frac{x}{r} \cdot \nabla \rchi_r \right]}_{L^1} \lesssim 1.
%\end{align}
%However, we see that the average of this term is zero and support lies in $B_{3 r}$. To see that we note
%\begin{align}
%x \cdot \nabla \rchi_r = |x| \rchi_r^\prime,
%\end{align}
%i.e., only radially dependent, whereas in the support of $\rchi^\prime_r$, we have
%\begin{align}
%\ol{V}_r = (\ol{V}_{r, 1}, \ol{V}_{r, 2}) = \left(\frac{r}{r^2} \cos 2 \theta, - \frac{r}{r^2} \sin 2 \theta\right).
%\end{align}
%Therefore, the antidivergence will gain us a factor of $r$ for this term.
\end{proof}


\begin{lemma}
We can write the velocity field $V_r^\ast$ from (\ref{principal bb: V star}) as
\begin{align}
V_r^\ast = W^p_r + \nabla \Pi + r \div(F_3),
\end{align}
where $W^p_r$ is the periodic version of $W_r$, $\Pi$ is a periodic function and $F_3$ is a symmetric tensor which obeys
\begin{align}
\norm{F_3}_{L^1} \lesssim r^3.
\end{align}
\end{lemma}
%\begin{lemma}
%Let $V_r^\ast \in C^{1, 1} (\mathbb{T}^2; \mathbb{R}^2)$ be as defined in (\ref{principal bb: V star}). Then
%\begin{align}
%\partial_r V^\ast_r = \frac{1}{r} Q^p_r + \nabla \Pi^\ast + \div(F_3),
%\end{align}
%where $Q^p_r$ is the periodic version of $Q_r$, $\Pi^\ast$ is a pressure and $F_3: \mathbb{T}^2 \to \mathbb{R}^2$ obeys:
%\begin{align}
%\norm{F_3}_{L^1} \lesssim r
%\end{align}
%and that
%\begin{align}
%\int_{\mathbb{T}^2} \frac{1}{r} Q^p_r = 
%\begin{bmatrix}
%\pi \\
%0
%\end{bmatrix}.
%\end{align}
%\end{lemma}
\begin{proof}
From XX(ref to def zeta) and YY(ref to rchi) we note that the supports of $\nabla \zeta_r$ and $\nabla \rchi_r$ are disjoint, a fact that we will use in several places in rest of the proof. Recall from (ref to dcomp.), we can write
\begin{align}
\rchi_r \ol{V}_r = \rchi_r W_r + \rchi_r \nabla(\zeta_r \wt{\Phi}_r) = W_r + \rchi_r \nabla(\zeta_r \wh{\Phi}_r) - \rchi_r \nabla(\zeta_r \Lambda_r)  \nonumber \\
= W_r + \rchi_r \nabla(\zeta_r \wh{\Phi}_r) -  \nabla(\rchi_r \zeta_r \Lambda_r) + \Lambda_r \nabla \rchi_r  ,
\end{align}
and we also have
\begin{align}
\wh{V}_r(1-\rchi_r) = (1 - \rchi_r)\nabla  \wh{\Phi}_r = (1 - \rchi_r)\nabla  (\zeta_r \wh{\Phi}_r). 
\end{align}
Combining above and using YY(ref to vel in D), inside $\mathcal{D}$, we can write 
\begin{align}
V^\ast & = W_r +  \nabla(\zeta_r \wh{\Phi}_r) -  \nabla(\rchi_r \zeta_r \Lambda_r) + \Lambda_r \nabla \rchi_r - \Gamma_r \nabla^\perp \rchi_r, \nonumber \\
& = W_r +  \nabla(\zeta_r \wh{\Phi}_r) -  \nabla(\rchi_r \zeta_r \Lambda_r) + \nabla (\rchi_r \Lambda_r) - \nabla^\perp \Gamma_r \rchi_r - \Gamma_r \nabla^\perp \rchi_r, \nonumber \\
& = W_r +  \nabla(\zeta_r \wh{\Phi}_r)  + \nabla (\, (1 - \zeta_r) \Lambda_r) - \nabla^\perp (\Gamma_r \rchi_r).
\end{align}
Next, we define
\begin{align}
F_3 \coloneqq \div^{-1}\left(\frac{1}{r} \nabla^\perp (\Gamma_r \rchi_r)^p\right), \qquad \text{and} \qquad E_3 = V^\ast - W_r^p - \nabla^\perp (\Gamma_r \rchi_r)^p,
\end{align}
From lemma ZZ $F_3$ obeys the estimate XX.  The function $E_3$ is periodic and using XX (avg. V), YY(avg. W) and ZZ(above calc), we see that
\begin{align}
\int_{\mathcal{D}} E_3 = 0, \qquad \text{and} \qquad \nabla \times E_3 = 0.
\end{align}
Therefore, there must exists a periodic function $\Pi$ such that 
\begin{align}
\nabla \Pi = E_3.
\end{align}




\end{proof}



























































































%Earlier
%Earlier
%Earlier
%Earlier
%Earlier
%Earlier

\section{Principal building block of our construction}
\label{sec: principal bb}
In this section, we describe the construction of the principal building block of our construction.
\subsection{A few preliminaries}
Let $v$ be a smooth velocity field given by a smooth streamfunction
\begin{align}
v = \nabla^\perp \phi.
\end{align}
Suppose that $\Omega \in \mathbb{R}^2$ is a connected domain whose boundary $\partial \Omega$ is a rectifiable curve. Then, we see that the integration of $v$ over $\Omega$ can be evaluated as
\begin{align}
\int_{\Omega} v dx = \int_{\Omega} \nabla^\perp \psi \, {\rm d} x = \int_{\partial \Omega} \psi \, n^\perp \, {\rm d} s,
\end{align}
which is a simple consequence of the divergence theorem. The integral on the right hand side make sense even if the velocity field $v$ is singular. Now we state a way to evaluate this integral in situations which are useful to us.
\begin{lemma}
Let $f(z) = \phi(x_1, x_2) + i \psi(x_1, x_2)$ be a complex function such that $\psi(x_1, x_2) = - \phi(x_2, x_1)$. If $\Omega = \left[-\frac{1}{2}, \frac{1}{2}\right]^2$ then
\begin{align}
\int_{\partial \Omega} \psi \, n^\perp \, {\rm d} s = \left( - \frac{1}{2} \operatorname{Im} \oint_{\partial \Omega} f(z) \, {\rm d}z,  \; \frac{1}{2} \operatorname{Re} \oint_{\partial \Omega} f(z) \, {\rm d}z \right)
\end{align}
\end{lemma}
The complex functions we will be using fall under this category.
% \begin{proof}
% Let $z(t) : [0, \ell] \to \mathbb{C}$ be the parameterization of $\gamma$ with arc length. 
% Writing $z(t) = x_1(t) + i x_2(t)$, we have
% \begin{align}
% \operatorname{Im} \oint_{\gamma} f(z) \, {\rm d}z & = \operatorname{Im} \int_0^\ell f(z(t)) z^\prime(t) \, {\rm d}t \nonumber \\
% & = \operatorname{Im} \int_0^\ell \left( \; \phi(x_1(t), x_2(t)) \, + \, i \psi(x_1(t), x_2(t)) \; \right) \; (x_1^\prime(t) + i x_2^\prime(t)) \; {\rm d}t \nonumber \\
% & = \int_0^\ell \phi(x_1(t), x_2(t)) \; x_2^\prime(t) \; {\rm d}t + \int_0^\ell \psi(x_1(t), x_2(t)) \; x_1^\prime(t) \; {\rm d}t \nonumber \\
% & = \int_0^\ell \psi(x_1(t), x_2(t)) \; ( x_1^\prime(t) - x_2^\prime(t) ) \; {\rm d}t
% \end{align}
% Similarly, we can also get
% \begin{align}
% \operatorname{Re} \oint_{\gamma} f(z) \, {\rm d}z 
% & = - \int_0^\ell \psi(x_1(t), x_2(t)) \; ( x_1^\prime(t) + x_2^\prime(t) ) \; {\rm d}t
% \end{align}
% \end{proof}

\subsection{A few simple facts about potential flows}
\label{sec: potential flow}
A potential flow describes a divergence-free velocity field given by potential of a scalar function $\phi:\mathbb{R}^2 \to \mathbb{R}$:
\begin{align}
v = \nabla \phi. 
\label{principal bb: potential flow}
\end{align}
As the velocity field is divergence, we can also use a streamfunction $\psi: \mathbb{R}^2 \to \mathbb{R}$ to write
\begin{align}
v = \nabla^\perp \psi.
\end{align}
It is easy to check that the potential $\phi$ and streamfunction $\psi$ are harmonic conjugate.
\begin{lemma}[Potential flow]
Let $\Omega \subseteq \mathbb{R}^2$ be an open and connected domain. Let $\psi, \phi : \Omega \to \mathbb{R}$ be harmonic conjugates. We define a velocity field $v : \Omega \to \mathbb{R}^2$ as 
\begin{align}
v = \nabla \phi = \nabla^\perp \psi,
\end{align}
and a pressure field $p : \Omega^2 \to \mathbb{R}$ as
\begin{align}
p = c \, \partial_1 \phi - \frac{|\nabla \phi|^2}{2}.
\end{align}
Then the velocity field $v$ and pressure $p$ solves
\begin{align}
- c \, \partial_1 v + v \cdot \nabla v = - \nabla p.
\end{align}
in $\Omega$.
\end{lemma}
From this lemma it is clear that 
\begin{align}
v(t, x) = v(x - c t e_1), \qquad p(t, x) = p(x - c t e_1)
\end{align}
solves the Euler equation.








\subsection{A doublet on $\mathbb{R}^2$}
\label{subsec: doublet}
The complex function $\wt{F} = \wt{\Phi} + i \wt{\Psi}$ that defines a doublet is 
\begin{align}
F(z) = \frac{1}{z}.
\end{align}
Next, we define a potential flow known as the doublet flow. A doublet can be thought of a flow generated by ``infinite'' source and sink of vorticity when placed infinitesimally close to each other. We define a potential $\wt{\Phi}: \mathbb{R}^2 \to \mathbb{R}$ as
\begin{align}
\wt{\Phi} = -\frac{x_1}{x_1^2 + x_2^2},
\end{align}
and a streamfunction
\begin{align}
\wt{\Psi} = \frac{x_2}{x_1^2 + x_2^2}.
\end{align}
It is clear that $\wt{\Phi}$ and $\wt{\Psi}$ are harmonic conjugate away from the origin. Based on which we define a velocity field
\begin{align}
\wt{V} = \nabla^\perp \wt{\Psi} = \nabla \wt{\Phi}.
\end{align}
Next, we define a pressure field
\begin{align}
\wt{P} = \wt{P}^t + \wt{P}^s
\end{align}
where
\begin{align}
\wt{P}^t = \partial_1 \wt{\Phi}, \qquad \wt{P}^s = - \frac{|\nabla \wt{\Phi}|^2}{2}.
\end{align}
It is then clear that
\begin{align}
- \partial_1 \wt{V} + \wt{V} \cdot \nabla \wt{V} = - \nabla \wt{P}.
\end{align}
\subsubsection{A scaled doublet on $\mathbb{R}^2$}
Let $\varepsilon > 0$. We define
\begin{align}
\wt{\Phi}_{\varepsilon} = \wt{\Phi}\left(\frac{x}{\varepsilon}\right), \quad 
\wt{\Psi}_{\varepsilon} = \wt{\Psi}\left(\frac{x}{\varepsilon}\right), \quad 
\wt{V}_{\varepsilon} = \frac{1}{\varepsilon}\wt{V}\left(\frac{x}{\varepsilon}\right), \quad
\wt{P}_{\varepsilon} = \frac{1}{\varepsilon^2}\wt{P}\left(\frac{x}{\varepsilon}\right).
\end{align}
It is clear that
\begin{align}
\wt{V}_{\varepsilon} = \varepsilon \wt{V}.
\end{align}
Moreover, we can write the scaled pressure as
\begin{align}
\wt{P}_{\varepsilon} = \wt{P}_{\varepsilon}^t + \wt{P}_{\varepsilon}^s,
\end{align}
where
\begin{align}
\wt{P}^t_{\varepsilon} = \frac{1}{\varepsilon^2}\wt{P}^t\left(\frac{x}{\varepsilon}\right) = \wt{P}^t(x)
\end{align}
and
\begin{align}
\wt{P}^s_{\varepsilon} = \frac{1}{\varepsilon^2}\wt{P}^s\left(\frac{x}{\varepsilon}\right) = \varepsilon^2 \wt{P}^s(x).
\end{align}
Finally, it is clear that
\begin{align}
- \frac{1}{\varepsilon} \partial_1 \wt{V}_{\varepsilon} + \wt{V}_{\varepsilon} \cdot \nabla \wt{V}_{\varepsilon} = - \nabla \wt{P}_{\varepsilon}.
\end{align}






\subsection{A periodic doublet on $\mathbb{R}^2$}
\label{subsec: periodic doublet}
Our goal in this section is to periodize the doublet from the previous section. We will define $\wh{\Phi}, \wh{\Psi}: \mathbb{R}^2 \to \mathbb{R}$. We first define
\begin{align}
\wh{\Psi}(x_1, x_2) 
= \lim_{N \to \infty} \sum_{\substack{(i, j) \in \mathbb{Z}^2 \\ |i|, \, |j| \leq N}}\wt{\Psi}(x_1 + i, x_2 + j) 
= \lim_{N \to \infty} \sum_{\substack{(i, j) \in \mathbb{Z}^2 \\ |i|, \, |j| \leq N}}  \frac{x_2 + j}{(x_1 + i)^2 + (x_2 + j)^2}.
\end{align}
It is not immediately apparent that the sum converges as we take $N \to \infty$. To show the convergence, we notice a few appropriate cancellations. To begin with, we have
\begin{align}
\lim_{N \to \infty} \sum_{\substack{(i, j) \neq (0, 0) \\ |i|, |j| \leq N}} \frac{j}{i^2 + j^2} = 0.
\end{align}
Using this we rewrite,
\begin{align}
\wh{\Psi} & = \wt{\Psi} + \lim_{N \to \infty} \sum_{\substack{(i, j) \in \mathbb{Z}^2 \\ (i, j) \neq (0, 0) \\ |i|, |j| \leq N }} \left( \frac{x_2 + j}{(x_1 + i)^2 + (x_2 + j)^2} - \frac{j}{i^2 + j^2} \right) \nonumber \\
& = \wt{\Psi} + \lim_{N \to \infty} \sum_{\substack{(i, j) \in \mathbb{Z}^2 \\ (i, j) \neq (0, 0) \\ |i|, |j| \leq N }} \frac{x_2 (i^2 - j^2) - 2 x_1 i j - j (x_1^2 + x_2^2)}{\left[(x_1 + i)^2 + (x_2 + j)^2\right] \left[i^2 + j^2\right]}
\end{align}
This sum still does not converge absolutely. But we note that
\begin{align}
\lim_{N \to \infty} \sum_{\substack{(i, j) \in \mathbb{Z}^2 \\ (i, j) \neq (0, 0) \\ |i|, |j| \leq N }} \frac{x_2 (i^2 - j^2)}{(i^2 + j^2)^4} = 0 \qquad \text{and} \qquad \lim_{N \to \infty} \sum_{\substack{(i, j) \in \mathbb{Z}^2 \\ (i, j) \neq (0, 0) \\ |i|, |j| \leq N }} \frac{x_1 i j}{(i^2 + j^2)^4} = 0.
\end{align}
Using which we finally define our streamfunction for the periodized doublet
\begin{align}
\wh{\Psi} & = \wt{\Psi} + \sum_{\substack{(i, j) \neq (0, 0) \\ (i, j) \in \mathbb{Z}^2}} \left( \frac{x_2 (i^2 - j^2) - 2 x_1 i j - j (x_1^2 + x_2^2)}{\left[(x_1 + i)^2 + (x_2 + j)^2\right] \left[i^2 + j^2\right]} - \frac{x_2 (i^2 - j^2)}{(i^2 + j^2)^4} + \frac{2 x_1 i j}{(i^2 + j^2)^4} \right) \nonumber \\
& = \wt{\Psi} + \sum_{\substack{(i, j) \neq (0, 0) \\ (i, j) \in \mathbb{Z}^2}}  \frac{(- x_2 (i^2 - j^2) + 2 x_1 i j ) (x_1^2 + x_2^2 + 2 x_1 i + 2 x_2 j) - j (i^2 + j^2) (x_1^2 + x_2^2)}{\left[(x_1 + i)^2 + (x_2 + j)^2\right] \left[i^2 + j^2\right]^2}. 
\end{align}
It is now clear that the sum converges absolutely (except for the singular points which are integer lattice $\mathbb{Z}^2$). We let
\begin{align}
\Gamma = \sum_{\substack{(i, j) \neq (0, 0) \\ (i, j) \in \mathbb{Z}^2}}  \frac{(- x_2 (i^2 - j^2) + 2 x_1 i j ) (x_1^2 + x_2^2 + 2 x_1 i + 2 x_2 j) - j (i^2 + j^2) (x_1^2 + x_2^2)}{\left[(x_1 + i)^2 + (x_2 + j)^2\right] \left[i^2 + j^2\right]^2}.
\end{align}
Both $\wt{\Psi}$ and $\Gamma$ are defined on $\mathbb{R}^2$ are not periodic function. Nor there some
$\wh{\Psi} = \wt{\Psi} + \Gamma$ is a periodic function. Similarly, we can define $\wh{\Phi}$, the harmonic conjugate, as
\begin{align}
\wh{\Phi} = \wt{\Phi} + \Lambda,
\end{align}
where
\begin{align}
\Lambda = - \sum_{\substack{(i, j) \neq (0, 0) \\ (i, j) \in \mathbb{Z}^2}}  \frac{(- x_1 (i^2 - j^2) + 2 x_2 i j ) (x_1^2 + x_2^2 + 2 x_2 i + 2 x_1 j) - j (i^2 + j^2) (x_1^2 + x_2^2)}{\left[(x_1 + i)^2 + (x_2 + j)^2\right] \left[i^2 + j^2\right]^2}.
\end{align}
Next we define the velocity field
\begin{align}
\wh{V} = \nabla \Phi = \nabla^\perp \Psi
\end{align}
and the pressure field
\begin{align}
\wh{P} = \wh{P}^t + \wh{P}^s,
\end{align}
where
\begin{align}
\wh{P}^t = \partial_1 \wh{\Phi} \qquad \wh{P}^s = - \frac{|\nabla \wh{\Phi}|^2}{2}.
\end{align}
It is then clear that
\begin{align}
- \partial_1 \wh{V} + \wh{V} \cdot \nabla \wh{V} = - \nabla \wh{P}.
\end{align}

\subsubsection{A scaled periodic doublet on $\mathbb{R}^2$}
Let $\varepsilon > 0$. We define
\begin{align}
\wh{\Phi}_{\varepsilon} = \varepsilon \wh{\Phi}, \quad 
\wh{\Psi}_{\varepsilon} = \varepsilon \wh{\Psi}, \quad 
\wh{V}_{\varepsilon} = \nabla^\perp \wh{\Psi}_{\varepsilon}, \quad
\wh{P}_{\varepsilon} = \wh{P}^t_\varepsilon + \wh{P}^s_\varepsilon,
\end{align}
where
\begin{align}
\wh{P}^t_\varepsilon = \frac{1}{\varepsilon} \partial_1 \wh{\Phi}_{\varepsilon} = \partial_1 \wh{\Phi} \qquad 
\wh{P}^s_\varepsilon = - \frac{|\nabla \wh{\Phi}_\varepsilon|^2}{2}.
\end{align}
Finally, it is clear that
\begin{align}
- \frac{1}{\varepsilon} \partial_1 \wh{V}_{\varepsilon} + \wh{V}_{\varepsilon} \cdot \nabla \wh{V}_{\varepsilon} = - \nabla \wh{P}_{\varepsilon}.
\end{align}
For later, purposes, we also define
\begin{align}
\Gamma_\varepsilon = \varepsilon \Gamma, \qquad \Lambda_\varepsilon = \varepsilon \Lambda.
\end{align}

\subsection{Desingularization of doublet on $\mathbb{R}^2$: The Lamb--Chaplygin dipole}
The Lamb--Chaplygin dipole consists of two regions: (i) $x_1^2 + x_2^2 \leq 1$ the desingularized region in which the vorticity is nonzero, (ii) $x_1^2 + x_2^2 \geq 1$ it is the potential flow given in section \ref{subsec: doublet}. In the polar coordinates we define
\begin{align}
\ol{\Psi} \coloneqq 
\begin{cases}
r \sin \theta - \frac{2 J_1(br)}{b J_0(b)} \sin \theta \qquad & \text{when} \quad r \leq 1 \\
\frac{\sin \theta}{r} \qquad & \text{when} \quad r \geq 1 
\end{cases}
\end{align}
Here $J_0$ and $J_1$ are the Bessel functions of first kind of zero and first order respectively. The number $b \approx 3.831705970\dots$ is the first non-trivial zero of $J_1$. It is clear that for $r \geq 1$
\begin{align}
\ol{\Psi} = \wt{\Psi}.
\end{align}
Using this streamfunction, we define the velocity field as
\begin{align}
\ol{V} = \nabla^\perp \ol{\Psi}.
\end{align}
The velocity field defined in such a way belongs to $C^{1, 1}$, i.e., the derivative is Lipschitz. We define the pressure field in the two regions separately as well. For $ r \leq 1$, we define
\begin{align}
\ol{P} = \ol{V}_1 - \frac{b^2}{2} (\ol{\Psi} - x_2)^2 - \frac{V_1^2 + V_2^2}{2}.
\end{align}
For $r \geq 1$, we define
\begin{align}
\ol{P} = \ol{V}_1 - \frac{V_1^2 + V_2^2}{2}.
\end{align}
A simple calculation then shows
\begin{align}
- \partial_1 \ol{V} + \ol{V} \cdot \nabla \ol{V} = - \nabla \ol{P}.
\end{align}

\subsubsection{A scaled Lamb--Chaplygin dipole}
Let $\varepsilon > 0$. We define
\begin{align}
\ol{\Psi}_{\varepsilon} = \ol{\Psi}\left(\frac{x}{\varepsilon}\right), \quad 
\ol{V}_{\varepsilon} = \frac{1}{\varepsilon}\ol{V}\left(\frac{x}{\varepsilon}\right), \quad
\ol{P}_{\varepsilon} = \frac{1}{\varepsilon^2}\ol{P}\left(\frac{x}{\varepsilon}\right).
\end{align}
Finally, it is clear that
\begin{align}
- \frac{1}{\varepsilon} \partial_1 \ol{V}_{\varepsilon} + \ol{V}_{\varepsilon} \cdot \nabla \ol{V}_{\varepsilon} = - \nabla \ol{P}_{\varepsilon}.
\end{align}






\subsection{Patching up}
In this section, we patch up the Lamb--Chaplygin dipole with periodic doublet to produce an approximate solution that is periodic. 

We first define a cutoff function $\rchi: \mathbb{R}^2 \to \mathbb{R}$ such that $\rchi$ is $1$ in $B_2(0)$ and $0$ in $\mathbb{R}^2 \setminus B_3(0)$. We define a rescaled version of this cutoff function as 
\begin{align}
\rchi_\varepsilon \coloneqq \rchi \left(\frac{x}{\varepsilon}\right).
\end{align}
Let's also define periodized version of this cutoff function
\begin{align}
\rchi_\varepsilon^p \coloneqq \sum_{(i, j) \in \mathbb{Z}^2} \rchi_\varepsilon(x_1 + i, x_2 + j).
\end{align}
Next, we define a velocity field as 
\begin{align}
V^\ast = \sum_{(i, j) \in \mathbb{Z}^2} (\ol{V}_\varepsilon \rchi_\varepsilon)(x_1 + i, x_2 + j) \; + \wh{V}_\varepsilon (1 - \rchi_\varepsilon^p) \; + \sum_{(i, j) \in \mathbb{Z}^2} \left((\ol{\Psi}_\varepsilon - \wh{\Psi}_\varepsilon) \nabla^\perp \rchi_\varepsilon\right)(x_1 + i, x_2 + j).
\label{principal bb: V star}
\end{align}
We also define a pressure
\begin{align}
P^\ast = \ol{P}_\varepsilon (1 - \rchi)  + \wh{P}_\varepsilon \rchi.
\label{principal bb: P star}
\end{align}
It is clear that the pressure is also periodic.
\begin{lemma}
The velocity field $V^\ast$ is $C^{1, 1}$, periodic and divergence-free.
\end{lemma}
\begin{proof}
It is clear by construction that $V^\ast$ is $C^{1, 1}$ and periodic. Now we perform a simple computation to see that $V^\ast$ is also divergence-free.
\begin{align}
\nabla \cdot V^\ast = \sum_{(i, j) \in \mathbb{Z}^2} (\ol{V}_\varepsilon \cdot \nabla \rchi_\varepsilon)(x_1 + i, x_2 + j) \; - \wh{V}_\varepsilon \cdot \nabla \rchi_\varepsilon^p \; + \sum_{(i, j) \in \mathbb{Z}^2} \left(\nabla (\ol{\Psi}_\varepsilon - \wh{\Psi}_\varepsilon) \cdot \nabla^\perp \rchi_\varepsilon\right)(x_1 + i, x_2 + j).
\end{align}
Using the fact that $\wh{V}_\varepsilon$ is periodic, we get that
\begin{align}
\wh{V}_\varepsilon \cdot \nabla \rchi^p = \wh{V}_\varepsilon \cdot \sum_{(i, j) \in \mathbb{Z}^2} \nabla \rchi_\varepsilon(x_1 + i, x_2 + j) = \sum_{(i, j) \in \mathbb{Z}^2} (\wh{V}_\varepsilon \cdot\nabla \rchi_\varepsilon)(x_1 + i, x_2 + j).
\end{align}
Therefore,
\begin{align}
\nabla \cdot V^\ast =  \sum_{(i, j) \in \mathbb{Z}^2} \left(\nabla (\ol{\Psi}_\varepsilon - \wh{\Psi}_\varepsilon ) \cdot \nabla^\perp \rchi_\varepsilon + \nabla^\perp (\ol{\Psi}_\varepsilon - \wh{\Psi}_\varepsilon) \cdot \nabla \rchi_\varepsilon\right)(x_1 + i, x_2 + j) = 0.
\end{align}
\end{proof}

The main result of this section is
\begin{proposition}[Patching up]
For every $0 < \varepsilon < \frac{1}{12}$, the velocity field $V_\varepsilon^\ast \in C^{1, 1} (\mathbb{T}^2; \mathbb{R}^2)$ and the pressure $P_\varepsilon^\ast \in C^{1, 1} ( \mathbb{T}^2; \mathbb{R})$ obey the following
\begin{align}
\nabla \cdot V_\varepsilon^\ast = 0, \\
- \frac{1}{\varepsilon} \partial_1 V_\varepsilon^\ast + V_\varepsilon^\ast \cdot \nabla V_\varepsilon^\ast = - \nabla P_\varepsilon^\ast + \div(F_\varepsilon^\ast),
\end{align}
where $F^\ast: \mathbb{T}^2 \to \mathbb{R}^2$. Moreover, we have:
\begin{enumerate}[label = (\roman*)]
\item $\norm{F_\varepsilon^\ast}_{L^1} \lesssim \varepsilon^3$,
\item $\norm{V_\varepsilon^\ast}_{L^2} \lesssim 1$,
\item $\norm{\nabla \times V_\varepsilon^\ast}_{L^1} \lesssim 1$.
\end{enumerate}
\end{proposition}


% \begin{proposition}[Patching up]
% For every $0 < \varepsilon < \frac{1}{12}$, there exist a vector field $V^\ast \in C^{1, 1} (\mathbb{T}^2; \mathbb{R}^2)$ and a pressure $P^\ast \in C^{1, 1} ( \mathbb{T}^2; \mathbb{R})$ such that
% \begin{align}
% \nabla \cdot V^\ast = 0, \\
% - \frac{1}{\varepsilon} \partial_1 V^\ast + V^\ast \cdot \nabla V^\ast = - \nabla P^\ast + E^\ast,
% \end{align}
% where $E^\ast: \mathbb{T}^2 \to \mathbb{R}^2$ satisfies the following properties:
% \begin{enumerate}[label = (\roman*)]
% \item $E^\ast \in C^\infty(\mathbb{T}^2; \mathbb{R}^2)$,
% \item $\norm{E^\ast}_{L^\infty} \lesssim 1$,
% \item $\supp E^\ast \subseteq B_{3 \varepsilon}(0,0)$,
% \item $\int_{\mathbb{T}^2} E^\ast \, {\rm d}x = 0$.
% \end{enumerate}
% In particular, we have
% \begin{align}
% \norm{\div^{-1} E^\ast}_{L^1} \lesssim \varepsilon^3.
% \end{align}
% \end{proposition}





\begin{proof}
Let $V^\ast_\varepsilon$ be the periodic velocity field on $\mathbb{R}^2$ from (\ref{principal bb: V star}) and $P^\ast_\varepsilon$ from (\ref{principal bb: P star}). We set
\begin{align}
E^\ast \coloneqq - \frac{1}{\varepsilon} \partial_1 V^\ast + V^\ast \cdot \nabla V^\ast + \nabla P^\ast,
\end{align}
which is our error. From the periodicity of $V^\ast$ and $P^\ast$, it is clear that $E^\ast$ is periodic. Therefore, it sufficient to characterize the behavior of $E^\ast$ on 
\begin{align}
\mathcal{D} \coloneqq \left[-\frac{1}{2}, \frac{1}{2}\right]^2.
\end{align}
We note that
\begin{align}
V^\ast = \ol{V}_\varepsilon, \qquad P^\ast = \ol{P}_\varepsilon \qquad \qquad \text{when} \quad x \in B_{2 \varepsilon}(0)
\end{align}
and 
\begin{align}
V^\ast = \wh{V}_\varepsilon, \qquad P^\ast = \wh{P}_\varepsilon \qquad \qquad \text{when} \quad x \in \mathcal{D} \setminus B_{3 \varepsilon}(0).
\end{align}
Therefore, 
\begin{align}
E^\ast = 0 \qquad \text{when} \quad x \in B_{2 \varepsilon}(0) \bigcup \left( \mathcal{D} \setminus B_{3 \varepsilon}(0) \right).
\end{align}
From the periodicity of $E^\ast$, we therefore have
\begin{align}
E^\ast = 0 \qquad \text{when} \quad  (x_1 + i, x_2 + j) \in B_{2 \varepsilon}(0) \bigcup \left( \mathcal{D} \setminus B_{3 \varepsilon}(0) \right).
\end{align}
To see where $E^\ast$ is nonzero, it is sufficient to focus on $\mathcal{D}$. In fact, we are only left with the region $B_{3 \varepsilon}(0) \setminus B_{2 \varepsilon}(0)$. Therefore, in rest of the calculation we implicitly assume that $x \in B_{3 \varepsilon}(0) \setminus B_{2 \varepsilon}(0)$.
\begin{align}
\Psi^\ast = \ol{\Psi}_\varepsilon (1 - \rchi)  + \wh{\Psi}_\varepsilon \rchi = \wt{\Psi}_\varepsilon + \Gamma_\varepsilon \rchi,
\end{align}
which gives
\begin{align}
V^\ast = \nabla^\perp \Psi^\ast = \wt{V}_\varepsilon + \nabla^\perp \Gamma_\varepsilon \rchi + \Gamma_\varepsilon \nabla^\perp \rchi.
\end{align}
Moreover, when $x \in B_{3 \varepsilon}(0) \setminus B_{2 \varepsilon}(0)$, we have
\begin{align}
P^\ast = \wt{P}_\varepsilon + (\wh{P}_\varepsilon - \wt{P}_\varepsilon) \rchi.
\end{align}
From this we see that 
\begin{align}
E^\ast = \div F = \div F_1 + \div F_2 + \div F_3,
\end{align}
where
\begin{align}
F_1 \coloneqq - \frac{1}{\varepsilon} \rchi \nabla^\perp \Gamma_\varepsilon \otimes e_1  - \frac{1}{\varepsilon}  \Gamma_\varepsilon \nabla^\perp \rchi \otimes e_1,
\end{align}
\begin{align}
F_2 \coloneqq \wt{V}_\varepsilon \otimes (\nabla^\perp \Gamma_\varepsilon \rchi + \Gamma_\varepsilon \nabla^\perp \rchi) + (\nabla^\perp \Gamma_\varepsilon \rchi + \Gamma_\varepsilon \nabla^\perp \rchi) \otimes \wt{V}_\varepsilon,
\end{align}
\begin{align}
F_3 \coloneqq (\wh{P}_\varepsilon - \wt{P}_\varepsilon) \rchi \, \text{I}_{2 \times 2}.
\end{align}
Next, we make quick estimates on all of these terms. First, note that
\begin{align}
\Gamma_{\varepsilon} \lesssim \varepsilon^3, \qquad |\nabla \Gamma_{\varepsilon}| \lesssim \varepsilon^2 \qquad \text{when} \quad x \in B_{3 \varepsilon}(0) \setminus B_{2 \varepsilon}(0),
\end{align}
which gives
\begin{align}
\norm{F_1}_{L^\infty} \lesssim \varepsilon \qquad \implies \qquad \norm{F_1}_{L^1} \lesssim \varepsilon^3.
\end{align}
The $L^1$ norm is calculated in $\left[-\frac{1}{2}, \frac{1}{2}\right]^2$.
Next, noting that 
\begin{align}
\wt{V}_\varepsilon \lesssim \frac{1}{\varepsilon} \qquad \text{when} \quad x \in B_{3 \varepsilon}(0) \setminus B_{2 \varepsilon}(0),
\end{align}
we obtain same estimates for the second term
\begin{align}
\norm{F_2}_{L^\infty} \lesssim \varepsilon \qquad \implies \qquad \norm{F_2}_{L^1} \lesssim \varepsilon^3.
\end{align}
Finally, we now calculate estimates on $F_3$. We note that
\begin{align}
\wh{P}_\varepsilon - \wt{P}_\varepsilon = \wh{P}^t_\varepsilon - \wt{P}^t_\varepsilon + \wh{P}^s_\varepsilon - \wt{P}^s_\varepsilon
\end{align}
We have that
\begin{align}
\wh{P}^t_\varepsilon - \wt{P}^t_\varepsilon = \frac{1}{\varepsilon} \partial_1 (\wh{\Phi}^t_\varepsilon - \wt{\Phi}^t_\varepsilon) = \frac{1}{\varepsilon} \partial \Lambda_\varepsilon \qquad \implies \qquad \norm{\wh{P}^t_\varepsilon - \wt{P}^t_\varepsilon}_{L^\infty} \lesssim \varepsilon.
\end{align}
We also have
\begin{align}
\wh{P}^s_\varepsilon - \wt{P}^s_\varepsilon = \frac{1}{2} \left[|\nabla \wh{\Phi}_\varepsilon|^2 - |\nabla \wt{\Phi}_\varepsilon|^2\right] = \nabla \wt{\Phi}_\varepsilon \cdot \nabla \Gamma_\varepsilon + \frac{1}{2} |\nabla \Gamma_\varepsilon|^2 \qquad \implies \qquad \norm{\wh{P}^s_\varepsilon - \wt{P}^s_\varepsilon}_{L^\infty} \lesssim \varepsilon.
\end{align}
In total we have
\begin{align}
\norm{F_3}_{L^\infty} \lesssim \varepsilon \qquad \implies \qquad \norm{F_3}_{L^1} \lesssim \varepsilon^3.
\end{align}
Finally, associating the periodic functions $V^\ast$, $P^\ast$ and $E^\ast$ with functions on torus, which we continue to call $V^\ast$, $P^\ast$ and $E^\ast$ completes the proof of the proposition.
\end{proof}




\begin{lemma}
Let $V_\varepsilon^\ast \in C^{1, 1} (\mathbb{T}^2; \mathbb{R}^2)$ be as defined in (\ref{principal bb: V star}). Then
\begin{align}
\partial_\varepsilon V^\ast_\varepsilon = \frac{1}{\varepsilon} V^\ast_\varepsilon + \div(F_2),
\end{align}
where $F_2: \mathbb{T}^2 \to \mathbb{R}^2$ obeys:
\begin{align}
\norm{F_2}_{L^1} \lesssim \varepsilon.
\end{align}
\end{lemma}
\begin{proof}
We work with the periodic version of $V^\ast$ defined on $\mathbb{R}^2$. We first note that
\begin{align}
\partial_\varepsilon \ol{V}_\varepsilon = \frac{1}{\varepsilon} \ol{V}_\varepsilon - \div\left(\ol{V}_\varepsilon \otimes \frac{x}{\varepsilon}\right).
\end{align}
To see this, we have the following simple computation
\begin{align}
\partial_\varepsilon \ol{V}_\varepsilon & = \partial_\varepsilon \left(\frac{1}{\varepsilon} \ol{V}\left(\frac{x}{\varepsilon}\right)\right) \nonumber \\
& = - \frac{1}{\varepsilon^2} \ol{V} \left(\frac{x}{\varepsilon}\right) - \frac{x}{\varepsilon^3} \cdot \nabla \ol{V}\left(\frac{x}{\varepsilon}\right) \nonumber \\
& = - \frac{1}{\varepsilon} \ol{V}_\varepsilon - \frac{x}{\varepsilon^2} \cdot \nabla \ol{V}_\varepsilon \nonumber \\
& = \frac{1}{\varepsilon} \ol{V}_\varepsilon - \div\left(\ol{V}_\varepsilon \otimes \frac{x}{\varepsilon}\right).
\end{align}
We also see that 
\begin{align}
\partial_\varepsilon \wh{V}_\varepsilon = \partial_\varepsilon \left(\varepsilon \wh{V}(x) \right) =  \frac{1}{\varepsilon} \wh{V}_\varepsilon,
\end{align}
and that
\begin{align}
\partial_\varepsilon \rchi_\varepsilon = - \frac{x}{\varepsilon^2} \cdot (\nabla \rchi) \left(\frac{x}{\varepsilon}\right) = -  \frac{x}{\varepsilon} \cdot \nabla \rchi_\varepsilon.
\end{align}
Next, we let
\begin{align}
E_2 \coloneq \partial_\varepsilon V^\ast_\varepsilon - \frac{1}{\varepsilon} V^\ast_\varepsilon.
\end{align}
By construction, $E_2$ is periodic. Therefore, it is sufficient to analyze its behavior in 
\begin{align}
\mathcal{D} = \left[-\frac{1}{2}, \frac{1}{2}\right]^2.
\end{align}
We note that when $x \in \mathcal{D}$ then
\begin{align}
V^\ast = \ol{V}_\varepsilon \rchi_\varepsilon + \wh{V}_\varepsilon (1 - \rchi_\varepsilon) + (\ol{\Psi}_\varepsilon - \wh{\Psi}_\varepsilon) \nabla^\perp \rchi.
\end{align}
Therefore,
\begin{align}
E_2 = - \rchi_\varepsilon \div\left(\ol{V}_\varepsilon \otimes \frac{x}{\varepsilon}\right) + (\ol{V}_\varepsilon - \wh{V}_\varepsilon) \partial_\varepsilon \rchi_\varepsilon + \partial_\varepsilon [(\ol{\Psi}_\varepsilon - \wh{\Psi}_\varepsilon) \nabla^\perp \rchi] - \frac{(\ol{\Psi}_\varepsilon - \wh{\Psi}_\varepsilon)}{\varepsilon} \nabla^\perp \rchi.
\end{align}
We first focus on the last three terms in the expression.
\begin{align}
\partial_\varepsilon [(\ol{\Psi}_\varepsilon - \wh{\Psi}_\varepsilon) \nabla^\perp \rchi] = \frac{(\ol{\Psi}_\varepsilon - \wh{\Psi}_\varepsilon)}{\varepsilon} \nabla^\perp \rchi + (\ol{\Psi}_\varepsilon - \wh{\Psi}_\varepsilon) \nabla^\perp \partial_\varepsilon \rchi_\varepsilon.
\end{align}
Therefore, we have
\begin{align}
(\ol{V}_\varepsilon - \wh{V}_\varepsilon) \partial_\varepsilon \rchi_\varepsilon + \partial_\varepsilon [(\ol{\Psi}_\varepsilon - \wh{\Psi}_\varepsilon) \nabla^\perp \rchi] - \frac{(\ol{\Psi}_\varepsilon - \wh{\Psi}_\varepsilon)}{\varepsilon} \nabla^\perp \rchi = \nabla^\perp [(\ol{\Psi}_\varepsilon - \wh{\Psi}_\varepsilon)  \partial_\varepsilon \rchi_\varepsilon]
\end{align}
We notice that
\begin{align}
\norm{(\ol{\Psi}_\varepsilon - \wh{\Psi}_\varepsilon)  \partial_\varepsilon \rchi_\varepsilon}_{L^\infty} \lesssim \varepsilon^2.
\end{align}
Therefore,
\begin{align}
\norm{(\ol{\Psi}_\varepsilon - \wh{\Psi}_\varepsilon)  \partial_\varepsilon \rchi_\varepsilon}_{L^1} \lesssim \varepsilon^4.
\end{align}
Now, we analyze the first term in the expression of $E_2$.
\begin{align}
- \rchi_\varepsilon \div\left(\ol{V}_\varepsilon \otimes \frac{x}{\varepsilon}\right) = - \div \left(\rchi_\varepsilon \ol{V}_\varepsilon \otimes \frac{x}{\varepsilon}\right) + \ol{V}_\varepsilon \left[\frac{x}{\varepsilon} \cdot \nabla \rchi_\varepsilon \right]
\end{align}
We have the following estimate on the first term on RHS
\begin{align}
\norm{\rchi_\varepsilon \ol{V}_\varepsilon \otimes \frac{x}{\varepsilon}}_{L^\infty} \lesssim \frac{1}{\varepsilon}.
\end{align}
Therefore,
\begin{align}
\norm{\rchi_\varepsilon \ol{V}_\varepsilon \otimes \frac{x}{\varepsilon}}_{L^1} \lesssim \varepsilon.
\end{align}
For the last term, we see that
\begin{align}
\norm{\ol{V}_\varepsilon \left[\frac{x}{\varepsilon} \cdot \nabla \rchi_\varepsilon \right]}_{L^1} \lesssim 1.
\end{align}
However, we see that the average of this term is zero and support lies in $B_{3 \varepsilon}$. To see that we note
\begin{align}
x \cdot \nabla \rchi_\varepsilon = |x| \rchi_\varepsilon^\prime,
\end{align}
i.e., only radially dependent, whereas in the support of $\rchi^\prime_\varepsilon$, we have
\begin{align}
\ol{V}_\varepsilon = (\ol{V}_{\varepsilon, 1}, \ol{V}_{\varepsilon, 2}) = \left(\frac{\varepsilon}{r^2} \cos 2 \theta, - \frac{\varepsilon}{r^2} \sin 2 \theta\right).
\end{align}
Therefore, the antidivergence will gain us a factor of $\varepsilon$ for this term.
\end{proof}

\begin{lemma}
Let $V_\varepsilon^\ast \in C^{1, 1} (\mathbb{T}^2; \mathbb{R}^2)$ be as defined in (\ref{principal bb: V star}). Then
\begin{align}
\partial_\varepsilon V^\ast_\varepsilon = \frac{1}{\varepsilon} Q^p_\varepsilon + \nabla \Pi^\ast + \div(F_3),
\end{align}
where $Q^p_\varepsilon$ is the periodic version of $Q_\varepsilon$, $\Pi^\ast$ is a pressure and $F_3: \mathbb{T}^2 \to \mathbb{R}^2$ obeys:
\begin{align}
\norm{F_3}_{L^1} \lesssim \varepsilon
\end{align}
and that
\begin{align}
\int_{\mathbb{T}^2} \frac{1}{\varepsilon} Q^p_\varepsilon = 
\begin{bmatrix}
\pi \\
0
\end{bmatrix}.
\end{align}
\end{lemma}
\begin{proof}
To prove this lemma, we only need to show
\begin{align}
\frac{1}{\varepsilon} V^\ast = \frac{1}{\varepsilon} Q^p_\varepsilon + \nabla \Pi^\ast + \div F_4,
\end{align}
\begin{align}
\norm{F_4}_{L^1} \lesssim \varepsilon^2.
\end{align}
We set 
\begin{align}
E_4 = \frac{1}{\varepsilon} V^\ast - \frac{1}{\varepsilon} Q^p_\varepsilon
\end{align}
We restrict ourselves to $\mathcal{D}$. We have
\begin{align}
E_4 = 
\end{align}
\end{proof}


\subsubsection{Building Block velocity field}
% {\color{blue}MARIA: rename sections Building block with constant speed (here there must be a big, self contained proposition)

% Building blocks with time dependent velocity 
% (mainly contains Prop 4.2 and its proof, which should rely only on the Prop of the previous section)

% Keep only r(x(t)) instead of $\epsilon a^2$.
% }


% We now define our building block vector field




% \bigskip
% \bigskip
% {\color{red}Maria you should start from here}
% \bigskip
% \bigskip
Let $r: \mathbb{T}^2 \to (0,\infty)$ be a smooth spatial function satisfying $\| r \|_{L_x^\infty} < 1/9$ and let $\eta: \mathbb{R} \to (0,\infty)$ be a smooth function in time. Assume $x: \R \to \mathbb{T}^2$ be the trajectory that solves
\begin{align}
\begin{cases}
    x'(t) = \frac{\eta(t)}{r(x(t))} \xi,
    \\
    x(0) = x_0.
\end{cases}
\end{align}
We define our building block vector field to be
\begin{align}
V(x,t) = \eta(t) \, V^\ast_{r(t)}(x - x(t)).
\end{align}
In the following proposition, we use the shorthand notations: $r(t) \coloneq r(x(t))$ and $\nabla r(t) \coloneq \nabla r (x(t))$. 





% From this, it is clear that
% \begin{align}
% \frac{d \varepsilon(t)}{dt} = u_0 \frac{\nabla a^2(p(t))}{a^2(p(t))}.
% \end{align}
% Next, we outline the properties of our building block velocity field $V$.

\begin{proposition}[Building block vector field]
Let the functions $r$ and $\eta$ be as defined above and let $\xi \in \R$ with $|\xi| = 1$. There exists $V, W \in C^\infty (\mathbb{T}^2 \times \R; \mathbb{R}^2)$, a pressure $P\in C^\infty ( \mathbb{T}^2 \times \R; \mathbb{R})$ and a symmetric tensor $F\in C^\infty(\mathbb{T}^2 \times \R; \mathbb{R}^{2\times 2})$ that solves
\begin{align}
\partial_t V + \div(V\otimes V) = - \nabla P +  \left(\eta (t) \frac{\nabla r(t) \cdot \xi}{r(t)}\right) W + \div(F),
\\
\nabla \cdot V = 0, \qquad \qquad \qquad \qquad \qquad \qquad
\end{align}
and obeys the following properties:
\begin{enumerate}[label = (\roman*)]
\item $\norm{F}_{L_t^\infty L_x^1} \le C (\norm{\eta}_{L_t^\infty}^2 \norm{\nabla r}_{L_x^\infty} + \norm{\eta}_{L_t^\infty} \norm{r}_{L_x^\infty} + \norm{\eta^\prime}_{L_t^\infty} \norm{r}_{L_x^\infty})$,
\item the velocity field $V$ satisfies
\begin{align}
\| V(\cdot, t) \|_{L_x^1} \leq C \, \norm{\eta}_{L_t^\infty} \, r(t) \, |\log r(t)|, \quad \| V(\cdot, t) \|_{L_x^p} \leq C(p) \, \norm{\eta}_{L_t^\infty} \, r(t)^{\frac{2}{p}-1} \text{ for } p \in (1, \infty],
\end{align}
\item for all $p \in [1, \infty]$,
\begin{align}
     \| W(\cdot, t) \|_{L_x^p} +  r(t)\| \nabla \times V(\cdot, t) \|_{L_x^p}
    \le C(p) \, \norm{\eta}_{L_t^\infty} \, r(t)^{\frac{2}{p}-1}\, ,
\end{align}
\item finally 
\begin{align}
\supp W(\cdot, t) \subseteq B_{r(t)}(x(t)), \qquad    \frac{1}{r(t)} \int_{\mathbb{T}^2} W(x,t)\, {\rm d} x = \xi .
\end{align}






\end{enumerate}
\end{proposition}




% \subsubsection{Building Block velocity field}
% All the required details are here but this section needs to be organized properly.
% Finally, it is time to define the building block velocity field:
% \begin{align}
% V = \frac{1}{a^2} V^\ast \left(\frac{1}{a^2} \left(x - \frac{p(t)}{\varepsilon} e_1\right)\right)
% \end{align}
% and the pressure
% \begin{align}
% P = \frac{1}{a^4} P^\ast \left(\frac{1}{a^2} \left(x - \frac{p(t)}{\varepsilon} e_1\right)\right)
% \end{align}
% where
% \begin{align}
% \frac{d p(t)}{d t} = \frac{1}{\varepsilon a^2(p(t))} e_1.
% \end{align}
% We immediately see that $V$ is divergence-free. We also see that $V$ satisfies
% \begin{align}
% \nabla \cdot V^\ast = 0, \\
% \partial_t V + V \cdot \nabla V = - \nabla (P + P_1) + E + F + G + \frac{\nabla a^2}{a^2} Q,
% \end{align}
% Here,
% \begin{align}
% E = \frac{1}{a^2} E^\ast \left(\frac{1}{a^2} \left(x - \frac{p(t)}{\varepsilon} e_1\right)\right)
% \end{align}
% and $F$ is a new error term given by
% \begin{align}
% F = - \frac{\nabla a^2}{\varepsilon a^6} \div \left(V \otimes \left(x - \frac{p(t)}{\varepsilon} e_1\right)\right).
% \end{align}
% This gives
% \begin{align}
% \norm{\div^{-1} F}_{L^1} \lesssim |\nabla a^2| \; \varepsilon^2
% \end{align}
% $G$ is yet another error term
% \begin{align}
% G = \frac{\nabla a^2}{\varepsilon a^6} \left[ \nabla^\perp \ol{\Psi}_\varepsilon (1 - \rchi) + ( \wh{\Psi}_\varepsilon - \ol{\Psi}_\varepsilon) \nabla^\perp \rchi + (\wt{\Phi}_\varepsilon - \wh{\Phi}_\varepsilon) \nabla \rchi \right]_{\left(\frac{x}{a^2} - \frac{p(t)}{\varepsilon a^2} e_1\right)}
% \end{align}
% This gives
% \begin{align}
% \norm{\div^{-1} G}_{L^1} \lesssim \frac{|\nabla a^2|}{a^8} \; \varepsilon
% \end{align}
% The pressure $P_1$ is given by
% \begin{align}
% P_1 = \frac{1}{\varepsilon} \Bigl[  \rchi \wh{\Phi}_\varepsilon \Bigr]_{\left(\frac{x}{a^2} - \frac{p(t)}{\varepsilon a^2} e_1\right)}
% \end{align}
% The term $Q$ is given by
% \begin{align}
% Q = - \frac{a^4}{\varepsilon} \Bigl[ \nabla \rchi \wt{\Phi}_\varepsilon \Bigr]_{\left(\frac{x}{a^2} - \frac{p(t)}{\varepsilon a^2} e_1\right)}
% \end{align}
% We see that
% \begin{align}
% \int_{\mathbb{T}^2} Q \, {\rm d} x = 
% \begin{bmatrix}
% \pi \\
% 0
% \end{bmatrix}.
% \end{align}

==> Figures/Old_Material/Anuj_Notes/old_new_bb_lamb_chaplygin.tex <==
\section{Principal building block of our construction}
\label{sec: principal bb}
\subsection{A doublet on $\mathbb{R}^2$}
\label{subsec: doublet}
A steady doublet is a potential flow on $\mathbb{R}^2$ given by
\begin{align}
V^{d}_s = \nabla \Phi^d_s,
\end{align}
where the potential $\Phi^d_s$ is given by
\begin{align}
\Phi^d_s = -\frac{x_1}{x_1^2 + x_2^2}.
\end{align}
A doublet can be thought of a flow generated by ``infinite'' source and sink of vorticity when placed infinitesimally close to each other. In the component form, we have
\begin{align}
V^d_s = (V^d_{s, 1}, V^d_{s, 2}) = \left(\frac{x_1^2 - x_2^2}{(x_1^2 + x_2^2)^2}, \frac{2 x_1 x_2}{(x_1^2 + x_2^2)^2}\right).
\end{align}
The streamfunction $\Psi^d_s$, such that $V^d_s = \nabla^\perp \Psi^d_s = (\partial_{x_2} \Psi^d_s, -\partial_{x_1} \Psi^d_s)$, is given by
\begin{align}
\Psi^d_s = \frac{x_2}{x_1^2 + x_2^2}.
\end{align}
Because the velocity field $V^d$ is generated by a potential, therefore it is irrotational. The velocity field $V^d$ solves the Euler equation with pressure term
\begin{align}
\Pi^d_s = - \frac{1}{2} |V^d_s|^2 = - \frac{1}{2 (x_1^2 + x_2^2)^2}.
\end{align}
\begin{lemma}[Translation of irrotational flow]
Let a vector field $V$ be irrotational flow solving steady Euler then a velocity field $V(x - \xi t)$ also solves Euler for any $\xi \in \mathbb{R}^2$.
\end{lemma}
From this lemma we see that 
\begin{align}
V^d(t, x) = \nabla (\Phi^d_s(x_1 -t, x_2)) = \nabla^\perp (\Psi^d_s(x_1 - t, x_2))
\end{align}
also solves Euler with pressure
\begin{align}
\Pi^d = \wt{\Pi}^d(t, x_1, x_2)  + \Pi^d_s(x_1 - t, x_2), \qquad \text{where} \quad \wt{\Pi}^d = V_1^d.
\end{align}


\subsection{A doublet on $\mathbb{T}^2$}
\label{subsec: doublet on torus}
We can periodize the doublet defined in previous section. We use the following streamfunction
\begin{align}
\Psi^{pd}_s = \sum_{(i, j) \in \mathbb{Z}^2}\Psi^{d}_s(x_1 + i, x_2 + j) = \sum_{(i, j) \in \mathbb{Z}^2} \frac{x_2 + j}{(x_1 + i)^2 + (x_2 + j)^2}.
\end{align}
The sum on the right hand side does not converge but we notice appropriate cancellation. In particular, we have
\begin{align}
\lim_{N \to \infty} \sum_{\substack{(i, j) \neq (0, 0) \\ |i|, |j| \leq N}} \frac{j}{i^2 + j^2} = 0.
\end{align}
Using this we redefine,
\begin{align}
\Psi^{pd}_s & = \Psi^d_s + \sum_{(\substack{(i, j) \neq (0, 0) \\ (i, j) \in \mathbb{Z}^2}} \left( \frac{x_2 + j}{(x_1 + i)^2 + (x_2 + j)^2} - \frac{j}{i^2 + j^2} \right) \nonumber \\
& = \Psi^d_s + \sum_{\substack{(i, j) \neq (0, 0) \\ (i, j) \in \mathbb{Z}^2}} \frac{x_2 (i^2 - j^2) - 2 x_1 i j - j (x_1^2 + x_2^2)}{\left[(x_1 + i)^2 + (x_2 + j)^2\right] \left[i^2 + j^2\right]}
\end{align}
This sum still does not converge absolutely. But we note that
\begin{align}
\lim_{N \to \infty} \sum_{\substack{(i, j) \neq (0, 0) \\ |i|, |j| \leq N}} \frac{x_2 (i^2 - j^2)}{(i^2 + j^2)^4} = 0 \qquad \text{and} \qquad \lim_{N \to \infty} \sum_{\substack{(i, j) \neq (0, 0) \\ |i|, |j| \leq N}} \frac{x_1 i j}{(i^2 + j^2)^4} = 0
\end{align}
Using which we finally define our streamfunction for the periodized doublet
\begin{align}
\Psi^{pd}_s & = \Psi^d_s + \sum_{\substack{(i, j) \neq (0, 0) \\ (i, j) \in \mathbb{Z}^2}} \left( \frac{x_2 (i^2 - j^2) - 2 x_1 i j - j (x_1^2 + x_2^2)}{\left[(x_1 + i)^2 + (x_2 + j)^2\right] \left[i^2 + j^2\right]} - \frac{x_2 (i^2 - j^2)}{(i^2 + j^2)^4} + \frac{2 x_1 i j}{(i^2 + j^2)^4} \right) \nonumber \\
& = \Psi^d_s + \sum_{\substack{(i, j) \neq (0, 0) \\ (i, j) \in \mathbb{Z}^2}}  \frac{(- x_2 (i^2 - j^2) + 2 x_1 i j ) (x_1^2 + x_2^2 + 2 x_1 i + 2 x_2 j) - j (i^2 + j^2) (x_1^2 + x_2^2)}{\left[(x_1 + i)^2 + (x_2 + j)^2\right] \left[i^2 + j^2\right]^2}. 
\end{align}
In rest of the computation the exact expression is not important but we wrote it here for convenience. We define the velocity field as
\begin{align}
V^{pd}_s = \nabla^\perp \Psi^{pd}_s.
\end{align}
which solves the Euler equation with the pressure term
\begin{align}
\Pi^{pd}_s = - \frac{1}{2} |V^{pd}_s|^2.
\end{align}
Next, we define translating periodized doublet
\begin{align}
\Psi^{pd}(t,x) = \Psi^{pd}_s(x_1 - t, x_2)
\end{align}
The corresponding velocity field is
\begin{align}
V^{pd}_s(t, x) = \nabla^\perp \Psi^{pd}.
\end{align}
and the pressure
\begin{align}
\Pi^{pd} = \wt{\Pi}^{pd} - \frac{1}{2} |V^{pd}|^2, \qquad \text{where} \quad \wt{\Pi}^{pd} = V^{pd}_1.
\end{align}

\subsection{Desingularization of doublet on $\mathbb{R}^2$: Lamb--Chaplygin dipole}
The Lamb--Chaplygin dipole consists of two regions: (i) $x_1^2 + x_2^2 \leq 1$ the desingularized region in which the vorticity is nonzero, (ii) $x_1^2 + x_2^2 \geq 1$ it is the potential flow given in section \ref{subsec: doublet}. In the polar coordinates we define
\begin{align}
\Psi^{lc}_s \coloneqq 
\begin{cases}
r \sin \theta - \frac{2 J_1(br)}{b J_0(b)} \sin \theta \qquad & \text{when} \quad r \leq 1 \\
\frac{\sin \theta}{r} \qquad & \text{when} \quad r \geq 1 
\end{cases}
\end{align}
Here $J_0$ and $J_1$ are the Bessel functions of first kind of zero and first order respectively. The number $b \approx 3.831705970\dots$ is the first non-trivial zero of $J_1$. The velocity field in such a way belongs to $C^{1, 1}$, i.e., the derivative is Lipschitz.

==> Figures/Old_Material/Elia_Notes/nonunique-Euler2D-6.tex <==











%numbers








\section{Introduction}\subsection{Strategy of proof}



             


\section{Preliminaries}

Let $\tau = K T_\xi$ be an integer multiple of the period $T_\xi$, i.e., $K\in \mathbb{Z}$, $K\ge 1$. We define the time projector:
\begin{equation}
	P_\tau f(t) := \frac{1}{\tau}\int_{k\tau}^{(k+1)\tau} f(s)\, ds \, , \quad \text{for every $t\in [k\tau, (k+1)\tau)$}\, ,
\end{equation}
where $f: \mathbb{R} \to \mathbb{R}$.






\section{Moving jets}

The building blocks of our construction consist of \textit{moving jets} with non-constant velocity, whose centers follow a periodic trajectory \(x: \mathbb{R} \to \mathbb{T}^2\) in the two-dimensional torus. They are shaped as ellipsoids with axes depending on time.
The trajectory of the center solves a differential equation
\begin{equation}
	x'(t) = \mu(x(t)) \xi \, ,
\end{equation}
where \(\xi \in \mathbb{R}^2\) is a unitary vector with rationally dependent components. The velocity \(\mu\) is a positive smooth function designed in terms of \(R_q\), the error in the previous stage of the iteration.





\subsection{The static jet}
We begin by building the profile of the jet. Let us fix parameters $r_\perp \ll r_\parallel\ll 1$ and $\xi \in \mathbb{R}^2$ unitary with rationally dependent components.



Consider functions $\Phi, \psi: \RR\to \RR$ supported in $(-1,1)$, we set $\phi := -\Phi'''$ and assume $\int \psi^2 = \int \phi^2 =1$. We define the {\it static jet} centered at the origin $x=0$ as
\begin{equation}
	W_{\xi,r_\perp,r_\parallel}^p (x) := \psi_{r_\parallel}(x)\phi_{r_\perp}(x) \xi \, ,
\end{equation}
where $\xi^\perp:= (-\xi_2,\xi_1)$ and
\begin{equation}
	\psi_{r_\parallel}(x)
	:= 
	\frac{1}{r_\parallel^{1/2}} \psi\left( \frac{x\cdot \xi}{r_\parallel}\right)\, ,
	\quad
	\phi_{r_\perp}(x)
	:=
	\frac{1}{r_\perp^{1/2}}
	\phi\left( \frac{x\cdot \xi^\perp}{r_\perp}\right) \, . 
\end{equation}
With a slight abuse of notation, $W^p_{\xi,r_\perp,r_\parallel}(x)$ denote its $1$-periodic extension when $x\in \mathbb{T}^2$.








\subsection{Correction of the divergence}


The static jet $W_{\xi,r_\perp,r_\parallel}^p$ is not divergence free:

\begin{align}
	\div(W_{\xi,r_\perp,r_\parallel}^p)(x) 
	=
    \frac{1}{r_\perp} \, \cdot \frac{1}{r_\parallel^{1/2}} \psi'\left( \frac{x\cdot \xi}{r_\parallel}\right)\, \cdot \frac{1}{r_\perp^{1/2}} \phi\left( \frac{x\cdot \xi^\perp}{r_\perp}\right)
\end{align}
With the obvious notation, we define the {\it divergence corrector} as
\begin{equation}
	W_{\xi,r_\perp,r_\parallel}^c(x) :=  \frac {r_\perp}{r_\parallel} \,
	\psi'_{r_\parallel} 
	 \Phi''_{r_\perp}\, \xi^\perp \, .
\end{equation}
Notice that
\begin{equation}
	\div(W_{\xi,r_\perp,r_\parallel}^p + W_{\xi,r_\perp,r_\parallel}^c) = 0 \, .
\end{equation}




\subsection{The potential matrix $A$}


In this section we build smooth, symmetric potentials $A_{\xi,r_\perp,r_\parallel}^p, A_{\xi,r_\perp,r_\parallel}^c : \mathbb{T}^2 \to \mathbb{R}^{n\times n}$ such that
\begin{equation}\label{eq:A}
	\div (A_{\xi,r_\perp,r_\parallel}^p) = W_{\xi,r_\perp,r_\parallel}^p \, , 
	\quad
	\div(A_{\xi,r_\perp,r_\parallel}^c) = W_{\xi,r_\perp,r_\parallel}^c \, .
\end{equation} 
It is immediate to check that the following satisfy \eqref{eq:A}: 

\begin{align}
	A^p_{\xi,r_\perp,r_\parallel}(x) & : = - r_\perp \,  \cdot  \left(\xi \otimes \xi^\perp + \xi^\perp \otimes \xi \right)
	\, \cdot  \frac{1}{r_\parallel^{1/2}} \psi\left( \frac{x\cdot \xi}{r_\parallel}\right)\, \cdot \frac{1}{r_\perp^{1/2}} \Phi''\left( \frac{x\cdot \xi^\perp}{r_\perp}\right)
	\\& \quad \quad
	+ r_\perp\, \cdot \frac{r_\perp}{r_\parallel}\, \cdot  \xi^\perp\otimes \xi^\perp\, \cdot 
	\frac{1}{r_\parallel^{1/2}} \psi'\left( \frac{x\cdot \xi}{r_\parallel}\right)\, \cdot \frac{1}{r_\perp^{1/2}} \Phi'\left( \frac{x\cdot \xi^\perp}{r_\perp}\right)
	\\
	A_\xi^c(x) & := \frac{r_\perp}{r_\parallel}\, \cdot 
	r_\perp\,  \cdot  \left(\xi \otimes \xi^{\perp} + \xi^{\perp}\otimes \xi \right)
	\, \cdot  \frac{1}{r_\parallel^{1/2}} \psi'\left( \frac{x\cdot \xi}{r_\parallel}\right)\, \cdot \frac{1}{r_\perp^{1/2}} \Phi'\left( \frac{x\cdot \xi^\perp}{r_\perp}\right)
	\\& \quad \quad
	- r_\perp\, \cdot \left(\frac{r_\perp}{r_\parallel}\right)^2\, \cdot  \xi^\perp\otimes \xi^\perp\, \cdot 
	\frac{1}{r_\parallel^{1/2}} \psi''\left( \frac{x\cdot \xi}{r_\parallel}\right)\, \cdot \frac{1}{r_\perp^{1/2}} \Phi\left( \frac{x\cdot \xi^\perp}{r_\perp}\right)
\end{align}



The following estimates hold:
\begin{align}
	&\| A^p_{\xi,r_\perp,r_\parallel} \|_{L^1} + \frac{r_\parallel}{r_\perp} \| A_{\xi,r_\perp,r_\parallel}^c\|_{L^1}
	\le C(\xi,\psi,\Phi) r_\perp (r_\perp r_\parallel)^{1/2}
	\\
	&\| \xi \cdot \nabla A^p_{\xi,r_\perp,r_\parallel} \|_{L^1} + \frac{r_\parallel}{r_\perp} \| \xi \cdot \nabla A_{\xi,r_\perp,r_\parallel}^c\|_{L^1}
	\le C(\xi,\psi,\Phi) r_\perp \left(\frac{r_\perp}{r_\parallel}\right)^{1/2}
\end{align}




\subsection{Orbit of the center}
Given a smooth positive function $a: \mathbb{T}^2 \to (0,\infty)$ and a parameter $\mu_0>0$, we define
\begin{equation}
	\mu(x) = \frac{\mu_0}{a(x)} \, .
\end{equation}
Let $x(t)$ be solving the following equation with $x(0) = 0$:
\begin{equation}
	x'(t) = \mu(x(t)) \xi \,  .
\end{equation} 
The orbit $x(t)$ is periodic, with period
\begin{equation}
	T_\xi = \frac{1}{\mu_0}\int_0^{\tilde T_\xi} a(s\xi)\, ds
\end{equation}
where $\tilde T_\xi$ is the period of $t \xi$.


\begin{lemma}
	\begin{equation}
		\Big| T_\xi - \frac{\tilde T_\xi}{\mu_0} \int_{\mathbb{T}^2} a(x)\, dx \Big|
		\le \frac{\| \nabla a \|_{L^\infty}}{\mu_0} \, .
	\end{equation}
\end{lemma}

\begin{proof}
	The trajectory $t\xi$ is $1/\tilde T_\xi$-dense...
\end{proof}





The {\it moving axis} are defined as
\begin{align}
	r_\parallel(t)
	:= 
	a(x(t)) r_\parallel^0 \, ,
	\quad 
	r_\perp(t):= a(x(t)) r_\perp^0 \, ,
\end{align}

{\color{red}
	Probably better notation $r_0^\perp$?
}

\bigskip


where $r_\perp^0 \le r_\parallel^0 \le 1$ will be chosen later. Notice that 
\begin{equation}
	\frac{r_\perp(t)}{r_\parallel(t)} = \frac{r_\perp^0}{r_\parallel^0} < 1 \, ,
\end{equation}
is independent of time.


\bigskip

The {\it moving jet} and its potential matrix is defined according to
\begin{align}
	&W^p_\xi(x,t):= W_{\xi, r_\perp(t), r_\parallel(t)}^p(x-x(t)) \, ,
	\\
	&W^c_\xi(x,t):= W_{\xi, r_\perp(t), r_\parallel(t)}^c(x-x(t)) \, ,
	\\
	&A^p_\xi(x,t):= A_{\xi, r_\perp(t), r_\parallel(t)}^p(x-x(t)) \, ,
	\\
	&A^c_\xi(x,t):= A_{\xi, r_\perp(t), r_\parallel(t)}^c(x-x(t)) \, .
\end{align}


{\color{blue}MAYBE HERE ALL THE ESTIMATE ON $W$ AND $A$}


\subsection{Time correction}

We define the {\it first time corrector} as
\begin{align}
	Q_{\xi}^1(x,t) := \frac{a(x(t))}{\mu_0}\, \cdot \frac{1}{r_\parallel(t)} \psi^2\left( \frac{(x-x(t))\cdot \xi}{r_\parallel(t)}\right)\, \cdot \frac{1}{r_\perp(t)} \phi^2\left( \frac{(x-x(t))\cdot \xi^\perp}{r_\perp(t)}\right)\cdot \xi \, .
\end{align}


\begin{propos}
	The following equation is satisfied:
	\begin{align}
		\partial_t  Q_{\xi}^1 + \div(W^p_\xi\otimes W^p_\xi)
		=
		\frac{\xi \cdot \nabla a (x(t))}{a(x(t))}\, \cdot  V_\xi(x,t) \, ,
	\end{align}
    where $V_\xi$ is a smooth velocity field satisfying
    \begin{itemize}
    	\item[(i)] $\int V_\xi(x,t)\, dx = \xi$ for every $t\in \mathbb{R}$,
    	
    	\item[(ii)] $\supp V_\xi(\cdot,t) \subset B_{10 r_\parallel(t)}(x(t))$.
    \end{itemize}
\end{propos}

\begin{proof}
	Explicit expression for $V_\xi$
	 \begin{align}
		V_\xi(x,t) = -\frac{\xi \cdot \nabla a(x(t))}{a(x(t))}
		\left( (\psi^2)_{r_\parallel(t)}(\phi^2)_{r_\perp(t)} + (2\psi'\tilde \psi)_{r_\parallel(t)} (\phi^2)_{r_\perp(t)} 
		+ 
		(\psi^2)_{r_\parallel(t)}
		(2\phi' \tilde \phi)_{r_\perp(t)}  \right)
	\end{align}
	where $\tilde \phi(y) = y \phi(y)$.
	
	
	\bigskip
	
	
	
	\begin{align}
		\div (W_\xi^p \otimes W_\xi^p) 
		&=
		\frac{2}{r_\parallel}\, \cdot \frac{1}{r_\parallel} (\psi\cdot \psi') \left(\frac{(x-x(t))\cdot \xi}{r_\parallel}\right) 
		\, \cdot \frac{1}{r_\perp} \phi^2 \left(\frac{(x-x(0))\cdot \xi^\perp}{r_\perp}\right)\, \cdot \xi
	\end{align}
	
	
\end{proof}




The following estimates hold for every $t\in \mathbb{R}$:
\begin{align}
	&\| \nabla Q^1_\xi(\cdot, t) \|_{L^p}
	\le \frac{C }{\mu_0 r_\perp^0} (r_\perp(t) r_\parallel(t))^{1-1/p}
	\\
	& \| Q^1_\xi(\cdot,t)\|_{L^2}
	\le \frac{C}{\mu_0} \frac{1}{(r_\perp^0 r_\parallel^0)^{1/2}} \, .
\end{align}



\subsection{The time average}

We consider an auxiliary jet with constant axis $r_0^\perp(t) = r_0^\parallel(t) = r$,
\begin{align}
	&U_{\xi, r}(x) 
	:= \frac{1}{r} \psi^2\left( \frac{x\cdot \xi}{r}\right)\, \cdot \frac{1}{r} \phi^2\left( \frac{x\cdot \xi^\perp}{r}\right)\cdot \xi
	\\
	&U_{\xi,r}(x,t) := U_{\xi,r}(x-x(t)) \, ,
\end{align}
and we study its time average over a period $T_\xi$.



\bigskip

{\color{red}
We Will choose $r = 1/\lambda$ in the sequel..
}



\begin{lemma}
	Let $f\in C^\infty(\mathbb{R})$, it holds
	\begin{align}
		\frac{1}{T_\xi} \int_0^{T_\xi} f(x(s)) U_{\xi,r}(x,s)\, ds 
		= 
		\frac{f(x) a(x)}{\mu_0}\, \frac{1}{T_\xi}
		\tilde{\phi_r}(x)^2\, \xi 
		+ e_1(x)
	\end{align}
    where $\tilde{\phi_r}(x) = \sum_{k\in \mathbb{Z}^2} \phi_r(x+k)$ is the $1$-periodic extension of $\phi_r$ and 
    \begin{equation}
    	|e_1(x)| \le 2 \frac{r}{\mu_0} \| \nabla fa\|_{L^\infty} \, \cdot  \frac{1}{T_\xi}\, \cdot \tilde{\phi_r}(x)^2\, .
    \end{equation}
\end{lemma}

\begin{proof}
	We change variables according to
	\begin{equation}
		x(s(t)) = t \xi \, . 
	\end{equation}
    Notice that $s'(t) = a(t\xi)/\mu_0$, hence
    \begin{align}
    	\frac{1}{T_\xi} \int_0^{T_\xi}& 
    	f(x(s)) U_{\xi,r}(x,s)
    	\, ds
    	\\& =
    	\frac{1}{T_\xi} \int_0^{\tilde T_\xi} \frac{1}{\mu_0} f(t\xi)a(t\xi) U_{\xi,r}(x-t\xi)\, dt
    	\\&
    	= \frac{f(x)a(x)}{\mu_0}\, \cdot \frac{1}{T_\xi} \int_0^{\tilde T_\eps} U_{\xi,r}(x-t\xi)\, dt + e(x)
    	 \, ,
    \end{align}
where $\tilde T_\xi$ is the period of $\xi t$ and 
\begin{equation}
	|e_1(x)| \le 2 \frac{r_0}{\mu_0} \| \nabla fa\|_{L^\infty} \, \cdot  \frac{1}{T_\xi} \int_0^{\tilde T_\eps} |U_{\xi,r_0}|(x-t\xi)\, dt \, .
\end{equation} 
Finally, we observe that if $r \le C(\xi)$, then
\begin{align}
	\frac{1}{T_\xi}\int_0^{\tilde T_\xi} U_{\xi,r}(x - t\xi)\, dt
	& =
	\frac{1}{T_\xi}\, 
	\cdot  \int \psi^2(t)\, dt \, 
	\cdot \tilde{\phi_r}(x)^2 \xi
	\\&
	 = \frac{1}{T_\xi} \, \cdot  \tilde{\phi_r}(x)^2  \xi \, .
\end{align}


\end{proof}








\section{Decomposition of the error}

Let $\lambda\in \mathbb{N}$, $\lambda \ge 10$. We decompose the error $R_0(x,t)$ according to
\begin{equation}
	-\div(R_0) = \div\left(\sum_{i=1}^4 a_i^2(x,t) \xi_i\otimes\xi_i\right) + \nabla P \, ,
\end{equation}
where
\begin{itemize}
	\item[(i)] $\xi_1 := (1,1/\lambda)/c_1$, $\xi_2 :=(1/\lambda,1)/c_2$, $\xi_3 :=(1+1/\lambda,-1)/c_3$, $\xi_4:= (1+1/\lambda,1)c_4$. Where $c_i> 0$ are normalizing constants to ensure $|\xi_i|=1$.
	
	
	
	\item[(ii)] The coefficients $a_i(x,t)$ are smooth and satisfy the following estimates
	\begin{align}
		& a_i^2(x,t) \ge \| R_0 \|_{L^\infty_tL_x^1}
		\\
		& \| a_i \|_{L^\infty_tL_x^1} \le C \| R_0 \|_{L^\infty_tL_x^1}^{1/2}
		\\
		& \| \partial_t^M \nabla^N a_i\|_{L^\infty} \le C(M,N) \| \partial_t^M \nabla^N R_0\|_{L^\infty} \, .
	\end{align}
\end{itemize}



\section{The perturbation}
Let $\mu_0, \tau >0$ such that $\frac{1}{\tau} \in \mathbb{N}$, $\frac{1}{\tau} \ge 10$.
For every $k\in \{0, \ldots, 1/\tau -1\}$ we define $I_k:=[k\tau, (k+1)\tau]$ and time cut-off
\begin{equation}
	\chi_{i,k}(t) := \chi\left(\frac{t-k\tau-(i-1)/4}{\tau/4}\right) \, , \quad i\in \{1,2,3,4\}\, ,
\end{equation}
where $\chi$...



\subsection{Adapted moving jets}

\begin{equation}
	a_{ki}(x):= \frac{1}{\tau} \int_{k\tau}^{(k+1)\tau} a_i^2(x,t)\, dt
\end{equation}

\begin{equation}
	\mu_{ki}(x):= \frac{\mu_0}{a_{ki}^2(x)}
\end{equation}
{\color{blue}
Notice that
\begin{equation}
	\frac{\mu_0}{C\| R_0 \|_{L^\infty}}
	\le
	\| \mu_{ki} \|_{L^\infty} \le \frac{\mu_0}{\| R_0 \|_{L^\infty_t L_x^1}}
\end{equation}
}




Let $x_{ki}: \mathbb{R} \to \mathbb{T}^2$ solve
\begin{equation}
	\begin{cases}
		& x_{ki}'(t) = \mu_{ki}(x_{ki}(t)) \xi_i
		\\
		& x_{ki}(0) = 0
	\end{cases}	
\end{equation}
We denote by $T_{ki}$ the period of $x_{ki}$, from ..., we deduce that
\begin{equation}
	\Big|T_{ki} - \frac{c_i\lambda}{\mu_0}\int_{\mathbb{T}^2} a_{ik}^2 \Big|
	\le C \frac{\|\nabla R_0\|_{L^\infty}}{\mu_0}\, .
\end{equation}
Notice that the $\tilde T_{ki}$, the period of $t\xi_i$, coincides with $c_i \lambda$.


Following the notation in .... we set
\begin{align}
	& W_{ki}^p(x,t) = W_{\xi_i}^p(x,t) \, , 
	\quad
	W_{ki}^c(x,t) = W_{\xi_i}^c(x,t) \, , 
	\\
	& A_{ki}^p(x,t) := A_{x_i}^p(x,t)\, ,
	\quad 
	A^x_{ki}(x,t) = A_\xi^c(x,t)\, , 
	\\
	&Q^1_{ki}(x,t) = Q^1_{\xi_i}(x,t)\, ,
	\\
	& U_{ki}(x,t) := U_{\xi, 10^{-10}/\lambda}(x,t)\, .
\end{align}


\subsection{The perturbation}

Let $U_0\ge 0$ to be fixed later.


\begin{equation}
	u_1(x,t) = u_0(x,t) + u_1^{(p)}(x,t) + u_1^{(t)}(x,t) + Q^2(x,t)
\end{equation}


\begin{equation}
	u_1^{(p)}(x,t) := U_0 \sum_{ki} \chi_{ki}(t)(W_{ki}^p(x,t) + W_{ki}^c(x,t)) \, , 
	\quad
	u_1^{(t)} := U_0^2 \sum_{ki} \chi_{ki}(t) \mathbb{P} Q_{ki}(x,t)
\end{equation}


Finally, the second temporal corrector
\begin{equation}
	Q^2_{ki}(x,t) := U_0^2\int_0^t \sum_{ki} \chi_{ki}^2(s) \frac{\xi \cdot \nabla a(x(s))}{a(x(s))} (U_{ki}(x,s) - P_\tau U_{ki}(x,s))\, ds \, .
\end{equation}





\subsection{Estimate on $\|u_1 - u_0\|_{L^p}$}



\begin{align}
	&\| u_1^{(p)}(\cdot,t) \|_{L^p} \le U_0 (\| W^p_{ki}(\cdot,t) \|_{L^p} + \| W_{ki}^c(\cdot,t)\|_{L^p}
	\le 4 U_0 (r_\parallel r_\perp)^{1/p-1/2} \, .
\end{align}
As a consequence of ... for every $1<p< \infty$ it holds
\begin{equation}
	\| u_1^{(t)}(\cdot, t) \|_{L^p} \le C(p) U_0^2 \frac{\| R_0 \|_{L^\infty}}{\mu_0 } (r_\parallel r_\perp)^{1/p - 1}\, .
\end{equation}
Finally, we estimate
\begin{equation}
	\| Q^2(\cdot, t) \|_{L^p}...
\end{equation}





\section{The new error}
We define the new error $R_1$ such that
\begin{equation}
	\partial_t u_1 + \div(u_1 \otimes u_1) + \nabla p_1 = \div(R_1) \, ,
\end{equation}
which by subtracting the equation for $u_0$ gives
\begin{align}
		\div(R_1) & = \div( u_0 \otimes (u_1-u_0) +  (u_1-u_0) \otimes u_0 + (u_1-u_0) \otimes (u_1-u_0) + R_0)
		\\& \qquad  + \partial_t (u_1 - u_0) + \nabla (p_1 - p_0) \, .
\end{align}
We are going to define 
\begin{equation}
	R_1 := R_1^{(l)} + R_1^{(t)} + R_1^{(q)} \, ,
\end{equation}
where the various addends are defined in the following paragraphs, and show that
\begin{equation}
	\| R^{(l)}_1\|_{L^1} + \| R^{(t)} \|_{L^1} +  \| R^{(q)} \|_{L^1} \le \eps C(t_0, \| R_0\|_{C^3}) \, .
\end{equation}


\subsection{Linear error}
Let us set
\begin{equation}\label{eq:linear error}
	R^{(l)}_1 :=  u_0 \otimes (u_1-u_0) +  (u_1-u_0) \otimes u_0 \, ,
\end{equation}



\begin{align}
	\| R^{(l)}_1\|_{L^\infty_t L^1_x} \le 2 \| u_0 \|_{L^\infty} \| u_1 - u_0 \|_{L^\infty_t L_x^1 }
	\le 
\end{align}



\subsection{Temporal error} 
Let us set


\begin{align}
	R_1^{(t)} & := U_0\sum_k \sum_i \chi'_{ki}(t) A_{ki} + U_0\sum_{ki} \chi_{ki}(t) \partial_t A_{ki} 
	\\& \quad 
	+U_0^2 \sum_k \sum_i \chi'_{ki}(t) \mathcal{R}\mathbb{P} Q_{ki}
\end{align}



\subsection{Quadratic error}








\section{Estimates on building blocks}
In this section we collect the relevant estimates on the building blocks.
Given $N\ge 0$ we write 
$D^N = D^{\left \lfloor{N}\right \rfloor  } \Delta^{s/2}$
where $\left \lfloor{N}\right \rfloor$ is the integer part of $N$,
$s:= N - \left \lfloor{N}\right \rfloor$ and $D^{\left \lfloor{N}\right \rfloor  }$ is the standard derivative operator.











\begin{lemma}\label{lemma: first estimates}
	For any $N\in [0,\infty)$, $M\ge 0$ integer and $p\in [1,\infty]$ there exists $C=C(N,M,p,|\xi|,\Phi,\psi)>0$ such that the following hold.
	\begin{equation}
		\| D^N \partial_t^M \psi_{(\xi)} \|_{L^p(\TT)} \le C {\lambda}^{-1/p} r_\parallel^{1/p - 1/2} \left( \frac{ \lambda}{r_\parallel} \right)^N  \left( \frac{ \lambda \mu}{r_\parallel} \right)^M \, ,
	\end{equation}

	\begin{equation}
		\| D^N (\Phi')_{(\xi)}\|_{L^p(\TT)} 
		+ \| D^N (\Phi'')_{(\xi)}\|_{L^p(\TT)}
		+	\| D^N \phi_{(\xi)}\|_{L^p(\TT)}
		\le C  {\lambda}^{-1/p} r_\perp^{1/p-1/2} \left( \frac{ \lambda}{r_\perp} \right)^N \, ,
	\end{equation}

	\begin{equation}
		\| D^N \partial_t^M W_{(\xi)}^{\alpha} \|_{L^p(\TT^2)} + \frac{r_{\parallel}}{r_\perp} \| D^N \partial_t^M (W_{(\xi)}^{\alpha})^c \|_{L^p(\TT^2)}
		\le C  {\lambda}^{-2/p} (r_{\parallel}r_\perp)^{1/p-1/2} \left(\frac{\lambda}{r_\perp}\right)^N \left( \frac{ \lambda \mu}{r_\parallel} \right)^M \, ,
	\end{equation}

	\begin{equation}
		\mu \| D^N \partial_t^M Q_{(\xi)}^{\alpha}\|_{L^p(\TT^2)}
		\le 
		C {\lambda}^{-2/p} 
		(r_{\parallel}r_\perp)^{1/p-1} \left(\frac{\lambda}{r_\perp}\right)^N \left( \frac{ \lambda \mu}{r_\parallel} \right)^M \, .
	\end{equation}
\end{lemma}
The proof of Lemma \ref{lemma: first estimates} is a simple computation, so we omit it. 



 \begin{equation}\label{eq: W L2}
	\| W_{(\xi)}^{\alpha} \|_{L^2(\TT^2)} + \frac{r_{\parallel}}{r_\perp} \|( W_{(\xi)}^{\alpha})^c \|_{L^2(\TT^2)}
	\le C \lambda^{-1}\, 
\end{equation}
(in particular, this says that the principal part is much smaller than the corrector),
\begin{equation}\label{eq: Q L2}
		\| Q^\alpha_{(\xi)} \|_{L^2(\TT^2)} 
		\le \frac{C}{\mu\lambda (r_\parallel r_\perp)^{1/2}} \, ,
\end{equation}
%and
%\begin{equation}\label{eq: W Lp}
%	\| W_{\xi,K,n_0}^p \|_{L^p(\TT^2)} + \frac{r_{\parallel}}{r_\perp} \| W_{\xi,K,n_0}^c \|_{L^p(\TT^2)}
%	\le C \frac{(r_\perp r_\parallel)^{1/p-1/2}}{K^{1/2}} \, ,
%	\quad \text{for any $p\in [1,2)$} \, .
%\end{equation}
	Moreover, it holds
\begin{equation}
	\| D W_{(\xi)}^{\alpha} \|_{L^1(\TT^2)} + \frac{r_{\parallel}}{r_\perp} \| D (W_{(\xi)}^{\alpha})^c \|_{L^1(\TT^2)}
	\le 
	\frac{C}{\lambda} \left(\frac{r_{\parallel}}{r_\perp}\right) ^{1/2} \, ,
\end{equation}

\begin{equation}
	 \| D Q_{(\xi)}^{\alpha} \|_{L^1(\TT^2)}
	\le 
	C
	%(r_{\parallel}r_\perp)^{1/p-1} 
    \frac{1}{\mu \lambda r_\perp}
	\, .
\end{equation}
%where $\gamma:= -s - 1 + 2/p >0$. In particular
% \begin{equation}\label{eq: W Ds}
%	\| D^s W_{\xi,K,n_0}^p \|_{L^p(\TT^2)} + \frac{r_{\parallel}}{r_\perp} \| D^s W_{\xi,K,n_0}^c \|_{L^p(\TT^2)}
%	\le C 2^{- n_0 \gamma} K^{-1/2}(r_{\parallel}r_\perp)^{1/p-1/2} \left(\frac{\lambda}{r_\perp}\right)^s
%	\, ,
%\end{equation}
%
%
%
%\begin{equation}\label{eq: Q Ds}
%	\| D^s Q_{\xi,K,n_0} \|_{L^p(\TT^2)} 
%	\le 
%	C2^{ - n_0 \gamma} \mu^{-1} K^{-1}
%	(r_{\parallel}r_\perp)^{1/p-1} \left(\frac{\lambda}{r_\perp}\right)^s  \, .
%\end{equation}
%



%
%\begin{lemma}[Gradient estimates]\label{lemma: Lorentz}
%There exists $C=C(|\xi|, \Phi,\psi)>0$ such that
%\begin{equation}
%	\| D W_{\xi,K,n_0} \|_{L^{1,\infty}} \le C\frac{ \lambda}{K^{1/2}} \left(\frac{ r_\parallel}{r_\perp} \right)^{1/2}\, ,
%\end{equation}
%%	\begin{equation}
%%		\| \omega_{\xi,K,n_0} \|_{L^{1,q}} \le \frac{C n_* \lambda_{q+1}}{K^{1/2-1/q}} \left(\frac{ r_\parallel}{r_\perp} \right)^{1/2}\, ,
%%	\end{equation}
%   \begin{equation}
%   	\| D Q_{\xi,K,n_0} \|_{L^{1,\infty}} \le C \frac{\lambda}{\mu r_\perp K} \, .
%   \end{equation}
%\end{lemma}
%
%
%\begin{proof}
%	Observe that
%	\begin{align*}
%		|D W_{(\xi)}^k| & =	\lambda 2^k | r_\parallel^{-1} \frac{\xi}{|\xi|} \otimes \frac{\xi}{|\xi|} (\psi')^k_{(\xi)}(x,t)\phi^k_{(\xi)}(x)
%		+  r_\perp^{-1} \frac{\xi}{|\xi|}\otimes \frac{\xi^\perp}{|\xi|} \psi^k_{(\xi)}(x,t)(\phi')^k_{(\xi)}(x)|
%		\\& \le  \lambda 2^k r_\perp^{-1}  ( |(\psi')^k_{(\xi)}(x,t)||\phi^k_{(\xi)}(x)| + |\psi^k_{(\xi)}(x,t)||(\phi')^k_{(\xi)}(x)|   )
%		\\& = \lambda \left(\frac{ r_\parallel}{r_\perp} \right)^{1/2}  \frac{1}{2^{-k}(r_\perp r_\parallel)^{1/2}}( |(\psi')^k_{(\xi)}(x,t)||\phi^k_{(\xi)}(x)| + |\psi^k_{(\xi)}(x,t)||(\phi')^k_{(\xi)}(x)|   )
%		\\& := \lambda\left(\frac{ r_\parallel}{r_\perp} \right)^{1/2} \Omega_1^k(x,t) \, ,
%	\end{align*}
%and similarly
% \begin{align*}
%    	| D Q_{(\xi)}^k | \le \frac{\lambda}{\mu r_\perp} \Omega_2^k(x,t) \, ,
%    \end{align*}
%        where for $i=1,2$
%    \begin{equation}\label{z1}
%    	|\Omega_i^k| \le C 2^{2k}(r_\perp r_\parallel)^{-1}\, ,
%    	\quad
%    	\Leb2(\supp (\Omega_i^k)) \le C 2^{-2k} r_\perp r_\parallel \, ,
%    	\quad
%    	\supp(\Omega_i^k)\cap \supp(\Omega_i^{k'})= \emptyset\, , \, \, \, \text{for $k\neq k'$} \, .
%    \end{equation}
%    Let us now fix $s\ge 1$ and $k_*$ the smallest integer satisfying $k_*\ge n_0+1$ and $C2^{2k_*} \ge s K^{1/2} r_\perp r_\parallel$. It holds
%    \begin{equation}
%    \Leb2\left(\left\lbrace\frac{1}{K^{1/2}} \sum_{k=n_0+1}^{K + n_0} \Omega_1^k \ge s \right\rbrace \right)
%    =
%    \sum_{k = n_0+1}^{K + n_0} \Leb2(\{\Omega_1^k \ge s K^{1/2}\})
%    \le 
%    \sum_{k=k_*}^{K + n_0} \Leb2(\{\Omega_1^k \ge s K^{1/2}\}) \, .
%    \end{equation}
%    From \eqref{z1} and the choice of $k_*$ we get
%    \begin{align*}
%    	\sum_{k=k_*}^{K + n_0} \Leb2(\{\Omega_k \ge s K^{1/2} \})
%    	\le
%    	\sum_{k=k_*}^{K+n_0} C 2^{-2k} r_\perp r_\parallel
%    	\le  \frac{C}{ s K^{1/2}}\sum_{k\ge k_*} 2^{2k_*-2k} 
%    	 \le \frac{C}{s K^{1/2}}\, ,
%    \end{align*}
%    hence
%    \begin{equation}
%    	\| D W_{\xi,K,n_0}^p \|_{L^{1,\infty}}
%    	\le 
%    	  \lambda\left(\frac{ r_\parallel}{r_\perp} \right)^{1/2} \Big\|  \frac{1}{K^{1/2}} \sum_{k=n_0+1}^{K+n_0} \Omega^k \Big\|_{L^{1,\infty}}
%    	 \le C^2 \frac{\lambda}{K^{1/2}} \left(\frac{ r_\parallel}{r_\perp} \right)^{1/2}\, ,
%    \end{equation}
%   the estimate on $\| D W^c_{\xi,K,n_0} \|_{L^{1,\infty}}$ can be obtained following the same strategy.
%   An analogous argument gives
%   \begin{equation}
%   	\Leb2\left(\left\lbrace\frac{1}{K} \sum_{k=n_0+1}^{K + n_0} \Omega_2^k \ge s \right\rbrace \right)
%   	\le \frac{C}{s K} \, ,
%%   	=
%%   	\sum_{k = n_0+1}^{K + n_0} \Leb2(\{\Omega_1^k \ge t K^{1/2}\})
%%   	\le 
%%   	\sum_{k=k_*}^{K + n_0} \Leb2(\{\Omega_1^k \ge t K^{1/2}\}) \, ,
%   \end{equation}
%   yielding
%   \begin{equation*}
%   	\| D Q_{\xi,K,n_0} \|_{L^{1,\infty}}
%   	\le 
%   	C\frac{\lambda}{\mu r_\perp} \Big\|  \frac{1}{K} \sum_{k=n_0+1}^{K+n_0} \Omega^k \Big\|_{L^{1,\infty}}
%   	\le 
%   	C^2 \frac{ \lambda}{ \mu r_\perp K}
%   	\, .\qedhere
%   \end{equation*}
%\end{proof}
%
%


%
%
%
%
%\begin{remark}\label{rmk:improved Lorentz}
%	It is not hard to prove the following extension of Lemma \ref{lemma: Lorentz}. For any $q\ge 1$ it holds
%	\begin{equation}
%		\| D W_{\xi,K,n_0} \|_{L^{1,q}} \le C\frac{ \lambda}{K^{1/2 - 1/q}} \left(\frac{ r_\parallel}{r_\perp} \right)^{1/2}\, ,
%	\end{equation}
%	\begin{equation}
%		\| D Q_{\xi,K,n_0} \|_{L^{1,\infty}} \le C \frac{\lambda}{\mu r_\perp K^{1-1/q}} \, .
%	\end{equation}
%\end{remark}








\section{Definition of perturbation}

$$I_\alpha = [\tau (\alpha-1), \tau \alpha) \qquad \alpha= 1,...,\tau^{-1},\; $$
$$I_\alpha = \cup_{i=1}^{\lambda^2} I_{\alpha,i} $$
$$\ell_{\alpha, i} = \tau^{-1} | I_{\alpha,i}|$$
so $\sum_i \ell_{\alpha, i} =1$.

$Q_i$ cubes of size $\lambda^{-1}$.

$$\bar R_0 = \sum_{i, \alpha} R_0^{i,\alpha} \chi_{Q_i}(x) \chi_{I_\alpha}(t)$$

$$R_0^{i,\alpha}  = \mean{Q_i \times I_\alpha} R_0 = \frac 1 \tau \int_{\tau(\alpha-1)}^{\tau\alpha} \lambda^2 \int_{Q_i} R_0$$

Observe
$$\|\bar R_0- R_0 \|_{C^0_{x,t}} \leq \max\left\{ \lambda^{-2}, \tau\right\} \|R_0\|_{C^1_{x,t}}.$$
Define
$$\delta_{i,\alpha} =\int_{Q_i \times I_\alpha} |R_0|, \qquad \delta_{\alpha}= \sum_{i=1}^{\lambda^2} \delta_{i,\alpha}$$
so that $|R_0^{i,\alpha}| \leq \frac{\lambda^2}{\tau}  \delta_{i,\alpha}$.

Define the perturbation
$$W =  \sum_{\alpha=1}^{\tau^{-1}} \sum_{i=1}^{\lambda^2} \sqrt{R_0^{i,\alpha}
} \chi_{I_i}(t)  \frac 1 {\sqrt{\ell_i} r} W$$
$$\ell_{i,\alpha} = \frac 1 2 \Big(\frac{ \delta_{i,\alpha}}{ \delta_\alpha} + \frac 1 \lambda\Big)
$$
[In reality there are five different building blocks and weights ]

With this definition we have
$$\|W\|_{L^2} + \|\nabla W\|_{L^1} \leq \delta
$$



